Contextual Combinatorial Bandits with Probabilistically Triggered Arms

We study contextual combinatorial bandits with probabilistically triggered arms (C$^2$MAB-T) under a variety of smoothness conditions that capture a wide range of applications, such as contextual cascading bandits and contextual influence maximization bandits. Under the triggering probability modulated (TPM) condition, we devise the C$^2$-UCB-T algorithm and propose a novel analysis that achieves an $\tilde{O}(d\sqrt{KT})$ regret bound, removing a potentially exponentially large factor $O(1/p_{\min})$, where $d$ is the dimension of contexts, $p_{\min}$ is the minimum positive probability that any arm can be triggered, and batch-size $K$ is the maximum number of arms that can be triggered per round. Under the variance modulated (VM) or triggering probability and variance modulated (TPVM) conditions, we propose a new variance-adaptive algorithm VAC$^2$-UCB and derive a regret bound $\tilde{O}(d\sqrt{T})$, which is independent of the batch-size $K$. As a valuable by-product, our analysis technique and variance-adaptive algorithm can be applied to the CMAB-T and C$^2$MAB setting, improving existing results there as well. We also include experiments that demonstrate the improved performance of our algorithms compared with benchmark algorithms on synthetic and real-world datasets.

==> content/10_icml_rebuttal.tex <==
\clearpage
\onecolumn
\section{Rebuttal}

\subsection{Reviewer 7kVf: score 6 (weak accept), confidence 4}
\textbf{About the regret lower bound for Table 2.}

We thank the reviewer for the positive comments.
In general, our results match the (known) lower bounds with a factor up to $\tilde{O}(\sqrt{d})$, where the details are as follows.

For Online Influence Maximization (Table 2, row 1), to the best of our knowledge, there are no existing lower bounds, even for the non-contextual case (i.e., we assume the features for arm $i\in [d]$ are one-hot vectors $e_i$ as in Remark 1). Likewise, for conjunctive cascading bandits (Table 2, row 3), the non-contextual case lower bound is also an open problem. The lower bounds for these cases will be left for future work.

For disjunctive cascading bandits (Table 2, row 2) and linear cascading bandits (Table 2, row 4), there are no known lower bounds for the contextual setting, but for the non-contextual setting, [Vial et al. 2022] give a lower bound of $\Omega(\sqrt{dT})$, and our result matches the lower bound up to a factor of $\tilde{O}(\sqrt{d})$.

For Multi-layered network exploration (Table 2, row 5) and PMC (Table 2, row 6), we also consider the non-contextual setting where [1] gives a $\Omega(\sqrt{d|V|T}/\log(k))$ lower bound, and our result matches the lower bound regret up to a factor of $\tilde{O}(\sqrt{d})$. 

There is also one notable case (which does not appear in Table 2) for the contextual CMAB with the linear reward function where $r(S;\mu)=\sum_{i \in S} \mu_i$: [Takemura et al. 2021] give the lower bound $\Omega(d\sqrt{KT})$ when total number of base arms $m=\Theta(K\cdot2^d)$. Our work gives the $\tilde{O}(d\sqrt{KT})$ regret bound which matches the lower bound up to logarithmic factors. In the future, we will investigate whether the similar lower bound analysis can give some insights on whether the $O(d)$ dependence is necessary for rows 2, 4, 5, 6. If this $O(d)$ dependence is necessary, this means that our results are tight up to logarithmic factors.

[1] Merlis, Nadav, and Shie Mannor. "Tight lower bounds for combinatorial multi-armed bandits." Conference on Learning Theory. PMLR, 2020.


\subsection{Reviewer ob9a: score 3 (Reject), confidence 3}
\textbf{About the analysis involving the weighted least squared estimator.}

% We thank the reviewer for raising the concern about the technical correctness of the Lemma 2. If we understand it correctly, the reviewer thinks that we cannot use the self-normalized bound for the weighted least squared estimator since the vector $b_t$ involves weight ${V}_{t,i}$, which is related to the data for all $T$ rounds.  

% We first need to clarify that Equation (5) is just to give some intuition why our algorithm computes $\hat{\theta}_t$ as in line 4 of Algorithm 2 with weights $\bar{V}_{t,i}$ defined in Equation (6), but Equation (5) is actually not used in our algorithm or analysis. In our algorithm, since we do not know the true variance $V_{t,i}$, we use the optimistic weight $\bar{V}_{t,i}$ to estimate the true $V_{t,i}$, which is only related to the (observed) data before time $t$ (i.e., $\mathcal{H}_t$ defined in line 159), and is irrelevant to any data from rounds $t, t+1, \cdots, T$. Now given historical data $\cH_t$, the actual weighted least squared estimator of the true $\theta$ is given by 
% \begin{equation}
%     \hat{\theta}_t = \argmin_{\theta \in \Theta} \sum_{s<t}\sum_{i \in \tau_s}(\inner{\theta, \bphi_s(i)}-X_{s,i})^2/\bar{V}_{s,i} + \gamma \norm{\theta}_2^2,
% \end{equation}
% where the optimistic weights $\bar{V}_{t,i}$ for $t\in [T]$ are defined in Equation (6), and are only related to UCB and LCB values $\bar{\mu}_{t,i}$ and $\underline{\mu}_{t,i}$, which are all measurable given the historical data $\mathcal{H}_t$ before time $t$. And the closed-form solution for the above equation coincides with the line 4 of our Algorithm 2: $\hat{\theta}_{t}=G_{t}^{-1}b_{t}$ where the Gram matrix $G_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i) \phi_{s}(i)^{\top}$ and the b-vector $b_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i)X_{s,i}$. Again, the above equation is for the intuition of line 4, but not explicitly used in our analysis.

% For the correctness of our analysis, We agree that if $b_t$ is related to all $T$ rounds' data, Lemma 2 does not hold. But if we carefully check the indices $s$ that are accumulated over, $b_t$ is only related to weights $(\bar{V}_{s,i})_{s<t, i \in \tau_s}$ (determined by data $\mathcal{H}_{t-1}$ before time $t-1$) and observation $(\phi_s(i), X_{s,i})_{s<t, i \in \tau_s}$ (determined by data $\mathcal{H}_t$ before time $t$), which are enough to conduct the self-normalized bound analysis. Notably, we are not the only ones who use the weighted least square estimator with weights that are determined by historical data. For the classical contextual bandit setting, Lattimore et al., 2015 also adopt the idea of using the historical data in the self-normalized bound with weights $\bar{V}_{t,i}$ that are measurable by data before time $t$, and our analysis can cover theirs by setting the triggering arm set $\tau_t$ to be the single arm $M_t$ chosen for their respective algorithms. In particular, their weights $\gamma_{t}$ defined in Equation (2) shares the similar property as our $\bar{V}_{t,i}$, and we are largely inspired by their respective analysis of weighted least square estimation for their Theorem 3. We will add this clarification in our final version.

We thank the reviewer for the question. We believe that the reviewer is concerned about the analysis of our algorithm using the weighted least squared estimator, specifically the use of the weight vector $V_{t,i}$ that is related to data from all $T$ rounds.

We first want to clarify that Equation (5) is only intended to provide intuition for the weights $(\bar{V}_{s,i})_{s < t}$ in Algorithm 2 to compute $\hat{\theta}_t$, and is not used in our analysis or algorithm. Our algorithm uses the optimistic weight $\bar{V}_{t,i}$ to estimate the unknown true variance $V_{t,i}$. Note that $\bar{V}_{t,i}$ is only related to the observed data before time $t$ (i.e., it is calculated by Eq. (6) and only depends on $\mathcal{H}_t$), and is not relevant to any data from rounds $t, t+1, \cdots, T$. Concretely, given historical data $\mathcal{H}_t$, the actual weighted least squared estimator of the true parameter $\theta$ is given by:
$$\hat{\theta}_t = \argmin_{\theta \in \Theta} \sum_{s<t}\sum_{i \in \tau_s}(\inner{\theta, \bphi_s(i)}-X_{s,i})^2/\bar{V}_{s,i} + \gamma \norm{\theta}_2^2,$$
where the optimistic weights $\bar{V}_{s,i}$ could be different in each time step $s$. The closed-form solution for the above equation coincides with the line 4 of our Algorithm 2: $\hat{\theta}_t=G_t^{-1}b_t$ where the Gram matrix $G_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i) \phi_{s}(i)^{\top}$ and the b-vector $b_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i)X_{s,i}$.

Regarding the correctness of our analysis, we agree that if $b_t$ is related to all $T$ rounds' data, Lemma 2 does not hold. However, $b_t$ are only related to weights $(\bar{V}_{s,i})_{s<t, i \in \tau_s}$ (determined by data $\mathcal{H}_{t-1}$ before time $t-1$) and observation $(\phi_s(i), X_{s,i})_{s<t, i \in \tau_s}$ (determined by data $\mathcal{H}_t$ before time $t$), which are sufficient to conduct the self-normalized bound analysis. Notably, we are not the only ones who use the weighted least square estimator with weights that are determined by historical data.  For the classical contextual bandit setting, [Lattimore et al., 2015] also adopt this idea in their Section 4, and our analysis can cover theirs by setting the triggering arm set $\tau_t$ to be the single arm $M_t$ chosen by their respective algorithm. In particular, their weights $\gamma_{t}^{-1}$ defined in Equation (2) [Lattimore et al., 2015] shares the similar property as our $\bar{V}_{t,i}$, and we are largely inspired by their respective analysis of weighted least square estimation for their Theorem 3. We will add this clarification in our final version.





\textbf{About the 1-norm TPM smoothness condition (Condition 2).}

We thank the reviewer for this comment. We guess that the reviewer may confuse the triggering probability $p_i^{\mu, S}$ with the selection probability of the arm $i$. We kindly remind that $p_i^{\mu,S}$ represents the probability $i$ is observed after action $S$ is selected. For example, in cascading bandits,  given a list $S$ (or action), the user sequentially scans from the first item to the last item of $S$, and stops either he clicks any item in $S$ or exhausts the whole list. Suppose there are five items (base arms, indexed by 1-5) with click rates $\mu=(0.1, 0.2, 0.3, 0.4, 0.5)$, and the algorithm selects the first 3 arms as the action $S=(1,2,3)$. The triggering probability of each item is $p_1^{\mu, S}=1$, $p_2^{\mu,S}=1-0.1=0.9, p_3^{\mu,S}=(1-0.1)*(1-0.2)=0.72, p_4^{\mu,S}=p_5^{\mu,S}=0$. For the arm selection probability $p_i$, $p_i=1$ if $i \in S$ and $p_i= 0$ otherwise, so it is easy to check $p_1=p_2=p_3=1$ and $p_4=p_5=0$, which are quite different from the triggering probabilities.

Indeed, the triggering probability $p_{i}^{\mu, S}$ is related to our algorithm via the action taken $S$. But if we give a closer look at Condition 2, it needs to hold for every possible $S\in \cS$, so it is not relevant to the specific action $S_t$ selected by the specific algorithm at round $t$. Again, for $p_{\min}$, we also claim that it is irrelevant to the specific algorithm, due to its definition in line 216, which considers every $S \in \cS$.

Finally, we would like to emphasize that Condition 2 is standard in the literature of CMAB-T, supported by applications like cascading bandits, online influence maximization [Chen et al. 2017, Perrault et al 2020, Liu et al. 2022, Zuo et al. 2022]. As mentioned in Section 2.1, the modulation of $p_i^{\mu,S}$ is very natural: if arm $i$'s triggering probability is small, then its contribution to the total regret is multiplied by a small $p_i^{\mu,S}$, which compensates the insufficient observation given by the small observation probability, and hence gives improved regret bounds. 


Perrault, Pierre, et al. "Budgeted online influence maximization." International Conference on Machine Learning. PMLR, 2020.




\subsection{Reviewer bHVT: score 7 (Accept), confidence 3}

\textbf{About the related works whose base-arm outcomes are non-linear in contexts.}

We thank the reviewer for pointing out this line of works. We will emphasize our current work focuses on contextual combinatorial bandits with linear base arm outcomes in our final version, and we will include the above works in our related work section. For future work, it will be interesting to investigate whether our TPE technique can be leveraged to extend their semi-bandit setting to that with probabilistically triggered arms, and whether our variance-adaptive algorithm can help to remove the batch-size $K$ in face of base arm outcomes that are non-linear in contexts.

\textbf{Suggestion about putting condition 5 before Theorem 3.}

We thank the reviewer for this comment, and we will move Condition 5 to Section 2.1 as suggested. We will also include the discussions and the implications for the common applications right after Condition 5 (like what we do for Conditions 1-4) in the final version.

\textbf{About the claim of Equation (5) to be the best linear unbiased estimator (BLUE).}

We thank the reviewer for pointing out this inaccurate claim. We double-check our claim and find out that Equation (5) is BLUE under certain conditions, which means Equation (5) is in fact \textit{closely related} to BLUE (but not always BLUE). Concretely, in the literature of linear regression, Equation (5) is BLUE when the regularization term $\gamma=0$, $V_{s,i}$ are the true variance proxy of outcomes $(X_{s,i})_{s<t, i \in \tau_s}$ (or equivalently for the outcome noise $\epsilon_{s,i}=X_{s,i}-{\theta^*}^{\top}\phi_s(i)$) and the context sequence $(\phi_{s}(i))_{s<t, i \in \tau_s}$ follows the fixed design in Equation (5). It is notable that  similar claims are also made by [1] (the last paragraph before Theorem 3), [2] (the first paragraph before Section 5.1) for their respective problem settings.

[1]. Zhou, Dongruo, Quanquan Gu, and Csaba Szepesvari. "Nearly minimax optimal reinforcement learning for linear mixture markov decision processes." *Conference on Learning Theory*. PMLR, 2021.

[2]. Kirschner, Johannes, and Andreas Krause. "Information directed sampling and bandits with heteroscedastic noise." *Conference On Learning Theory*. PMLR, 2018.


\subsection{additional question}

\textbf{Q1.} Thank you for your replies. It would help discussion if the authors specify exactly how Vbar looks like. There seem to be two possibilities. Either way, there seems to be a problem. If the variance uses the data upto t-1 (which is the usual weighted least square estimator based on common weights for all rounds), the relevant function of $b_t$ that normally becomes a supermartingale is no longer shown to be a supermartingale. Alternatively, if the weight for each round to compute the weighted estimator changes each round (which is a bizarre or unusual estimator), that means one has to store all the previous estimators to compute the weight. The strength of usual weighted estimators relies on the fact that the weight is a consistent estimator of the true variance. This unusual estimator cannot have the benefit of this strength. More directly, de la Pena's theorem does not apply in usual way.

We thank the reviewer for the follow-up question. At round $t$, we have $G_t$ and $b_t$ which are determined by historical data before $t$. We first compute $\hat{\theta}_t=G_t^{-1}b_t$ at line 4 of Algorithm 2 (where there is a small typo that we use $b_{t-1}$ instead of the correct $b_t$). Then in line 6 and 7, we compute the UCB value $\bar{\mu}_{t,i}=\langle\hat{\theta}_t,\phi_t(i)\rangle+2\rho(\delta)||\phi_t(i)||_{G_t^{-1}}$ and LCB value $\underline{\mu}_{t,i}=\langle\hat{\theta}_t,\phi_t(i)\rangle-2\rho(\delta)||\phi_t(i)||_{G_t^{-1}}$. Based on UCB and LCB values, $\bar{V}_{t,i}=\max_{\mu\in [\underline{\mu}_{t,i}, \bar{\mu}_{t,i}]}(1-\mu)\mu$ solves an optimization problem that upper bounds the true variance $V_{t,i}$ which lies within $\underline{\mu}_{t,i}$ and $\bar{\mu}_{t,i}$ with high probability. After playing action $S_t$ and triggers $\tau_t$, the  data $(\phi_t(i),X_{t,i})_{i \in \tau_t}$ in round $t$ is reweighted by $\bar{V}_{t,i}^{-1}$ to incrementally update $G_{t+1}=G_{t} + \sum_{i \in \tau_{t}} \bar{V}_{t,i}^{-1}\phi_t(i)\phi_t(i)^{\top}$, $b_{t+1}=b_{t} + \sum_{i \in \tau_{t}} \bar{V}_{t,i}^{-1}\phi_{t}(i)X_{t,i}$. For rounds $s=t+1, ..., T$, the similar process follows as above for the weights $\bar{V}_{s,i}$ and estimator $\hat{\theta}_s$.

For the correctness of our analysis, [Lattimore et al. 2015] also use a similar weighted least square estimator. If we change their notation to match ours, their $G_t=\sum_{s < t}\bar{V}_{s,i_s}^{-1}\phi_s(i_s)\phi_s(i_s)^{\top}$, $b_t=\sum_{s<t}\bar{V}_{s,i_s}^{-1}\phi_s(i_s)X_{s, i_s}$, where $i_s$ is the arm that is chosen by the algorithm at round $s$ (where ours consider arm set $\tau_s$ instead of single arm $i_s$). The definition of $\bar{V}_{t,i}=\max_{\mu\in [\underline{\mu}_{t,i}, \bar{\mu}_{t,i}]}(1-\mu)\mu$, $\bar{\mu}_{t,i}=\langle\hat{\theta}_t,\phi_t(i)\rangle+2\rho(\delta)||\phi_t(i)||_{G_t^{-1}}$ and $\underline{\mu}_{t,i}=\langle\hat{\theta}_t,\phi_t(i)\rangle-2\rho(\delta)||\phi_t(i)||_{G_t^{-1}}$ are exactly the same as our work using the $G_t$ and $b_t$ defined above. For the self-normalized bound, their Theorem 3 is proved with a smaller confidence radius $\rho(\delta)$ (up to factor of $O(\log K )$) compared with our Lemma 2, because only a single arm is played in each round for their work. For the super-martingale concern raised by the reviewer, we do not use any martingale or super-martingale derivation, so we are not exactly sure  which part of the proof the reviewer may find incorrect. We would appreciate it if the reviewer could point out more specific errors in our proof for further discussion.


Tor Lattimore, Koby Crammer, and Csaba Szepesvári. Linear multi-resource allocation with semi-bandit feedback. Advances in Neural Information Processing Systems 28 (2015).

% A1. We thank the reviewer for the follow-up question. We actually use the unusual weighted estimator mentioned by the reviewer (the latter possibility). Similar to [Lattimore et al. 2015], to compute the weighted estimator $\hat{\theta}_t=G_t^{-1}b_t$, we need to use the Gram matrix $G_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i) \phi_{s}(i)^{\top}$ and the b-vector $b_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bar{V}_{s,i}^{-1}\phi_{s}(i)X_{s,i}$.
% For the weights $\bar{V}_{1,i}, \bar{V}_{2,i}, ..., \bar{V}_{t-1,i}$ used above, they are all different across different rounds (but gradually approaching the true variance by the reduction to be introduced shortly), where $\bar{V}_{s,i}=\max_{\mu\in [\underline{\mu}_{s,i}, \bar{\mu}_{s,i}]}(1-\mu)\mu$ solves an optimization problem that upper bounds the true variance $V_{s,i}$ which lies within LCB value $\underline{\mu}_{s,i}$ and UCB value $\bar{\mu}_{s,i}$ with high probability. 
% Note that in above equations, we can incrementally represent $G_{t+1}=G_{t} + \sum_{i \in \tau_{t}} \bar{V}_{t,i}\phi_t(i)\phi_t(i)^{\top}$, $b_{t+1}=b_{t} + \sum_{i \in \tau_{t}} \bar{V}_{t,i}\phi_{t}(i)X_{t,i}$, where the weight $\bar{V}_{t,i}$ is determined by both LCB value $\underline{\mu}_{t,i}$ and UCB value $\bar{\mu}_{t,i}$ which can be computed by $\hat{\theta}_t=G_t^{-1}b_t$ and $G_t$. Therefore, to compute $\hat{\theta}_{t+1}$, only $G_t,b_t$ and data $(\bphi_{t,i},X_{t,i})$ in round $t$ are needed, which does not need all previous estimators.
% % Note that in the above equations, the data in round $1$ contains $(\bphi_1(i), X_{1,i})$ which is weighted by $\bar{V}_{1,i}$ to compute $G_2$ and $b_2$; The data in round $2$ contains  $(\bphi_1(i), X_{1,i}), (\bphi_2(i), X_{2,i})$, but they are not both weighted by $\bar{V}_{2,i}$ to compute $G_3$ and $b_3$, instead, $(\bphi_2(i), X_{2,i})$ is weighted by $\bar{V}_{2,i}$, and $(\bphi_1(i), X_{1,i})$ is weighted by $\bar{V}_{1,i}$, respectively. Therefore, one does not need to store all previous estimators but only needs to maintain $G_t$ and $b_t$ incrementally to compute the $t+1$-round's estimator.


% For the strength of our estimator, it  comes from our unusual variance-aware analysis that leverages the Freedman’s version of the Bernstein’s concentration inequality (Proposition 3 in Line 1510), which differs from the usual Cramer-Chernoff types of concentration used in de la Pena's analysis that does not consider the variance. To handle  the unknown $V_{s,i}$ and the $\bar{V}_{s,i}$ that are different across rounds, we use the reduction on round $t$ to guarantee that our unusual self-normalized bound holds from round $1$ to round $t$. In particular, the reduction at round $t$ relies on the used weight $\bar{V}_{s,i}$ is an upper bound of the true variance $\bar{V}_{s,i}$, which is guaranteed by previous reduction steps on $t-1$. Again, similar types of analysis can be found in [Lattimore et al., 2015], we do not directly follow de la Pena's theorem, but prove a new self-normalized bound with weights that are different across different rounds. For more details, please see the proof of Lemma 7 in Line 1570. 


\subsection{Complaint Letter to the AC}

Dear Area Chairs/Program Chairs/Senior Area Chairs,

We are writing to express our concerns about the review we received from reviewer ob9a. While we appreciate their time and effort in reviewing our paper, it appears that the reviewer may have misunderstood some of the key points we were making, and as a result, their feedback was not as constructive or helpful as we had hoped.

Specifically, the reviewer raises two questions about our paper. First, they express concerns about the way we construct the weighted least-squared estimators and the concentration bound built on them. However, the reviewer did not provide any specific problems or flaws for our proof, but only raise concerns in a very vague way. We believe our method and analysis are correct and can be supported by the sentinel work [Lattimore et al. 2015], which uses a very similar construction of the weighted least-squared estimator. The difference is that we have multiple arms triggered in each round instead of a single arm. To address this, we replaced the original concentration bound of the weighted least-squared estimator with a new one (Lemma 2 in line 341) that has an extra $K^4$ factor in $N$, which finally results in $\log K$ factor in the confidence radius $\rho(\delta)$.

Secondly, the reviewer challenges a very standard smoothness condition. We would like to highlight that this condition is widely used and supported by many applications, such as cascading bandits, online influence maximization bandits, and probabilistic maximum coverage bandits [Chen et al. 2017, Liu et al. 2022, Zuo et al. 2022].
The reviewer also mistakenly confuse the triggering probability and the arm selection probability in the condition. We clarify this in the rebuttal by providing a concrete example. 
Since the reviewer did not have follow-up questions, we believe this concern has been resolved.

We respectfully hope that you take our concerns into consideration when evaluating our paper, and we remain open to further discussions and clarifications. 

Again we want to emphasize that we are the first work to enhance the contextual CMAB framework by considering an arm triggering process (i.e., C$^2$MAB-T). For C$^2$MAB-T, we obtain novel bounds such as batch-size independence and removal of the triggering probability factor from the regret bound. As a by-product, our algorithms and analysis can also be applied to improve the reduced CMAB-T and C$^2$MAB works results, which are of independent interest to the CMAB/MAB community. 

Thank you for your time and consideration. 

Sincerely,

Authors of Paper 1575.



% Dear Area Chairs/Program Chairs/Senior Area Chairs,

% I am writing to express my concern about the review we received from the reviewer ob9a. Unfortunately, it seems that the reviewer misunderstood some of the key points we were making and as a result, their feedback was not constructive or helpful in justifying the quality of our paper.

% Specifically, the reviewer proposes two questions about (1) the way we construct the weighted least-squared estimators and the self-normalized bound built on it, (2) the 1-norm triggering probability modulated smoothness condition for the reward function.

% For (1), we feel that the reviewer's critique was largely unfounded. They only THOUGHT our method/analysis had flaws but did not provide any details or specific problems with our proof to show we are wrong. On the contrary, we can guarantee our correctness based on the sentinel work [Lattimore et al. 2015], which used a very similar construction of the weighted least-squared estimator. The difference is that we have multiple arms triggered in each round instead of a single arm,  where we need to replace the original self-normalized bound with a new one that has an extra $O(\log K)$ factor (Lemma 2 in our paper).

% For (2), the reviewer challenges a very standard smoothness condition that is widely used and supported by many applications, like cascading bandits, online influence maximization bandits, and probabilistic maximum coverage bandits [Chen et al. 2017, Liu et al. 2022, Zuo et al. 2022]. They even mistakenly confuse the triggering probability and the arm selection probability in the condition. Therefore, we are deeply concerned about the reviewer's expertise for the field of Combinatorial Multi-armed Bandits (CMAB), and we are not sure whether they are able to give a fair justification of the contribution for our work.

% Thank you for your attention to this matter. We look forward to hearing back from you soon.

% Sincerely,

% [Your Name]







==> content/1_introduction.tex <==
%%\vspace{-20pt}
\section{Introduction}


\begin{table*}[t]
	\caption{Summary of the main results for \ccmab-T, and additional results for CMAB-T and \ccmab.}	\label{tab:ccmab_res}	
	\centering
	\resizebox{1.96\columnwidth}{!}{
	\centering
	\begin{threeparttable}
	\begin{tabular}{|ccccc|}
 \hline
 % \multicolumn{5}{}{}
 % & \textbf{Summary }\\
 % \hline\hline
		\textbf{\ccmab-T}&\textbf{Algorithm}&\textbf{Condition}& \textbf{Coefficient} & \textbf{Regret Bound}\\
  \hline
    & C$^3$-UCB   \cite{li2016contextual}$^{*}$  & 1-norm & $B_1$   & $O({B_1d\sqrt{KT} \cdot\log T}/{p_{\min}})$\\
        %   \rowcolor{Gray}
        % & C$^2$-UCB-T  (\Cref{alg: C2UCB}) & 1-norm TPM& $B_1$  & $O(B_1d\sqrt{T}\cdot K^{1/2}\cdot\log (KT))$\\
                  \rowcolor{Gray}
       \textbf{(Main Result \ref{thm:c2mab_reg})} & C$^2$-UCB-T  (\Cref{alg: C2UCB}) & 1-norm TPM& $B_1$  & $O(B_1d\sqrt{KT}\cdot\log T)$\\
                     \rowcolor{Gray}
\textbf{(Main Result \ref{thm:ccmab_reg_VM})}& VAC$^2$-UCB (\Cref{alg:va_cucb})  & VM & $B_v$$^{\dagger}$& $O(B_v d\sqrt{T} \cdot \log T/\sqrt{p_{\min}})$\\
 \rowcolor{Gray}
	\textbf{(Main Result \ref{thm:ccmab_reg_TPVM_lambda})}& 	VAC$^2$-UCB 
 (\Cref{alg:va_cucb})  & TPVM  & $B_v$, $\lambda\ge1$$^{\ddagger}$ & $O(B_v d\sqrt{T} \cdot \log T)$\\
          % \rowcolor{Gray}
	% & 	VAC$^2$-UCB-K 
 % (Appendix XXX)  & TPVM, known variance bound   & $B_v$, $\lambda\ge1$ & $O(B_v d\sqrt{T} \cdot \log T)$\\
    \hline\hline
    \textbf{CMAB-T}&\textbf{Algorithm}&\textbf{Condition}& \textbf{Coefficient} & \textbf{Regret Bound}\\
  \hline
 % \textbf{Summary }&\textbf{of }&\textbf{additional }& \textbf{results} & \textbf{}\\
 % \hline\hline	
	 % &	CUCB~\cite{chen2016combinatorial}&  1-norm & $B_1$  & $O(B_1\sqrt{mKT}\cdot (\log T)^{1/2} /p_{\min})$ \\
  %  &	CUCB~\cite{wang2017improving}&  1-norm TPM & $B_1$  & $O(B_1\sqrt{mKT}\cdot (\log T)^{1/2})$ \\
  %  &BCUCB-T \cite{liu2022batch} & TPVM& $B_v$, $\lambda\ge2$ & $O(B_v \sqrt{m(\log K)T}\cdot(\log T)^{1/2})$\\
		&BCUCB-T \cite{liu2022batch} & TPVM& $B_v$, $\lambda\ge 1$  & $O(B_v \sqrt{m(\log K)T}\cdot\log T)$\\
  \rowcolor{Gray}
  % &BCUCB-T (Our new results)  & TPVM& $B_v$, $\lambda\ge 1$   & $O(B_v \sqrt{mT}\cdot(\log K )^{1/2}\cdot(\log T)^{1/2}\cdot p_{\max}^{(\lambda-1)/2})$$^{\ddagger}$ \\
   \textbf{(Additional Result 1)} &BCUCB-T (Our new analysis)  & TPVM& $B_v$, $\lambda\ge 1$   & $O(B_v \sqrt{m(\log K )T}\cdot(\log T)^{1/2})^{**}$ \\
		\hline\hline
    \textbf{\ccmab} &\textbf{Algorithm}&\textbf{Condition}& \textbf{Coefficient} & \textbf{Regret Bound}\\
    \hline
   &	C$^2$UCB~\cite{qin2014contextual}&  2-norm & $B_2$$^{\S}$  & $O(B_2d\sqrt{T}\log T)$ \\
  &	C$^2$UCB~\cite{takemura2021near}&  1-norm & $B_1$  & $O(B_1d\sqrt{KT}\log T)$ \\
       \rowcolor{Gray}
   \textbf{(Additional Result 2)}&	VAC$^2$-UCB~(\Cref{alg:va_cucb})& VM & $B_v$  & $O(B_vd\sqrt{T}\log T)$ \\
	\hline
	\end{tabular}
	  \begin{tablenotes}[para, online,flushleft]
	\footnotesize%\smallskip
 \item[]\hspace*{-\fontdimen2\font}$^{*}$ This work is specified for contextual combinatorial cascading bandits, without formally defining the  arm triggering process.
 \item[]\hspace*{-\fontdimen2\font}$^\dagger$ Generally,  
 coefficient $B_v=O(B_1\sqrt{K})$ and the existing regret bound is improved when $B_v=o(B_1\sqrt{K})$
 \item[]\hspace*{-\fontdimen2\font}$^{\ddagger}$ $\lambda$ is a coefficient in TPVM condition: when $\lambda$ is larger, the condition is stronger with smaller regret but can include less applications.
 \item[]\hspace*{-\fontdimen2\font}$^{**}$ We also show improved distribution-dependent regret bound in \Cref{apdx_sec:NC_C2MAB};
 \item[]\hspace*{-\fontdimen2\font}$^{\S}$ Almost all applications satisfy $B_2=\Theta(B_1\sqrt{K})$.
 
	% \item[]\hspace*{-\fontdimen2\font}$^*$ Requires exact offline oracle instead of $(\alpha, \beta)$-approximate oracle;
	% 	\item[]\hspace*{-\fontdimen2\font}$^{\dagger}$ This work gives sufficient smoothness condition with factor $\gamma_g$ and translates to $B_v=3\sqrt{2}\gamma_g$ in our setting;
	% 	\item[]\hspace*{-\fontdimen2\font}$^{*}$ Using our new and simplified  analysis;
	% \item[]\hspace*{-\fontdimen2\font}$^\dagger$ Generally,  
 % coefficient $B_v=O(B_1\sqrt{K})$ and the existing regret bound is improved when $B_v=o(B_1\sqrt{K})$; Coefficient $\lambda$ trades off the regret and satisfiability: when $\lambda$ is larger, the regret is better but TPVM condition can include less applications. 
 % 	\item[]\hspace*{-\fontdimen2\font}$^{\S}$ This work is specified for contextual combinatorial cascading bandits, without formally defining the  arm triggering process.
	% 	\item[]\hspace*{-\fontdimen2\font}$^{\ddagger}$ We also show improved distribution-dependent regret bound in Appendix XXX;
	\end{tablenotes}
			\end{threeparttable}
	}
\end{table*}

\ts{CMAB short intro}

The stochastic multi-armed bandit (MAB) problem is a classical sequential decision-making problem that has been widely studied~\cite{robbins1952some,auer2002finite,bubeck2012regret}. As an extension of MAB, combinatorial multi-armed bandits (CMAB) have drawn attention due to fruitful applications in online advertising, network optimization, and healthcare systems \cite{gai2012combinatorial, kveton2015combinatorial, chen2013combinatorial, chen2016combinatorial, wang2017improving, merlis2019batch}.
CMAB is a sequential decision-making game between a learning agent and an environment. In each round, the agent chooses a combinatorial action that triggers a set of base arms (i.e., a super-arm) to be pulled simultaneously, and the outcomes of these pulled base arms are observed as feedback (typically known as semi-bandit feedback). The goal of the agent is to minimize the expected \textit{regret}, which is the difference in expectation for the overall rewards between always playing the best action (i.e., the action with the highest expected reward) and playing according to the agent's own policy. 
% For CMAB, the agent not only needs to handle the exploration-exploitation tradeoff: whether the agent should explore arms in search for a better action, or should the agent stick to the best action observed so far to gain rewards; but also n eeds to deal with the exponential explosion of all possible actions. 

\ts{Intro of \ccmab~and drawbacks of \ccmab}

Motivated by large-scale applications with a huge number of items (base arms), there exists a prominent line of work that advances the CMAB model: the combinatorial contextual bandits (or \ccmab~for short) ~\cite{qin2014contextual,li2016contextual,takemura2021near}. Specifically, \ccmab~incorporates contextual information and adds the simple yet effective linear structure assumption to allow scalability, which provides regret bounds that are independent of the number of base arms $m$. Despite \ccmab's success in leveraging contextual information for better scalability, existing works fail to formulate the general arm triggering process, which is essential to model a wider range of applications, e.g., cascading bandits (CB) and influence maximization (IM), and more importantly, they do not provide satisfying results for settings with probabilistically triggered arms. For example, \citet{qin2014contextual,takemura2021near} only consider the deterministic semi-bandit feedback for \ccmab. \citet{li2016contextual,wen2017online} implicitly consider the arm triggering process for specific CB or IM applications but only gives sub-optimal results with unsatisfying factors (e.g., $1/p_{\min}, K$ that could be as large as the number of base arms), owing to loose analysis, weak conditions, or inefficient algorithms that explore the unknown parameters too conservatively. 

To handle the above issues, we enhance the \ccmab~framework by considering an arm triggering process.
Specifically, we propose the general framework of contextual combinatorial bandits with probabilistically triggered arms (or \ccmab-T for short). At the base arm level, \ccmab-T uses a time-varying feature map $\bphi_t$ to model the contextual information at each round $t$, and the mean outcome of each arm $i \in [m]$ is a linear product of the feature vector $\bphi_t(i) \in \R^d$ and an unknown vector $\theta^* \in \R^d$ (where $d\ll m$ to handle large-scale applications). At the (combinatorial) action level, inspired by the non-contextual CMAB with probabilistically triggered arms (or CMAB-T) works~\cite{chen2016general,wang2017improving,liu2022batch}, 
% \wei{\cite{liu2022batch} should be referring to the NeurIPS'2022 paper now.}
we formally define an arm-triggering process to cover more general feedback models such as semi-bandit, cascading, and probabilistic feedback.
We also inherit smoothness conditions for the non-linear reward function to cover different application scenarios, such as CB, IM, and online probabilistic maximum coverage (PMC) problems~\cite{chen2016combinatorial, wang2017improving}. With this formulation, \ccmab-T retains \ccmab's scalability while also enjoying CMAB-T's rich reward functions and general feedback models.


% existing works only either considers semi-bandit feedback which neglects the probabilistic nature of the feedback~\cite{qin2014contextual,takemura2021near} for specific CB or IM applications, or implicitly consider the arm-triggering  considers special 

% For example, existing works either 
% we observe that both the \ccmab~model and its algorithm/analysis have drawbacks that can be significantly improved: (1) For the modeling part, \ccmab~either cannot handle rich types of reward functions~\cite{li2016contextual,wen2017online}, or only adopts the deterministic semi-bandit feedback which neglects the probabilistic nature of the feedback~\cite{qin2014contextual,takemura2021near}; (2) For the algorithm/analysis part, the existing state-of-the-art algorithm still encounters additional factors (i.e., $p_{\min}, K$ that are could be as large as $m$) due to loose analysis, weak conditions, or inefficient algorithms that explore the unknown parameters too conservatively.  In this paper, we aim to conduct a systematic study to enhance the modeling power,  and provide improved results using novel algorithms/analysis under proper conditions.

% \ts{Two lines of work: \ccmab~and CMAB-T}


% In CMAB literature, there exist two prominent lines of work that advance the CMAB model: the combinatorial contextual bandits (or \ccmab~for short) and the combinatorial multi-armed bandits with probabilistically triggered arms (or CMAB-T for short). Specifically, \ccmab incorporates the context information and adds the simple yet effective base arm level linear structure assumptions to handle large-scale applications, which eventually provides regret bounds that are independent of the number of base arms; CMAB-T models the probabilistic nature of the feedback and allows arms to be triggered probabilistically, which can cover a broader range of applications scenarios, e.g., cascading bandits~\cite{combes2015combinatorial} (CB) and online influence maximization (OIM) bandit~\cite{wen2017online} problems. Despite 
%  the huge efforts that has been put into each line separately, it still remains open to studying the unification of both lines, which can hopefully inspire algorithms that achieve the best of both lines' properties and results.

\textbf{Contributions.} 
%
% \textbf{General Framework.} 
% To improve the model part, we propose the general framework of contextual combinatorial bandits with probabilistically triggered arms (or \ccmab-T for short). At the base arm level, \ccmab-T uses a time-varying feature map $\bphi_t$ to model the contextual information at each round $t$, and the mean of the outcomes of each arm $i \in [m]$ is a linear product of the feature vector $\bphi_t(i) \in \R^d$ and the unknown vector $\theta^* \in \R^d$ (where $d\ll m$ to handle large-scale applications). At the (combinatorial) action level, inspired by CMAB-T work, we formally define the arm-triggering process to cover general feedback models including semi-bandit, cascading, and probabilistic feedback.
% We also inherit proper smoothness conditions for the non-linear reward function to cover different application scenarios, such as cascading bandits (CB), online influence maximization (IM), and online probabilistic maximum coverage (PMC) problems. With this formulation, \ccmab-T enjoys \ccmab's scalability for large-scale applications, and the CMAB-T's rich reward functions and probabilistic feedback models.
% It is noted that there are prior works studying special cases that fit into our framework (e.g., contextual CB~\cite{li2016contextual} and contextual OIM~\cite{wen2017online}), but we are the first to study the unified framework and more importantly, we give new algorithms/analysis for improved results.
Our main results are shown in \Cref{tab:ccmab_res}. 

First, we study \ccmab-T under the triggering probability modulated (TPM) smoothness condition, a condition introduced by~\citet{wang2017improving} to remove a factor of $1/p_{\min}$ in the pioneer CMAB-T work~\cite{chen2016combinatorial}. This result follows a similar vein by devising C$^2$-UCB-T algorithm and proving a $\tilde{O}(d\sqrt{KT})$ regret, which removes a $1/p_{\min}$ factor for prior contextual CB applications~\cite{li2016contextual} (Main Result 1 in \Cref{tab:ccmab_res}). The key technical challenge is that the triggering group (TG) analysis~\cite{wang2017improving} for CMAB-T cannot handle the triggering probability determined by time-varying contexts. To tackle this issue, we devise a new technique, called the triggering probability equivalence (TPE), which links the triggering probabilities with the random triggering event under expectation. 
In this way, we no longer need to bound the regret caused by possibly triggered arms, but only need to bound the regret caused by actually triggered arms. 
As a result, we can then directly apply the simple non-triggering \ccmab~analysis to obtain the regret bound for \ccmab-T. 
In addition, our TPE can reproduce the results for CMAB-T in a similar way.

Second, we study the \ccmab-T under the variance modulated (VM) smoothness condition~\cite{liu2022batch}, in light of the recent variance-adaptive algorithms to remove the batch size dependence $O(\sqrt{K})$ for CMAB-T~\cite{merlis2019batch,liu2022batch,vial2022minimax}. We propose a new variance-adaptive algorithm VAC$^2$-UCB and prove a batch-size independent regret $\tilde{O}(d\sqrt{T/p_{\min}})$ under VM condition (Main Result 2 in \Cref{tab:ccmab_res}). The main technical difficulty is to deal with the unknown variance. Inspired by \citet{lattimore2015linear}, we use the UCB/LCB value to construct an optimistic variance and on top of that, we prove a new concentration bound to incorporate the triggered arms and optimistic variance to get the desirable results. 

Third, we investigate the stronger triggering probability and variance modulated (TPVM) condition~\cite{liu2022batch} in order to remove the additional $1/\sqrt{p_{\min}}$ factor. 
The key challenge is that we cannot directly use TPE to link the \textit{true} triggering probability with the random trigger event as before, since the TPVM condition only yields a mismatched triggering probability associated with the optimistic variance used in the algorithm. Our solution is to bound this additional mismatch by lower-order terms based on mild conditions on the triggering probability, which achieves the $\tilde{O}(d\sqrt{T})$ regret bounds (Main Result 3 in \Cref{tab:ccmab_res}). 
% The key challenge is that in order to use the variance information, the TPVM condition only produces a mismatched triggering probability rather than the true probability, so we cannot trivially apply the TPE trick as before. Our solution is to either consider mild conditions on the triggering probability to bound the amount of this mismatch and prove that this match, which eventually achieves the $\tilde{O}(d\sqrt{T})$ regret bounds (Main Result 3 in \Cref{tab:ccmab_res}). 

As a valuable by-product, our TPE analysis and VAC$^2$-UCB algorithm can be applied to non-contextual CMAB-T and \ccmab, improving the existing results by a factor $\sqrt{\log T}$ (Additional Result 1 in \Cref{tab:ccmab_res}) and $\sqrt{K}$ (Additional Result 2 in \Cref{tab:ccmab_res}), respectively.
Our empirical results on both synthetic and real data demonstrate that the VAC$^2$-UCB algorithm outperforms the state-of-art variance-agnostic and variance-aware bandit algorithms in the linear cascading bandit application that satisfies the TPVM condition.

% In addition to the general \ccmab-T setting, we find that the TPE trick and the variance-adaptive algorithm can help to improve the degenerate CMAB-T and \ccmab~settings, respectively. For CMAB-T, our TPE trick reproduces the results under 1-norm TPM condition and improves the results by a factor $\sqrt{\log T}$, compared with the more involved TG type of analysis. For \ccmab, our variance-adaptive algorithm achieves the first batch-size independent regrets for applications satisfying VM conditions.

% \adam{Do you want to add a short paragraph about numeric results here?}

\textbf{Related Work.}
% The multi-armed bandit (MAB) problem is first studied by \citet{robbins1952some} and then extended by many studies (cf. \cite{bubeck2012regret, slivkins2019introduction, lattimore2020bandit}).
% \jinhang{can be removed}
The stochastic CMAB model has received significant attention.  The literature was initiated by \cite{gai2012combinatorial}.  Since, its regret has been improved by \citet{kveton2015tight}, \citet{combes2015combinatorial}, \citet{chen2016combinatorial}. There exist two prominent lines of work in the literature related to our study: contextual CMAB and CMAB with probabilistically triggered arms (\ccmab~and CMAB-T). 
%At a high level, our work can be viewed as the first framework that unifies the \ccmab~and CMAB-T, which enjoys the best of both lines' properties and results. There are many studies considering specific applications rather than a general \ccmab-T framework, including contextual CB~\cite{zong2016cascading,li2016contextual,vial2022minimax}, contextual IM~\cite{wen2017online}, etc. These applications can fit into our framework by proving that they satisfy the TPM, VM, or TPVM conditions, and achieve improved results regarding $K, p_{\min}$ factors. We defer the detailed technical comparison to \Cref{sec:c2mab}, \Cref{sec:va_c2mab}, and \Cref{sec:app}. \citet{zuo2022online} studies the online competitive IM and also uses \ccmab-T to denote their contextual setting. Their context is at the action level, and only affects the reward function (or regret) but not the base arms' estimation, which is different and much simpler than our setting. 

For \ccmab~works, \citet{qin2014contextual} is the first study, which proposes C$^2$UCB algorithm that considers reward functions under 2-norm $B_2$ smoothness condition. Then \citet{takemura2021near} replaces the 2-norm smoothness condition with a new 1-norm $B_1$ smoothness condition, and proves a $O(B_1d\sqrt{KT}\log T)$ regret bound. 
%
In this work, we extend the \ccmab~with triggering arms to cover more application scenarios (e.g., contextual CB and contextual IM). Moreover, we further consider the stronger VM condition and propose a new variance-adaptive algorithm that can achieve a $\sqrt{K}$ factor improvement in the regret upper bound for applications like PMC.
%
%at least give matching regret bounds, and further achieve a $\sqrt{K}$ factor improvement under VM condition with $B_v=o(B_1\sqrt{K})$ (for applications like PMC).

For CMAB-T works, \citet{chen2016combinatorial} is the first work that considers the arm triggering process to cover CB and IM applications. The authors propose the CUCB algorithm, and give an $O(B_1\sqrt{mKT\log T}/p_{\min})$ regret bound under 1-norm $B_1$ smoothness condition. Then \citet{wang2017improving} proposes the stronger 1-norm triggering probability modulated (TPM) $B_1$ smoothness condition, and use the triggering group (TG) analysis to remove a $1/p_{\min}$ factor in the previous regret. Recently, \citet{liu2022batch} incorporates the variance information, and proposes the variance-adaptive algorithm BCUCB-T, which also uses the TG analysis and further reduces the regret's dependency on batch-size from $O(K)$ to $O(\log K)$ under the new variance and triggering probability modulated (TPVM) condition. The smoothness conditions considered in this work are mostly inspired by the above works, but directly following their algorithm and TG analysis fail to obtain any meaningful result for our \ccmab-T setting. 
% paralyzes \adam{not sure what you mean with "paralyzes" here} the direct use of CMAB-T's TG analysis. 
Conversely, our new TPE analysis can be applied to CMAB-T, reproducing CMAB-T's result under the 1-norm TPM condition, and improving a factor of $(\sqrt{\log T})$ under the TPVM condition. 

There are also many studies considering specific applications under the \ccmab-T framework (by unifying \ccmab~and CMAB-T), including contextual CB~\cite{li2016contextual,vial2022minimax}, contextual IM~\cite{wen2017online}, etc. One can see that these applications fit into our framework by verifying that they satisfy the TPM, VM, or TPVM conditions; thus achieving improved results regarding $K, p_{\min}$ factors.  We defer a detailed theoretical and empirical comparison to \Cref{sec:c2mab,sec:va_c2mab,sec:app}. \citet{zuo2022online} study the online competitive IM and also uses \ccmab-T to denote their contextual setting. However, their meaning of ``contexts" is the action of the competitor, which acts at the action level and only affects the reward function (or regret) but not the base arms' estimation.
This is very different from our setting, where contexts act at the base arm level and hence one cannot directly apply their results.
%different and much simpler than our setting. 


% For CMAB-T, our work improves (a) the general framework in \cite{chen2016combinatorial, wang2017improving}, (b) the combinatorial cascading bandit \cite{kveton2015combinatorial}, (c) the online multi-layered network exploration~\cite{liu2021multi} problem, (d) the online influence maximization bandits \cite{wang2017improving, perrault2020budgeted}, by reducing or removing the batch-size dependent factor $K$ in the regret bounds with our new TPVM condition and/or our refined analysis. We defer the detailed technical comparison to \cref{sec:TPVM} and \cref{sec:app}. 
% For the algorithm, most CMAB-T studies use Combinatorial Upper Confidence Bound (CUCB) based on Chernoff concentration bounds \cite{wang2017improving}, our BCUCB-T algorithm is different and uses the Bernstein concentration bound \cite{audibert2009exploration,merlis2019batch}
% that considers variance of the arms. 

% For non-triggering CMAB, \cite{gai2012combinatorial} is the first study on stochastic CMAB, and its regret has been improved by \citet{kveton2015tight}, \citet{combes2015combinatorial}, \citet{chen2016combinatorial}, but they still have $O(K)$ factor in their regrets. When arms are mutually independent, \citet{combes2015combinatorial} build a tighter ellipsoidal confidence region for exploration, and devise the Efficient Sampling for Combinatorial Bandit policy (ESCB), which reduces the dependence on $O(K)$ to $O(\log^2 K)$ at the cost of high computational complexity (since combinatorial optimization over the ellipsoidal region is NP-hard in general~\cite{atamturk2017maximizing}). Later on, the computational complexity is improved by AESCB~\cite{cuvelier2021statistically} in the linear CMAB problem. 
% Recently, \citet{merlis2019batch} focus on the Probabilistic Maximum Coverage (PMC) bandit problem and propose the BC-UCB algorithm with the Gini-smoothness condition to achieve a similar improvement as ESCB/AESCB, but without the independent arm assumption. 
% Our work is largely inspired by their work, however, our study generalizes theirs to the CMAB-T setting which can handle much broader application scenarios beyond the non-triggering CMAB
% 	(more detailed comparison is given in Section~\ref{sec:gini_cond}). 
% In addition,  we provide a refined analysis that can save a $O(\log K)$ factor for BC-UCB (or ESCB/AESCB) algorithm. 
% Compared with other ESCB-type algorithms for independent arms, as far as we know, our SESCB algorithm are the first to completely remove the dependence of $K$ in the leading regrets, owing to our non-triggering version of the TPVM condition. 
% The detailed comparisons are summarized in \cref{tab:triggering} and \cref{tab:non-triggering}.

% { The usage of variance-aware algorithms to give improved regret bounds can be dated back to \cite{audibert2009exploration}. Recently, there is a surge of interest to apply the variance-aware principle in bandit~\cite{merlis2019batch,vial2022minimax} and reinforcement learning (RL) settings~\cite{zhou2021nearly,zhang2021improved}. It is notable that Vial et al.~\cite{vial2022minimax} share a similar variance-aware principle as ours but focus on the distribution-independent regret bounds for the cascading bandits~\cite{vial2022minimax}. Our work is more general and achieves the matching regret bound when translating to the distribution-independent regret bound. Compared with RL works, our paper studies a different setting as we do not consider the state transitions.}

% From the application's point of view, this paper covers the applications of PMC
% bandit~\cite{merlis2019batch}, combinatorial cascading bandits~\cite{kveton2015combinatorial,li2016contextual}, network exploration~\cite{liu2021multi}, and online influence maximization~\cite{wen2017online,wang2017improving, li2020online}. 
% Our proposed algorithms can significantly reduce the regret bounds of them, e.g., from $O(K)$ to $O(\log^2 K)$ for OIM
% where $K$ can be hundreds of thousands in large social networks.

% To-dos:
% \begin{itemize}
%     % \item Two directions: either from variance-adaptive C2MAB to C2MAB-T, or from C2MAB-T but under two different assumptions.
%     \item Title \& scope of the paper:  Contextual Combinatorial Bandits with Probablistically Triggering Arms (alternative)
%     \item Table
%     \item Intro + related work: difference with Jinhang's C2MAB-T; 
%     \item Setting: independence
%     \item Analysis: (1) directly-triggering equality (DT), (2) triggering-probability triggering-event (TPTE) equality, (3) triggering probability equivalence (TPE)
%     \item two different contextual models: one $\theta$ and $L$ features, or one context and $L$ $\theta$s. Improving $\sqrt{K}$.
%     \item Lower bound for $B_v$.
%     \item Experiments
%     \item Future study: C-KL-UCB, fixed point


% \end{itemize}

==> content/2_preliminary.tex <==
%% \vspace{-5pt}
% Key words: variance control, triggering arms, discrete TPM gini-smoothness, two proofs (one is infinity many events, the other is reverse amortization).


\section{Problem Setting}\label{sec: problem setting}
% % \subsection{CMAB-T Problem Formulation}
% We first revisit the context-free combinatorial multi-armed bandit problem (CMAB-T) with probabilistic triggering arms~\cite{chen2016general, wang2017improving, liu2022batch}, and then generalize it to its contextual counterpart, the contextual CMAB-T (or \ccmab-T for short).

% \textbf{Context-free CMAB-T.} Following the settings of~\cite{chen2016combinatorial,wang2017improving,liu2022batch}, the CMAB-T problem can be described by a tuple $([m], \cS, \cD, D_{\text{trig}}, R)$,
% 	where $[m]=\{1,2,...,m\}$ is the set of base arms; 
% 	$\cS$ is the set of eligible actions and $S \in \cS$ is an action;\footnote{$\cS$ as a general action space. When $\cS$ is a collection of subsets of $[m]$, we often 
% 	refer to $S\in \cS$ as a super arm.}
% 	$\cD$ is the set of possible distributions over base arms' outcomes whose support is bounded within $[0,1]^m$;
% $ D_{\text{trig}}$ is the probabilistic triggering function to characterize the arm triggering process (and observations), and $R$ is the reward function. 

% In CMAB-T, a learning game is played between a learning agent (or player) and the unknown environment in a sequential manner.
% First, the environment chooses a distribution $D \in \cD$ unknown to the agent before the game starts.
% Then, at round $t=1,2,...,T$, the agent selects an action $S_t \in \cS$, and the environment draws from the unknown distribution $D$ a random outcome $\bX_t=(X_{t,1},...X_{t,m})\in [0,1]^m$, with mean $\bmu=\E_{X_t\sim D}[\bX_t]$. 
% % Let $D_{\text{trig}}(S,\bX)$ be a distribution over all possible subsets of $[m]$, i.e. its support is $2^{[m]}$.
% After the action $S_t$ is played on the outcome $\bX_t$, base arms in a random set $\tau_t \sim D_{\text{trig}}(S_t, \bX_t)$ are triggered, 
% 	meaning that the outcomes of arms in $\tau_t$, i.e. $(X_t)_{t\in \tau_t}$ are revealed as the feedback to the agent, and are involved in determining the reward of action $S_t$. 
% At the end of the round $t$, the agent will receive a non-negative reward $R(S_t, \bX_t, \tau_t)$, determined by $S_t,
% \bX_t$ and $\tau_t$, and similar to~\cite{wang2017improving}, the expected reward is assumed to be a $r(S;\bmu)\triangleq \E[R(S,\bX,\tau)]$ is a function of 
% the unknown mean vector $\bmu$, where the expectation is taken over the randomness of $\bX\sim D$ and $\tau \sim D_{\text{trig}}(S,\bX)$.
% In this context, we denote $r(S;\bmu)\triangleq \E[R(S,\bX,\tau)]$ and it suffices to learn the unknown mean vector instead of the joint distribution $D$, based on the past observation.

% CMAB-T significantly enhances the modeling power of CMAB~\cite{chen2013combinatorial, kveton2015tight} modeling the probabilistic nature of the feedback (v.s. the deterministic semi-bandit feedback), which can cover many applications such as combinatorial cascading bandits, multi-layered network exploration,  and online influence maximization~\cite{wang2017improving,liu2022batch}.

% \textbf{Contextual CMAB-T.}
\ts{Overall nations and the \ccmab-T tuple.}

We study contextual combinatorial bandits with probabilistically triggered arms (\ccmab-T). We use $[n]$ to represent set $\{1,...,n\}$. We use boldface lowercase letters and boldface CAPITALIZED letters for column vectors and matrices, respectively. $\norm{\bx}_p$ denotes the $\ell_p$ norm of vector $\bx$. For any symmetric positive semi-definite (PSD) matrix $\bM$ (i.e., $\bx^{\top} \bM \bx \ge 0, \forall \bx$), $\norm{\bx}_{\bM}=\sqrt{\bx^{\top} \bM \bx}$ denotes the matrix norm of $\bx$ regarding matrix $\bM$.

We specify a \ccmab-T problem instance using a tuple $([m], \cS, \Phi, \Theta, D_{\text{trig}}, R)$, where $[m]=\{1,2,...,m\}$ is the set of base arms (or arms); 
$\cS$ is the set of eligible actions where $S \in \cS$ is an action;\footnote{$\cS$ is a general action space. When $\cS$ is a collection of subsets of $[m]$, we often 
refer to $S\in \cS$ as a super arm.} 
$\Phi$ is the set of possible feature maps where any feature map $\bphi \in \Phi$ is a function $[m]\rightarrow \R^d$ that maps an arm to a $d$-dimensional feature vector (and w.l.o.g. we normalize $\norm{\bphi(i)}_2 \le 1$); $\Theta\subseteq R^d$ is the parameter space; 
$ D_{\text{trig}}$ is the probabilistic triggering function to characterize the arm triggering process (and feedback), and $R$ is the reward function.

\ts{The learning protocol.}

In \ccmab-T, a learning game is played between a learning agent (or player) and the unknown environment in a sequential manner.
Before the game starts, the environment chooses a parameter $\btheta^* \in \Theta$ unknown to the agent (and w.l.o.g. we also assume $\norm{\theta^*}_2 \le 1$). At the beginning of round $t$, the environment reveals feature vectors $(\bphi_t(1), ..., \bphi_t(m))$ for each arm, where $\bphi_t \in \Phi$ is the feature map known to the agent.  Given $\bphi_t$, the agent selects an action $S_t \in \cS$, and the environment draws Bernoulli outcomes $\bX_t=(X_{t,1},...X_{t,m})\in \{0,1\}^m$ for base arms\footnote{ We assume $X_{t,i}$ are Bernoulli for the ease of exposition, yet our setting can handle any distribution with bounded $X_{t,i}\in[0,1]$.}, with mean $\E[\bX_{t,i} | \cH_t]=\inner{\btheta^*, \bphi_{t}(i)}$ for each base arm $i$. 
%
Here $\cH_t$ denotes the history before the agent chooses $S_t$ and will be specified shortly after. Note that the outcome $\bX_t$ is assumed to be conditional independent across arms given history $\cH_t$, similar to previous works~\cite{qin2014contextual,li2016contextual,vial2022minimax}. For convenience, we use $\bmu_t\triangleq(\inner{\btheta^*, \bphi_{t}(i)})_{i \in [m]}$ to denote the mean vector and $\cM\triangleq\{\inner{\btheta, \bphi(i)}_{i \in [m]}: \bphi \in \Phi, \btheta \in \Theta\}$ to denote all possible mean vectors generated by $\Phi$ and $\Theta$. 
% \siwei{Should we say that $\inner{\btheta^*, \bphi_{t}(i)} \in [0,1]$?}.

After the action $S_t$ is played on the outcome $\bX_t$, base arms in a random set $\tau_t \sim D_{\text{trig}}(S_t, \bX_t)$ are triggered, 
meaning that the outcomes of arms in $\tau_t$, i.e. $(X_{t,i})_{i\in \tau_t}$ are revealed as the feedback to the agent, and are involved in determining the reward of action $S_t$. 
At the end of round $t$, the agent will receive a non-negative reward $R(S_t, \bX_t, \tau_t)$, determined by $S_t,
\bX_t$ and $\tau_t$, and similar to~\cite{wang2017improving}, the expected reward is assumed to be $r(S_t;\bmu_t)\triangleq \E[R(S_t,\bX_t,\tau_t)]$, a function of 
the unknown mean vector $\bmu_t$, where the expectation is taken over the randomness of $\bX_t$ and $\tau_t \sim D_{\text{trig}}(S_t,\bX_t)$. To this end, we can give the formal definition of the history $\cH_t=(\bphi_s, S_s, \tau_s, (X_{s,i})_{i\in \tau_s})_{s<t} \bigcup \bphi_t$, which contains all information before round $t$, as well as the contextual information $\bphi_t$ at round $t$.

\ts{The goal and the evaluation metrics (approximate regret).}

The goal of CMAB-T is to accumulate as much reward as possible over $T$ rounds by learning the underlying parameter $\theta^*$.
The performance of an online learning algorithm $A$ is measured by its \textit{regret}, defined as the difference of the expected cumulative reward between always playing the best action $S^*_t \triangleq \argmax_{S \in \cS}r(S;\bmu_t)$ in each round $t$ and playing actions chosen by algorithm $A$.
%Let $S^*=\argmax_{S \in \cS}r(S;\bmu)$ be the optimal action. 
For many reward functions, it is NP-hard to compute the exact $S^*_t$ even when $\bmu_t$ is known, so similar to~\cite{wang2017improving}, we assume that the algorithm $A$ has access to an offline $(\alpha, \beta)$-approximation oracle, which for mean vector $\bmu$ outputs an action $S$ such that $\Pr\left[r(S;\bmu)\ge \alpha \cdot r(S^*;\bmu)\right] \ge \beta$. 
% \jinhang{$\beta$}
The $T$-round $(\alpha, \beta)$-approximate regret is defined as
% \resizebox{1.0\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
\begin{equation}\textstyle
    \text{Reg}(T)=\E\left[\sum_{t=1}^T \left(\alpha\beta  \cdot r(S^*_t;\bmu_t)-r(S_t;\bmu_t)\right)\right],
\end{equation}
% \end{minipage}}
where the expectation is taken over the randomness of outcomes $\bX_1, ..., \bX_T$, the triggered sets $\tau_1, ..., \tau_T$, as well as the randomness of algorithm $A$ itself.

% \wei{I feel that the remarks do not need to be put in italic style. Only theorems and lemmas are put into italic to emphasize them. But either is fine.}

\begin{remark}[\textbf{Difference with CMAB-T}]\label{rmk:cmab-T_diff}
\ccmab-T strictly generalizes CMAB-T by allowing a probably time-varying feature map $\bphi_t$. Specifically, let $\btheta^*=(\mu_1, ..., \mu_m)$ and fix $\bphi_t(i)=\be_i$ where $\be_i \in \R^{m}$ is the one-hot vector with $1$ at the $i$-th entry and $0$ elsewhere, one can easily reproduce the CMAB-T setting in~\cite{wang2017improving}.
\end{remark}

\begin{remark}[\textbf{Difference with C$^2$MAB}]
\ccmab-T enhances the modeling power of prior \ccmab~\cite{qin2014contextual,takemura2021near} by capturing the probabilistic nature of the feedback (v.s. the deterministic semi-bandit feedback). This enables a wider range of applications such as combinatorial CB, multi-layered network exploration, and online IM~\cite{wang2017improving,liu2022batch}.
\end{remark}

\subsection{Key Quantities and Conditions}
\ts{Introduce two key quantities.}

In the \ccmab-T model, there are several quantities and assumptions that are crucial to the subsequent study.
We define \textit{{triggering probability}} $p_i^{\bmu, D_{\text{trig}}, S}$ as the probability that base arm $i$ is 
	triggered when the action is $S$, the mean vector is $\bmu$, and the probabilistic triggering function is $D_{\text{trig}}$.
Since $D_{\text{trig}}$ is always fixed in a given application context, we ignore it in the notation for simplicity, and use $p_{i}^{\bmu,S}$ henceforth.
Triggering probabilities  $p_i^{\bmu,S}$'s are crucial for the triggering probability modulated bounded smoothness conditions to be defined below.
We define $\tilde{S}$ to be the set of arms that can be triggered by $S$,  i.e.,$\{i \in [m]: p_i^{\bmu,S} > 0, \text{ for any }\bmu \in \cM\}$, the  \textit{{batch size}} $K$ as the maximum number of arms that can be triggered, i.e., $K=\max_{S \in \cS}|\tilde{S}|$, and $p_{\min}=\min_{i \in [m], \bmu \in \cM, S \in \cS, p_i^{\bmu,S}>0}{p_i^{\bmu,S}}$.

% Our main contribution of this paper is to remove or reduce the regret dependency on batch size $K$, where $K$ could be quite large, e.g., $K$ can be hundreds of thousands in a large social network.

\ts{Explain necessary conditions: monotonicity, TPM, TPVM smoothness.}

Owing to the nonlinearity and the combinatorial structure of the reward, it is essential to give some conditions for the reward function in order to achieve any meaningful regret bounds~\cite{chen2013combinatorial, chen2016combinatorial, wang2017improving,merlis2019batch,liu2022batch}. 
For \ccmab-T, we consider the following conditions.

% For the reward function $r(S;\bmu): \cS \times [0,1]^m \rightarrow \R$, we are interested in functions that are continuous for $\bmu \in [0,1]^m$ and differentiable for $\bmu \in (0,1)^m$, for any $S \in \cS$.
% For CMAB-T framework, \citet{wang2017improving} introduce two standard conditions for the reward function to guarantee the regret bounds, which we also use in this work, as we shall introduce in the following.

\begin{condition}[\textbf{Monotonicity}]\label{cond:mono}
We say that a \ccmab-T problem instance satisfies monotonicity condition, if for any action $S \in \cS$, any mean vectors $\bmu,\bmu' \in [0,1]^m$ such that $\mu_i \le \mu'_i $ for all $i \in [m]$, we have $ r(S;\bmu) \le r(S;\bmu') $. 
\end{condition}

\begin{condition}[\textbf{1-norm TPM Bounded Smoothness}, \cite{wang2017improving}]\label{cond:TPM}
% We say that a CMAB-T instance satisfies TPM $B_1$-bounded smoothness condition, if for any action $S \in \cS$, any distribution $D,D'$ with mean vector $\bmu \in (0,1)^m$, we have $\frac{\partial r(S;\bmu)}{\partial \mu_i } \frac{1}{p_{i}^{D,S}}\le B_1 $ for $i \in \tilde{S}$ and $\frac{\partial r(S;\bmu)}{\partial \mu_i }=0$ for $i \in [m] \backslash \tilde{S}$. 
We say that a \ccmab-T problem instance satisfies the triggering probability modulated (TPM) $B_1$-bounded smoothness condition, if for any action $S \in \cS$, any mean vectors $\bmu, \bmu' \in [0,1]^m$, we have $|r(S;\bmu')-r(S;\bmu)|\le B_1\sum_{i \in [m]}p_{i}^{\bmu,S}|\mu_i-\mu'_i|$.
%\siwei{seems no formal definition of this $p_{i}^{D,S}$?} 
\end{condition}

\begin{condition}[\textbf{VM Bounded Smoothness}, \cite{liu2022batch}]\label{cond:VM}
We say that a \ccmab-T problem instance satisfies the variance modulated (VM) $(B_v, B_1)$-bounded smoothness condition, if for any action $S \in \cS$, mean vector $\bmu, \bmu' \in (0,1)^m$, for any $\boldzeta, \boldeta \in [-1,1]^m$ s.t. $\bmu'=\bmu+\boldzeta+\boldeta$, we have
% $|r(S;\bmu')-r(S;\bmu)|\le B_v\norm{\left(\frac{(p_i^{\bmu,S})^{\lambda/2}}{\sqrt{(1-\mu_i)\mu_i}}\zeta_i\right)_{i\in[m]}}_{2} + B_1\norm{ (p_i^{\bmu,S}\eta_i)_{i \in [m]}}_1.$
$|r(S;\bmu')-r(S;\bmu)|\le B_v\sqrt{\sum_{i\in \tilde{S}}\frac{\zeta_i^2 }{(1-\mu_i)\mu_i}} + B_1 \sum_{i\in\tilde{S}}\abs{\eta_i}$. 
\end{condition}

\begin{condition}[\textbf{TPVM Bounded Smoothness}, \cite{liu2022batch}]\label{cond:TPVMm}
We say that a \ccmab-T problem instance satisfies the triggering probability and variance modulated (TPVM) $(B_v, B_1,\lambda)$-bounded smoothness condition, if for any action $S \in \cS$, mean vector $\bmu, \bmu' \in (0,1)^m$, for any $\boldzeta, \boldeta \in [-1,1]^m$ s.t. $\bmu'=\bmu+\boldzeta+\boldeta$, we have
% $|r(S;\bmu')-r(S;\bmu)|\le B_v\norm{\left(\frac{(p_i^{\bmu,S})^{\lambda/2}}{\sqrt{(1-\mu_i)\mu_i}}\zeta_i\right)_{i\in[m]}}_{2} + B_1\norm{ (p_i^{\bmu,S}\eta_i)_{i \in [m]}}_1.$
$|r(S;\bmu')-r(S;\bmu)|\le B_v\sqrt{\sum_{i\in [m]}(p_i^{\bmu,S})^{\lambda}\frac{\zeta_i^2 }{(1-\mu_i)\mu_i}} + B_1 \sum_{i\in[m]}p_i^{\bmu,S}\abs{\eta_i}$. 
\end{condition}

% \wei{It is unclear from the context whether these conditions are new or defined before. Perhaps adding reference to each condition.}

% \siwei{Should we put Condition 4 before Condition 3, as the order of your main results?}

\ts{Intuitions and remarks of the conditions}

Condition~\ref{cond:mono} indicates the reward is monotonically increasing when the parameter $\bmu$ increases. Condition~\ref{cond:TPM}, \ref{cond:VM} and \ref{cond:TPVMm} all bound the reward smoothness/sensitivity.%, i.e., the amount of the reward change caused by the parameter change from $\bmu$ to $\bmu'$.

% As mentioned in~\cite{liu2022batch}, Condition~\ref{cond:TPVMm} is stronger than Condition~\ref{cond:TPM} and Condition~\ref{cond:VM}, as the former degenerates to the other two conditions by setting $\boldzeta=\boldsymbol{0}$ and $p_i^{\bmu,S}=1 \text{ for } i \in \tilde{S}$, respectively. Conversely, by applying the Cauchy-Schwartz inequality, one can verify that if a reward function is TPM $B_1$-bounded smooth, then it is 
% TPVM $(B_1\sqrt{K}/2, B_1, \lambda)$-bounded smooth for any $\lambda\le 2$ (or similarly VM $(B_1\sqrt{K}/2, B_1)$-bounded smooth). \siwei{Why not mention VM condition here?}


%\begin{remark}
For Condition~\ref{cond:TPM}, the key feature is that the parameter change in each base arm $i$ is modulated by the triggering probability $p_i^{\bmu,S}$. Intuitively, for base arm $i$ that is unlikely to be triggered/observed (small $p_i^{\bmu, S}$), Condition~\ref{cond:TPM} ensures that a large change in $\mu_i$ (due to insufficient observation) only causes a small change (multiplied by $p_i^{\bmu,S}$) in reward, which helps to save a $p_{\min}$ factor for non-contextual CMAB-T.
%\end{remark}

%\begin{remark}
For Condition~\ref{cond:VM}, intuitively if we ignore the denominator $(1-\mu_i)\mu_i$ of the leading $B_v$ term, the reward change would be $O(B_v \sqrt{K}\Delta )$ when the amount of parameter change $|\mu'_i-\mu_i|=\Delta$ for each arm $i$. This introduces a $O(\sqrt{K})$ factor reduction in the reward change and translates to a $O(K)$ improvement in the regret, compared with $O(B_1 K\Delta)$ reward change when applying the non-triggering version of Condition~\ref{cond:TPM} (i.e., $p_i^{\bmu,S}=1$ if $i \in \tilde{S}$ and $p_i^{\bmu,S}=0$ otherwise). However, for real applications, $B_1=\Theta(B_1 \sqrt{K})$ which cancels the $O(\sqrt{K})$ improvement.
To reduce $B_v$ coefficient, the leading $B_v$ term is modulated by the inverse of the variance $V_i=(1-\mu_i)\mu_i$, and thus allow applications to achieve a $B_v$ coefficient independent of $K$ (or at least $B_v=o(B_1\sqrt{K}$), leading to significant savings in the regret bound for applications like PMC~\cite{liu2022batch}. The relation between Condition \ref{cond:TPM} and \ref{cond:VM} is generally not comparable, but compared with Condition~\ref{cond:TPM}'s non-triggering counterpart (i.e., 1-norm condition), Condition~\ref{cond:VM} is stronger. 
%\end{remark}

%\begin{remark}
%\label{rmk:TPVM}
Finally, for Condition~\ref{cond:TPVMm}, it combines both the triggering-probability modulation from Condition~\ref{cond:TPM} and the variance modulation from Condition~\ref{cond:VM}. The exponent $\lambda$ of $p_i^{\bmu,S}$ gives additional flexibility to trade-off between the strength of the condition and the regret, i.e., with a larger $\lambda$, one can obtain a smaller regret bound, while
with a smaller $\lambda$, the condition is easier to satisfy to include more applications. In general, Condition~\ref{cond:TPVMm} is stronger than Condition~\ref{cond:TPM} and Condition~\ref{cond:VM}, as the former degenerates to the other two conditions by setting $\boldzeta=\boldsymbol{0}$ and the fact that $p_i^{\bmu,S}\le1 \text{ for } i \in \tilde{S}$ and $p_i^{\bmu,S}=0$ otherwise, respectively. Conversely, by applying the Cauchy-Schwartz inequality, one can verify that if a reward function is TPM $B_1$-bounded smooth, then it is TPVM $(B_1\sqrt{K}/2, B_1, \lambda)$-bounded smooth for any $\lambda\le 2$ or similarly VM $(B_1\sqrt{K}/2, B_1)$-bounded smooth, respectively.
% More importantly, the $B_v$ term is further modulated by the inverse of the variance $V_i=(1-\mu_i)\mu_i$, and thus reduces their $B_v$ coefficient from $B_1\sqrt{K}/2$ to a coefficient independent of $K$, leading to significant savings in the regret bound of CMAB-T~\cite{liu2022batch}. 
% Another subtle yet critical point is that Condition~\ref{cond:TPVMm} strengthens the prior directional TPVM condition proposed by \citet{liu2022batch} (assuming $\boldeta, \boldzeta \in [0,1]^m$), which are necessary to guarantee desirable regret bounds for \ccmab-T as in \Cref{sec:va_c2mab}.
%\end{remark}

% \begin{remark}
%     For Condition~\ref{cond:VM}, it is a weaker version of Condition~\ref{cond:TPVMm}, by letting $p_i^{\bmu,S}=1$ for $i \in \tilde{S}$ and $0$ otherwise. 
%     % Condition~\ref{cond:VM} is stronger than Condition~\ref{cond:TPM}'s non-triggering counterpart (i.e., 1-norm condition).
% \end{remark}


In light of the above conditions that significantly advance the non-contextual CMAB-T, the goal of subsequent sections is to design algorithms and conduct analysis to derive the (improved) results for the contextual setting. And later in \Cref{sec:app}, we 
demonstrate how these conditions are applied to applications, such as CB and online IM, to achieve both theoretical and empirical improvements. Due to the space limit, the detailed proofs are included in the Appendix.
% \siwei{Maybe we can state some applications of these conditions here, and say "see details in Section 5".}

==> content/3_c2mab_TPM.tex <==
\section{Algorithm and Regret Analysis for \ccmab-T under the TPM Condition}\label{sec:c2mab}
\begin{algorithm}[t]
	\caption{C$^2$-UCB-T: \textbf{C}ontextual \textbf{C}ombinatorial \textbf{U}pper \textbf{C}onfidence \textbf{B}ound Algorithm for \ccmab-\textbf{T}}\label{alg: C2UCB}
			\resizebox{.96\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \STATE {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\gamma$, failure probability $\delta=1/T$, offline oracle ORACLE. 
	   % \OUTPUT Budget allocation $\bk$.
	   \STATE \textbf{Initialize:} Gram matrix $\bG_{1}=\gamma\boldsymbol{I}$, vector $\bb_{1}=\boldsymbol{0}$. 
	   \FOR{$t=1, ...,T$ }
	   \STATE $\hat{\btheta}_{t}=\bG_{t}^{-1}\bb_{t}$. \label{line:c2mab_estimate}%\COMMENT{Compute the least-square estimator.}
	   %\STATE Construct the confidence set, one for decision, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t}}^2 \le \beta\}$.
	   \FOR{$i \in [m]$}
	    \STATE $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + \rho(\delta)\norm{\bphi_{t}(i)}_{\bG_{t}^{-1}}$.\label{line:c2_ucb}
	    %\COMMENT{UCB value for base arm $i$.}
	    % \STATE $\bar{\mu}_{t,i} =\min\{\bar{\mu}_{t,i},1\} $
	    \ENDFOR
	   %\STATE $G_t=\gamma \boldsymbol{I} + \sum_{\tau < t}\bphi(i)\bphi(i)^{\top}$.
	   %$\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1, i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.
	   %\STATE Set UCB value $\bar{\mu}_{t,i}=\min \{\hat{\mu}_{t-1, i}+\rho_{t, i},1\}$.
	   %\STATE $S_t=\text{ORACLE}(C_t^{\theta}, \phi_t)$.  \qquad\qquad\qquad\qquad\qquad//$S_t=\arg\max_{S \in \cS, \bnu \in C_t^{\theta}} r(S;\bnu, \phi_t)$.
	   \STATE $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. %\COMMENT{Computational oracle using UCBs.}
	   \STATE Play $S_t$ and observe triggering arm set $\tau_t$ and observation set $(X_{t,i})_{i\in \tau_{t}}$.
	   % \FOR{$ i \in \tau_t$ } 
	   %\STATE $v_{t,i}=\max_{\bnu \in C^{v}_{t}}\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})$.
	   \STATE $\bG_{t+1}=\bG_{t}+\sum_{i \in \tau_t} \bphi_{t}(i)\bphi_{t}(i)^{\top}$.\label{line:c2_G}
	   \STATE $\bb_{t+1}=\bb_{t}+\sum_{i \in \tau_t} \bphi_{t}(i) X_{t,i}$.\label{line:c2_b} %\COMMENT{Update statistics using the triggered arms' observation.}
	   %\STATE Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
	   % \STATE For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
	   % \label{line:trigger_upd}
	   %\ENDFOR
	    	   \ENDFOR
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}
Our proposed algorithm C$^2$-UCB-T (\Cref{alg: C2UCB}) is a generalization of the C$^3$-UCB algorithm originally designed for contextual combinatorial cascading bandits~\cite{li2016contextual}. Our main contribution is to show an improved regret bound by a factor of $1/p_{\min}$ under the 1-norm TPM condition.

Recall that we define the data about the history as $\cH_t=(\bphi_s, S_s, \tau_s, (X_{s,i})_{i\in \tau_s})_{s<t} \bigcup \bphi_t$.
Different from the CUCB algorithm~\cite{wang2017improving} that directly estimates the mean $\bmu_{t,i}$ for each arm, \Cref{alg: C2UCB} estimates the underlying parameter $\btheta^*$ via a ridge regression problem over the history data $\cH_t$.
More specifically, we estimate $\btheta^*$ by solving the following $\ell_2$-regularized least-square problem with regularization parameter $\gamma >0$:
\begin{equation}
 \resizebox{.91\linewidth}{!}{$
            \displaystyle
    \hat{\btheta}_t = \argmin_{\btheta \in \Theta} \sum_{s<t}\sum_{i \in \tau_{s}}(\inner{\btheta, \bphi_{s}(i)}-X_{s,i})^2 + \gamma \norm{\btheta}_2^2.$}
\end{equation}
The closed form solution is precisely the $\hat{\theta}_t$ calculated in line~\ref{line:c2mab_estimate}, where the Gram matrix $\bG_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bphi_{s}(i) \bphi_{s}(i)^{\top}$ and the b-vector $\bb_t=\sum_{s< t}\sum_{i \in \tau_{s}}\bphi_{s}(i)X_{s,i}$ are computed in line~\ref{line:c2_G} and \ref{line:c2_b}. We claim that $\hat{\theta}_t$ is a good estimator of $\theta^*$ by bounding their difference via the following lemma, which is also used in \cite{qin2014contextual,li2016contextual}.

% \adam{Weird to call this "fact"..maybe Proposition?}
\begin{proposition}[Theorem 2, \cite{abbasi2011improved}]\label{lem:c2mab_good_est}
% Let $\rho(\delta)=\sqrt{\log\left(\frac{\det(\bG_{t})}{\gamma^d \cdot \delta^2}\right)}+\sqrt{\gamma}$, then with probability at least $1-\delta$, for all round $t\ge 0$, the estimate $\hat{\btheta}_t$ satisfies,
Let $\rho(\delta)=\sqrt{\log\left(\frac{(\gamma+KT/d)^d}{\gamma^d \cdot \delta^2}\right)}+\sqrt{\gamma}$, then with probability at least $1-\delta$, for all $t\in [T]$, $\norm{\hat{\btheta}_t-\btheta^*}_{\bG_{t}} \le \rho(\delta).$
% \begin{align}\label{eq:c2mab_est}
%     \norm{\hat{\btheta}_t-\btheta^*}_{\bG_{t}} \le \rho(\delta).
% \end{align}
\end{proposition}
% \siwei{The notation $\beta$ is used in the $(\alpha,\beta)$-oracle. Can we change a notation?}
% The proof of \cref{lem:c2mab_good_est} is based on the self-normalized theory and by considering $\norm{\btheta^*}_2\le 1$, $\norm{\bphi_t(i)}_2\le 1$, and $\det(\bG_{t+1})\le (\gamma+KT/d)^d$ in Theorem 2 of \citet{abbasi2011improved}. 
% \siwei{I'd like to write it as a Fact, since it is the same as some results in prior works. Also, we do not need to say anything about its proof, except that it is very important.}

Building on this, we construct an optimistic estimation of each arm's mean $\bar{\mu}_{t,i}$ in line~\ref{line:c2_ucb}, where $\rho(\delta)$ is in \Cref{lem:c2mab_good_est}, $\inner{\bphi_t(i), \hat{\btheta}_t}$ and $\rho(\delta)\norm{\bphi_{t}(i)}_{\bG_{t}^{-1}}$ are the empirical mean and confidence interval towards the direction $\bphi_t(i)$, respectively. As a convention, we clip $\bar{\mu}_{t,i}$ into $[0,1]$ if $\bar{\mu}_{t,i}> 1$ or $\bar{\mu}_{t,i}< 0$.
%that guides the exploration: the larger the confidence interval, the more bonus the agent gets to explore arm $i$, which reduces the uncertainty towards the direction $\bphi_t(i)$. 
% Similar to~\Cref{rmk:cmab-T_diff}, when $\bphi_t(i)=\be_i$, the confidence interval reproduces that of CUCB~\cite{wang2017improving}, where $\bG_t$ becomes a diagonal matrix $\text{diag}(T_{t,1},..., T_{t,m})$, and the confidence interval is proportional to $\sqrt{\log t/T_{t,i}}$, where $T_{t,i}$ is the number of times arm $i$ is triggered before round $t$. \siwei{Really? You have the $\gamma$ here, and hence it may not be exactly the same. Event if we let $\gamma = 0$, it also seems that the confidence bound is not the same as that one in CUCB, e.g., another factor of $\sqrt{d}$. Maybe we can remove this part...}

Thanks to \Cref{lem:c2mab_good_est}, we have the following lemma for the desired amount of the base arm level optimism,
\begin{restatable}{lemma}{lemccmabOptimism}
\label{lem:c2mab_optimism}
    With probability at least $1-\delta$, we have $\mu_{t,i}\le \bar{\mu}_{t,i}\le \mu_{t,i} + 2\rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}}$ for all $i \in [m], t \in [T]$. 
\end{restatable}
\begin{proof}
    See \Cref{apdx_sec:lemmas_thm1}.
\end{proof}
% \siwei{What do you mean by "when Lemma 1 holds"... Lemma 1 always holds, you can only say w.p. at least $1-\delta$, or when some event holds...}
% \begin{lemma}\label{lem:c2mab_optimism}
%     When \Cref{eq:c2mab_est} holds for $t-1$, we have $\mu_{t,i}\le \bar{\mu}_{t,i}\le \mu_{t,i} + 2\rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}}$ for all $i \in [m]$. 
% \end{lemma}

After computing the UCB values $\bar{\bmu}_t$, the agent selects action $S_t$ via the offline oracle with $\bar{\bmu}_t$ as input.
%
Then base arms in $\tau_t$ are triggered, and the agent receives observation set $(X_{t,i})_{i\in \tau_{t}}$ as feedback to improve future decisions.
%
% Compared with~\cite{li2016contextual}, we generalize the cascading feedback to the general arm triggering process, whose outcomes are then used for future decision rounds. \siwei{Do not understand the last sentence...}


% \subsection{Analysis and Discussion}
\begin{theorem}\label{thm:c2mab_reg}
     For a \ccmab-T instance that satisfies monotonicity (Condition~\ref{cond:mono}) and TPM smoothness (Condition~\ref{cond:TPM}) with coefficient $B_1$, C$^2$-UCB-T (\Cref{alg: C2UCB}) with an $(\alpha,\beta)$-approximation oracle achieves an $(\alpha,\beta)$-approximate regret bounded by $ O\left(B_1(\sqrt{d\log (KT/\gamma)}+\sqrt{\gamma})\sqrt{KTd\log(KT/\gamma)}\right).$
\end{theorem}
% \siwei{Why there is no $\delta$ in this theorem?}

% \begin{remark}
\textbf{Discussion.} Looking at \Cref{thm:c2mab_reg}, we achieve an $O(B_1d\sqrt{KT}\log T)$ regret bound when $d \ll K \le m \ll T$, which is independent of the number of arms $m$ and the minimum triggering probability $p_{\min}$. Consider the combinatorial cascading bandits~\cite{li2016contextual} satisfying $B_1=1$ (see \Cref{sec:app}), our result improves the~\citet{li2016contextual} by a factor of $1/p_{\min}$. Consider the linear reward function~\cite{takemura2021near} without triggering arms (i.e., $p_i^{\bmu,S}=1$ for $i \in S$,  and $0$ otherwise), one can easily verify $B_1=1$ and our regret matches the lower bound ${\Omega}(d\sqrt{KT})$~\citet{takemura2021near} up to logarithmic factors.
% \end{remark}

% 1. regret bound independent of $m$ 2. compare with degenerate CMAB-T
% 3. lower bound 

\textbf{Analysis.}
%\begin{proof}[Proof Sketch]
Here we explain how to prove a regret bound that removes the $1/p_{\min}$ factor under the 1-norm TPM condition. The main challenge is that the mean vector $\bmu_t$ and the triggering probability $p_i^{\bmu_t,S}$ are dependent on \textit{time-varying} contexts $\bphi_t(i)$, so it is impossible to derive any meaningful concentration inequality or regret bound based on $T_{t,i}$, which is the number of times that arm $i$ is triggered, and has been used by the \textit{triggering group (TG)} technique~\cite{wang2017improving} to remove $1/p_{\min}$. To deal with this problem, we bypass the quantity $T_{t,i}$ and use the \textit{triggering-probability equivalence (TPE)} technique that equalizes $p_i^{\bmu_t, S}$ with $\E_t[\I\{i \in \tau_t\}]$, which in turn replaces the expected regret produced by all possible arms with the expected regret produced by $i \in \tau_t$ to avoid $p_{\min}$. To sketch our proof idea, we assume the oracle is deterministic with $\beta=1$ (the randomness of the oracle and $\beta<1$ are handled in \Cref{apdx_sec:TPM}), and let filtration $\cF_{t-1}$ be the history data $\cH_t$ (defined in \Cref{sec: problem setting}). 
% \siwei{Why not just define $\cH_t$ as $\cF_{t-1}$?} 
Denote $\E_t[\cdot]=\E[\cdot\mid \cF_{t-1}]$, the $t$-round regret $\E_t[\alpha\cdot r(S^*_t;\bmu_t)-r(S_t;\bmu_t)]{\le}\E_t[r(S_t;\bar{\bmu}_t)-r(S_t;\bmu_t)]$, based on  Condition~\ref{cond:mono}, \Cref{lem:c2mab_optimism} and definition of $S_t$. Then
% \noindent
% \resizebox{\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
\begin{talign}\label{eq:TPE}
% &\E_t[\alpha\cdot r(S^*_t;\bmu_t)-r(S_t;\bmu_t)]\notag\\
%    &\overset{(a)}{\le}\E_t[\alpha\cdot r(S^*_t;\bar{\bmu}_t)-r(S_t;\bmu_t)]\overset{(b)}{\le} \E_t[r(S_t;\bar{\bmu}_t)-r(S_t;\bmu_t)]\notag\\
    &\E_t[r(S_t;\bar{\bmu}_t)-r(S_t;\bmu_t)]\overset{(a)}{\le}\E_t\left[\sum_{i \in \tilde{S}_t}B_1p_i^{\bmu_t,S_t}(\bar{\mu}_{t,i}-\mu_{t,i})\right]\notag\\
    &\overset{(b)}{=}\E\left[\sum_{i \in \tilde{S}_t}B_1\E_{\tau_t}[\I\{i \in \tau_t\}](\bar{\mu}_{t,i}-\mu_{t,i})\mid \cF_{t-1}\right]\notag\\
    &\overset{(c)}{=}\E_t\left[\sum_{i \in \tilde{S}_t}\I\{i \in \tau_t\}B_1(\bar{\mu}_{t,i}-\mu_{t,i})\right]\notag\\
    &\overset{(d)}{=}\E_t\left[\sum_{i \in \tau_t}B_1(\bar{\mu}_{t,i}-\mu_{t,i})\right],
\end{talign}
% \end{minipage}
% }

where (a) is by Condition~\ref{cond:TPM}, (b) is because $\bar{\mu}_{t,i}, \mu_{t,i}, S_t$ are $\cF_{t-1}$ measurable so that the only randomness is from triggering set $\tau_t$ and we can substitute $p_i^{\bmu_t, S_t}$ with event $\I\{i \in \tau_t\}$ under expectation, $(c)$ is by absorbing the expectation over $\tau_t$ to $\E_t$, and $(d)$ is a change of notation. 
After applying the TPE, we only need to bound the regret produced by $i \in \tau_t$. Hence %without considering the arm-triggering. Hence
% i.e., Reg$(T)\le\E\left[\sum_{t \in [T]}\E_t\left[\sum_{i \in \tau_t}B_1(\bar{\mu}_{t,i}-\mu_{t,i})\right]\right].$ Then its RHS $\le 2B_1\rho(\delta)\E\left[\sum_{t \in [T]}\sum_{i \in \tau_t}\norm{\bphi_t(i)}_{\bG_{t}^{-1}}\right]\le 2B_1\rho(\delta) \E\left[\sqrt{KT\sum_{t \in [T]}\sum_{i \in \tau_t}\norm{\bphi_t(i)}^2_{\bG_{t}^{-1}}}\right]\le {O}(B_1d\sqrt{KT}\log T)$,
% where the first inequality is by~\Cref{lem:c2mab_optimism}, the second inequality by Cauchy Schwarz inequality over both $i$ and $t$, and the last is by the ellipsoidal potential lemma \Cref{apdx_lem:ccmab_potential} in the Appendix.
\begin{talign}\label{eq:c2mab_reg}
&\text{Reg}(T){\le} \E\left[\sum_{t \in [T]}\E_t\left[\sum_{i \in \tau_t}B_1(\bar{\mu}_{t,i}-\mu_{t,i})\right]\right]\notag\\
&\overset{(a)}{\le} \E\left[\sum_{t \in [T]}\E_t\left[\sum_{i \in \tau_t}2B_1 \rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}}\right]\right]\notag\\
&\overset{(b)}{\le} 2B_1\rho(\delta) \E\left[\sqrt{KT\sum_{t \in [T]}\sum_{i \in \tau_t}\norm{\bphi_t(i)}^2_{\bG_{t}^{-1}}}\right]\notag\\
&\overset{(c)}{\le}{O}(B_1d\sqrt{KT}\log T).
\end{talign}
where (a) follows from~\Cref{lem:c2mab_optimism}, (b) is by Cauchy Schwarz inequality over both $i$ and $t$, and (c) is by the ellipsoidal potential lemma (\Cref{apdx_lem:ccmab_potential}) in the Appendix.


% \begin{align}\label{eq:c2mab_reg}
% &\text{Reg}(T)\overset{(a)}{=}\E\left[\sum_{t \in [T]}\E_t[\alpha\cdot r(S^*_t;\bmu_t)-r(S_t;\bmu_t)]\right]\notag\\
% &\overset{(b)}{\le} \E\left[\sum_{t \in [T]}\E_t\left[\sum_{i \in \tau_t}B_1(\bar{\mu}_{t,i}-\mu_{t,i})\right]\right]\notag\\
% &\overset{(c)}{\le} \E\left[\sum_{t \in [T]}\E_t\left[\sum_{i \in \tau_t}B_1 \rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}}\right]\right]\notag\\
% &\overset{(d)}{=}  B_1\rho(\delta)\E\left[\sum_{t \in [T]}\sum_{i \in \tau_t}\norm{\bphi_t(i)}_{\bG_{t}^{-1}}\right]\notag\\
% &\overset{(e)}{\le}  B_1\rho(\delta) \E\left[\sqrt{KT\sum_{t \in [T]}\sum_{i \in \tau_t}\norm{\bphi_t(i)}^2_{\bG_{t}^{-1}}}\right] \notag\\
% &\overset{(f)}{\le}{O}(B_1d\sqrt{KT}\log T).
% \end{align}
% where (a) follows from the definition and the tower rule, (b) by the TPE~\Cref{eq:TPE}, (c) by~\Cref{lem:c2mab_optimism}, (d) by tower rule, (e) by Cauchy Schwarz inequality, and (f) by the ellipsoidal potential lemma \Cref{apdx_lem:ccmab_potential_new} in the Appendix.
\begin{remark}
In addition to the general \ccmab-T setting, the TPE technique can also replace the more involved TG technique~\cite{wang2017improving} for CMAB-T. Such replacement can save an unnecessary union bound over the group index, which in turn reproduce Theorem 1 of \citet{wang2017improving} under Condition~\ref{cond:TPM}, and improve Theorem 1 of \citet{liu2022batch} under Condition~\ref{cond:TPVMm} by a factor of $O(\sqrt{\log T})$, see \Cref{apdx_sec:NC_C2MAB} for details.
\end{remark}



==> content/4_c2mab_TPVM.tex <==
\section{Variance-Adaptive Algorithm and Analysis for \ccmab-T under VM/TPVM Condition}\label{sec:va_c2mab}

\begin{algorithm}[t]
	\caption{VAC$^2$-UCB: \textbf{V}ariance-\textbf{A}daptive \textbf{C}ontextual \textbf{C}ombinatorial \textbf{U}pper \textbf{C}onfidence \textbf{B}ound Algorithm}\label{alg:va_cucb}
			\resizebox{.96\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \STATE {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\gamma$, failure probability $\delta=1/T$, offline oracle ORACLE.
	   % \OUTPUT Budget allocation $\bk$.
	   \STATE \textbf{Initialize:} Gram matrix $\bG_{1}=\gamma\boldsymbol{I}$, regressand $\bb_{1}=\boldsymbol{0}$. 
	   \FOR{$t=1, ...,T$ }
	   \STATE $\hat{\btheta}_{t}=\bG_{t}^{-1}\bb_{t}$. %\COMMENT{Compute empirical estimator.}
	   %\STATE Construct two confidence sets, one for decision and one for the variance, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t}}^2 \le \beta\}$, $C^{v}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t}}^2 \le 4\beta\}$.
	   \FOR{$i \in [m]$}
	   \STATE $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + 2\rho(\delta)\norm{\bphi_{t}(i)}_{\bG_{t}^{-1}}$\label{line:va_ucb}  %\COMMENT{UCB value for arm $i$.}
	   % \STATE $\bar{\mu}_{t,i}=\min \{\bar{\mu}_{t,i},1\}$.
	   \STATE $\ubar{\mu}_{t,i}=\inner{\bphi_t(i), \hat{\btheta}_t} - 2\rho(\delta)\norm{\bphi_{t}(i)}_{\bG_{t}^{-1}}$\label{line:va_lcb} %\COMMENT{LCB value for arm $i$.}
	   % \STATE $\ubar{\mu}_{t,i}=\max\{\ubar{\mu}_{t,i},0\}$.
	   %\STATE Compute the optimistic variance by solving $\max_{\bnu \in C^{v}_t}{\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})}$ 
    \STATE Set the optimistic variance $\bar{V}_{t,i}$ as \Cref{eq:var_upper}. \label{line:var_opt} %\COMMENT{Optimistic variance for true $V_{t,i}$.}
% \STATE Let $ \tilde{\bnu}_{t}(i), \tilde{\mu}_{t,i}$ are parameters that achieve $v_{t,i}$.
	   \ENDFOR
	   \STATE $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. %\COMMENT{Computational oracle using UCBs.}
	   \STATE Play $S_t$ and observe triggering arm set $\tau_t$ and observation set $(X_{t,i})_{i\in \tau_{t}}$.
	   % \FOR{$ i \in \tau_t$ }\COMMENT{Update statistics.}\label{line:update_G}
	   \STATE $\bG_{t+1}=\bG_{t}+\sum_{i \in \tau_t} \bar{V}_{t,i}^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.\label{line:update_G}
	   \STATE $\bb_{t+1}=\bb_{t}+\sum_{i \in \tau_{t}} \bar{V}_{t,i}^{-1}\bphi_{t}(i) X_{t,i}$.\label{line:update_b}%\COMMENT{Update statistics.}
	   \ENDFOR
	    	  % \ENDFOR
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}

In this section, we propose a new variance-adaptive algorithm VAC$^2$-UCB (\Cref{alg:va_cucb}) to further remove the $O(\sqrt{K})$ factor and achieve $\tilde{O}(B_v d\sqrt{T})$ regret bound for applications satisfying stronger VM/TPVM conditions.

% \siwei{Mention algorithm name here?}

Different from \Cref{alg: C2UCB}, VAC$^2$-UCB leverages the second-order statistics (i.e., variance) to speed up the learning process. 
To get some intuition, we first assume the variance $V_{s,i}=\text{Var}[X_{s,i}]$ for each base arm $i$ at round $s$ is known in advance. 
%
In this case, VAC$^2$-UCB adopts the \textit{weighted ridge-regression} to learn the parameter $\btheta^*$:
\begin{equation}\label{eq:var_opt}
 \resizebox{.91\linewidth}{!}{$
            \displaystyle
    \hat{\btheta}_t = \argmin_{\btheta \in \Theta} \sum_{s<t}\sum_{i \in \tau_s}(\inner{\btheta, \bphi_s(i)}-X_{s,i})^2/V_{s,i} + \gamma \norm{\btheta}_2^2,
    $}
\end{equation}
where the first term is ``weighted" by the true variance $V_{s,i}$. The closed-form solution of the above estimator is $\hat{\btheta}_{t}=\bG_{t}^{-1}\bb_{t}$ where the Gram matrix $\bG_t=\sum_{s< t}\sum_{i \in \tau_{s}}V_{s,i}^{-1}\bphi_{s}(i) \bphi_{s}(i)^{\top}$ and the b-vector $\bb_t=\sum_{s< t}\sum_{i \in \tau_{s}}V_{s,i}^{-1}\bphi_{s}(i)X_{s,i}$, which enjoys the similar form (but uses different weights $\bar{V}_{s,i}$) of  line~\ref{line:update_G} and line~\ref{line:update_b}.

The intuition of using the inverse of $V_{s,i}$ to re-weight the observation is that: the smaller the variance, the more accurate the observation $(\bphi_t(i), X_{t,i})$ is, and thus more important for the agent to learn unknown $\btheta^*$.
%
%Hence 
%
%The intuition of using the variance in this way is from the exploitation perspective: the smaller the variance, the more accurate the observation $(\bphi_t(i), X_{t,i})$ is, and thus more important for the agent to learn unknown $\btheta^*$. So we use the inverse of $V_{s,i}$ to re-weight the observation.
In fact, the above estimator $\hat{\btheta}_t$ is \textit{closely related} to the best linear unbiased estimator (BLUE)~\cite{henderson1975best}. Concretely, in the literature of linear regression, Equation (5) is the lowest variance estimator of $\btheta^*$ among all unbiased linear estimators, when the regularization term $\gamma=0$, $V_{s,i}$ are the true variance proxy of outcomes $(X_{s,i})_{s<t, i \in \tau_s}$ and the context sequence $(\bphi_{s}(i))_{s<t, i \in \tau_s}$ follows the fixed design in Equation (5). 


For our \ccmab-T setting, one new challenge arises since the variance $V_{s,i}=\mu_{s,i}(1-\mu_{s,i})$ is not known a priori. Inspired by \cite{lattimore2015linear,zhou2021nearly}, we construct an optimistic estimation $\bar{V}_{s,i}$ to replace the true variance $V_{s,i}$ in \Cref{eq:var_opt}. Indeed, we construct $\bar{V}_{t,i}$ by solving the optimal value for the problem $\max_{\mu\in [\ubar{\mu}_{t,i}, \bar{\mu}_{t,i}]}\mu(1-\mu)$, whose closed form solution immediately follows from the equation below,
\begin{align}\label{eq:var_upper}
    % \STATE If variance upper bound $\bar{\bV}$ is available: $\bar{V}_{t,i}=\bar{V}_{i}$; Otherwise, set the optimistic variance as\begin{equation}\label{eq:var_upper}
 \bar{V}_{t,i}= \begin{cases}
(1-\bar{\mu}_{t,i})\bar{\mu}_{t,i}, &\text{if $\bar{\mu}_{t,i} \le \frac{1}{2}$}\\
(1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}, &\text{if $\ubar{\mu}_{t,i} \ge \frac{1}{2}$}\\
\frac{1}{4}, &\text{otherwise}
\end{cases}
\end{align}
% \Cref{eq:var_upper} in line~\ref{line:var_opt}.
where $\bar{\mu}_{t,i}$ and $\ubar{\mu}_{t,i}$ are UCB and LCB values to be introduced later. Notice that with high probability the true $\mu_{t,i}$ lies within LCB and UCB values and as they are getting more accurate, the optimistic variance $V_{t,i}$ is also approaching the true variance $V_{t,i}$.

To guarantee $\hat{\btheta}_t$ is a good estimator, we prove a new lemma (similar to \Cref{lem:c2mab_good_est}) to guarantee the concentration bound of $\btheta_t$ but in face of the unknown variance. Note that the sentinel work \citet{lattimore2015linear} proves a similar concentration bound, the difference is that we have multiple arms triggered in each round instead of a single arm. To address this, we replaced the original concentration bound with the new one below that has an extra $K^4$ factor in $N$, which finally results in $\log K$ factor in the confidence radius $\rho(\delta)$. 

\begin{lemma}\label{lem:va_c2mab_good_est}
Let $\gamma>0, N=(4d^2K^4T^4)^d$ so that $\rho(\delta)=\left(1+\sqrt{\gamma}+4\sqrt{\log\left(\frac{6TN}{\delta}\log\left(\frac{3TN}{\delta}\right)\right)}\right)$. We have for all $t\le T$, with probability at least $1-\delta$, $\norm{\hat{\btheta}_t-\btheta^*}_{\bG_{t}}^2\le \rho(\delta)$.
\begin{proof}
    See \Cref{apdx_sec:TPVM_key_lem}.
\end{proof}
% $\norm{\hat{\btheta}-\btheta_t}_{\bG_{t}}^2\le \beta$
% \begin{align}\label{eq:va_c2mab_optimism}
%     \norm{\hat{\btheta}_t-\btheta^*}_{\bG_{t}}^2\le \beta
% \end{align} 
\end{lemma}
% \siwei{Why not $\rho(\delta)$ here?}

Building on this lemma, we construct $\bar{\mu}_{t,i}$ as an upper bound of $\bmu_{t,i}$ in line~\ref{line:va_ucb}, and $\ubar{\mu}_{t,i}$ as a lower bound of $\bmu_{t,i}$ in line~\ref{line:va_lcb}, based on our variance-adaptive $\hat{\btheta}_t$, $\bG_t$. Note that the doubling of the radius $2\rho(\delta)$ instead of using $\rho(\delta)$ in \Cref{lem:va_c2mab_good_est} is purely for the correctness of our technical analysis. As a convention, we clip $\bar{\mu}_{t,i}, \ubar{\mu}_{t,i}$ into $[0,1]$ if they are above 1 or below 0.
\begin{lemma}\label{lem:va_c2mab_optimism}
    With probability at least $1-\delta$, we have $\mu_{t,i}\le \bar{\mu}_{t,i}\le \mu_{t,i} + 3\rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}}$, and $\mu_{t,i}\ge \ubar{\mu}_{t,i}\ge \mu_{t,i} - 3\rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}}$ for all $i \in [m]$. 
\end{lemma}
\begin{proof}
This lemma follows from the similar derivation of \Cref{lem:c2mab_optimism}, where we have different definitions of $\bar{\mu}_{t,i}, \ubar{\mu}_{t,i}$ and the concentration now relies on  \Cref{lem:va_c2mab_good_est}.   
\end{proof}
% \siwei{Similar question with that after Lemma 2.}
After the agent plays $S_t$, the base arms in $\tau_t$ are triggered, and the agent receives observation set $(X_{t,i})_{i\in \tau_{t}}$ as feedback. These observations (reweighted by optimistic variance $\bar{V}_{t,i}$) are then used to update $\bG_t$ and $\bb_t$ for future rounds.


% Intuitively, if we know an upper bound of $\sigma_i$,  which we denote as $\bar{\sigma}_i$, and we only select one arm each round (i.e., $K=1$), then $\hat{\btheta}_t$ is the closed form solution of the following \textit{weighted ridge regression} problem:
% \begin{align}
%     \hat{\btheta}_t = \arg\min_{\btheta \in \R^d} \sum_{\tau=1}^{t}\sum_{i \in S_{\tau}}(\inner{\btheta, \bphi_\tau(i)}-X_{\tau,i})/\bar{\sigma}_i^2 + \lambda \norm{\btheta}_2^2.
% \end{align}
% The term ``weighted" corresponds the variance upper bound $\bar{\sigma}$. The above estimator is known as the best linear unbiased estimator (BLUE)~\cite{henderson1975best}. Concretely, $\hat{\btheta}_t$ is the lowest variance estimator of $\btheta$ among all unbiased linear estimators.

% \begin{remark}
% The intuition of using variance is from the exploitation perspective: the smaller the variance, the more accurate the data point is, and thus more important for the agent to learn unknown $\btheta$. So we use the inverse of $\bar{V}_{t,i}$ in line \ref{line:update_G} and \ref{line:update_b} to re-weight the observation.
% \end{remark}

% For our problem, we have three key ingredients: (1) We use $v_{t,i}$ is an estimation of $\bar{\sigma}_i$ at round $t$ instead of assuming a known upper bound $\bar{\sigma}_i$; (2) At each round, we select a combinatorial action which consists of multiple arms, i.e., $K > 1$. (3) We incorporate VM condition (\cref{cond:TPVMm}) to remove the factor of $\sqrt{K}$.

\begin{table*}[t]
	\caption{Summary of the coefficients, regret  bounds and improvements for various applications.}	\label{tab:app}	
         \centering 
		\resizebox{1.96\columnwidth}{!}{
	\centering
	\begin{threeparttable}
	\begin{tabular}{|ccccc|}
		\hline
		\textbf{Application}&\textbf{Condition}& \textbf{$(B_v, B_1, \lambda)$} & \textbf{Regret}& \textbf{Improvement}\\
	\hline
  Online Influence Maximization \cite{wen2017online} & TPM &$(-,|V|,-)$   & $O(d|V|\sqrt{|E|T}\log T)$ & $\tilde{O}(\sqrt{|E|})$\\
	    \hline
		Disjunctive Combinatorial Cascading Bandits~\cite{li2016contextual} &  TPVM & $(1,1,2)$ & $O(d\sqrt{T}\log T)$ & $\tilde{O}(\sqrt{K}/p_{\min})$ \\
			\hline
% 			\rowcolor{LightGray}
		Conjunctive Combinatorial Cascading Bandits~\cite{li2016contextual} & TPVM & $(1,1,1)$ & $O( d\sqrt{T}\log T)$ & $\tilde{O}(\sqrt{K} /r_{\max})$\\
			\hline
   Linear Cascading Bandits~\cite{vial2022minimax}$^*$  & TPVM & $(1,1,2)$ & $O(d\sqrt{T}\log T)$ & $\tilde{O}(\sqrt{K/d})$ \\
		   \hline
				% \rowcolor{LightGray}
% 			Influence Maximization on TPG \cite{wang2017improving} & TPVM & $(\sqrt{2}|V|,|V|,1)$ & $O( \sum_{i \in [m]}\log \frac{|E|}{\Delta_{\min}}\frac{|V|^2\log |E| \log T}{\Delta_i^{\min}})$  & $O(|E|/(\log |E|\log \frac{|E|}{\Delta_{\min}}))$\\
				% \hline

      Multi-layered Network Exploration~\citep{liu2021multi} & TPVM & $(\sqrt{1.25|V|},1,2)$ & $O(d\sqrt{|V|T}\log T)$ & $\tilde{O}(\sqrt{n}/p_{\min})$\\
			\hline
	   % 	\rowcolor{LightGray}
	Probabilistic Maximum Coverage \cite{chen2013combinatorial}$^{**}$& VM & $(3\sqrt{2|V|},1,-)$ & $O(d\sqrt{|V|T}\log T)$ & $\tilde{O}(\sqrt{k})$\\
	    \hline
     	   
	\end{tabular}
	  \begin{tablenotes}[para, online,flushleft]
	\footnotesize%\smallskip
	\item[]\hspace*{-\fontdimen2\font} $|V|, |E|, n, k, L$ denotes the number of target nodes, the number of edges that can be triggered by the set of seed nodes, the number of layers, the number of seed nodes and the length of the longest directed path, respectively;
  \item[]\hspace*{-\fontdimen2\font} $K$ is the length of the ordered list, $r_{\max}=\alpha\cdot\max_{t\in [T], S\in \cS} r(S;\bmu_t)$;
   \item[]\hspace*{-\fontdimen2\font}$^*$ A special case of disjunctive combinatorial cascading bandits. 
 \item[]\hspace*{-\fontdimen2\font}$^{**}$ This row is for \ccmab~application and the rest of rows are for \ccmab-T applications. 
% 	\item[]\hspace*{-\fontdimen2\font}$^\ddagger$ $|V|, |E|, n, |L|$ denotes the number of layers, the number of longest;
% 	\item[]\hspace*{-\fontdimen2\font}$^\ddagger$ $L$ is the number of ;
% 	\item[]\hspace*{-\fontdimen2\font}$^{\S}$ This work gives sufficient smoothness condition with factor $\gamma_g$ and translates to $B_v=3\sqrt{2}\gamma_g$ in our setting.
	\end{tablenotes}
			\end{threeparttable}
	}
\end{table*}

\subsection{Results and Analysis under VM condition}
We first show a regret bound for VAC$^2$-UCB that is independent of batch size $K$ when the VM condition holds.
\begin{theorem}\label{thm:ccmab_reg_VM}
    For a \ccmab-T instance that satisfies monotonicity (Condition~\ref{cond:mono}) and VM smoothness (Condition~\ref{cond:VM}) with coefficient $(B_v,B_1)$, VAC$^2$-UCB (\Cref{alg:va_cucb}) with an $(\alpha,\beta)$-approximation oracle achieves an $(\alpha,\beta)$-approximate regret bounded by $ O\left(\frac{B_v}{\sqrt{p_{\min}}}(\sqrt{d\log (KT/\gamma)}+\sqrt{\gamma})\sqrt{Td\log(KT/\gamma)}\right).$
\end{theorem}
% \begin{remark}
\textbf{Discussion.} Looking at \Cref{thm:ccmab_reg_VM}, we achieve an $O(B_vd\sqrt{T}\log T/\sqrt{p_{\min}})$ regret bound when $d \ll K \le m \ll T$. For combinatorial cascading bandits~\cite{li2016contextual} with $B_v=1$, our regret is independent of $m, K$ and improves~\citet{li2016contextual} by a factor $O(\sqrt{K/p_{\min}})$.
% \end{remark}

% \begin{remark} 
 In addition to the general \ccmab-T setting, one can verify that for non-triggering \ccmab, $p_{\min}=1$, and we obtain the batch-size independent regret bound $O(B_vd\sqrt{T}\log T)$. Recall $B_v=O(B_1\sqrt{K})$ for any \ccmab-T instances, so our regret bound reproduces $O(B_1d\sqrt{KT}\log T)$, and thus matches the similar lower bound~\cite{takemura2021near} for the linear reward functions. For the more interesting non-linear reward function with $B_v=o(B_1\sqrt{K})$, our regret improves non-variance-adaptive algorithm C$^2$UCB, whose regret is $O(B_1d\sqrt{KT}\log T)$~\cite{qin2014contextual,takemura2021near}.
% \end{remark}

\noindent\textbf{Analysis.} At a high level, the improvement of $\sqrt{K}$ comes from the VM condition and the optimistic variance, which together save the use of Cauchy-Schwarz inequality that generates a $O(\sqrt{K})$ factor in the step (b) of \Cref{eq:c2mab_reg}. In order to leverage the variance information, we decompose the regret into term (\rom{1}) and (\rom{2}),
\noindent
\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
\begin{talign}
&\text{Reg}(T)\le \E\left[\sum_{t=1}^T r(S_t; \bar{\bmu}_t)- r(S_t; \bmu_t)\right]\notag\\
&\le \E[\sum_{t=1}^T \underbrace{\abs{r(S_t; \bar{\bmu}_t)- r(S_t; \tilde{\bmu}_t)}}_{\text{(\rom{1})}}+\underbrace{\abs{r(S_t; \bmu_t)- r(S_t; \tilde{\bmu}_t)}}_{\text{(\rom{2})}}]\label{eq:regret_decompose},
% &\le B_v\E\left[\sum_{t=1}^T\left(\sqrt{\sum_{i \in [m]}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}+\sqrt{\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right)\right]\\
% &\le  B_v\E\left[\sqrt{T\sum_{t=1}^T\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}+\sqrt{T\sum_{t=1}^T\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right]\\
% &\le B_v\sqrt{T}\sqrt{\E\left[\sum_{t=1}^T\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}+\sqrt{\E\left[\sum_{t=1}^T\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}\\
\end{talign}
\end{minipage}}
where $\tilde{\bmu}_{t}$ is the vector whose $i$-th entry is the maximizer that achieves optimistic variance $\bar{V}_{t,i}$, i.e., $\tilde{\mu}_{t,i}=\argmax_{\mu\in [\ubar{\mu}_{t,i}, \bar{\mu}_{t,i}]}\mu(1-\mu)$.
Now we show a sketched proof to bound the term  (\rom{1}) and one can bound the term {(\rom{2})} similarly.
\noindent
\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
\begin{talign}
&\E\left[\sum_{t\in[T]}\text{(\rom{1})}\right] \overset{(a)}{\le} B_v\E\left[\sum_{t=1}^T\sqrt{\sum_{i \in \tilde{S}_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}}\right]\notag\\
& \overset{(b)}{\le}  \frac{B_v}{\sqrt{p_{\min}}}\cdot \E\left[\sum_{t=1}^T\sqrt{\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}}\right]\notag\\
% & \le  \frac{B_v}{\sqrt{p_{\min}}}\cdot \E\left[\sqrt{T\sum_{t=1}^T\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}}\right]\notag\\
& \overset{(c)}{\le}  \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}\right]}\notag\\
% & \overset{(d)}{=}  \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tau_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}\right]}\notag\\
&\overset{(d)}{\le} \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tau_t}{(6\rho(\delta)\norm{\bphi_t(i)}_{\bG_{t}^{-1}})^2}/{\bar{V}_{t,i}}\right]}\notag\\
&\overset{(e)}{\le} O(B_vd\sqrt{T\log T}/\sqrt{p_{\min}}),\label{eq:regret_derive_VM}
\end{talign}
\end{minipage}}
where (a) is by Condition~\ref{cond:VM}, (b) is by the definition of $p_i^{\bmu_t,S_t}\ge p_{\min}$ for $i \in \tilde{S}_t$, (c) is by Cauchy–Schwarz over $t$ and the Jensen's inequality, (d) follows from the TPE and \Cref{lem:va_c2mab_optimism}, (e) follows from \Cref{apdx_lem:ccmab_potential_new}.



\subsection{Results and Analysis under TPVM Condition}
Next, we show that VAC$^2$-UCB can achieve regret bounds that remove the $O(\sqrt{K})$ and $O(1/\sqrt{p_{\min}})$ factor for applications satisfying the stronger TPVM conditions.

We first introduce a mild condition over the triggering probability (which is similar to Condition~\ref{cond:TPM}) to give our regret bounds and analysis.

\begin{condition}[\textbf{1-norm TPM Bounded Smoothness for Triggering Probability}]\label{cond:TPM_P}
% We say that a CMAB-T instance satisfies TPM $B_1$-bounded smoothness condition, if for any action $S \in \cS$, any distribution $D,D'$ with mean vector $\bmu \in (0,1)^m$, we have $\frac{\partial r(S;\bmu)}{\partial \mu_i } \frac{1}{p_{i}^{D,S}}\le B_1 $ for $i \in \tilde{S}$ and $\frac{\partial r(S;\bmu)}{\partial \mu_i }=0$ for $i \in [m] \backslash \tilde{S}$. 
We say that a \ccmab-T problem instance satisfies the triggering probability modulated $B_p$-bounded smoothness condition over the triggering probability, if for any action $S \in \cS$, any mean vectors $\bmu, \bmu' \in [0,1]^m$, and any arm $i\in[m]$, we have $|p_i^{\bmu', S}-p_i^{\bmu, S}|\le B_p\sum_{j \in [m]}p_{j}^{\bmu,S}|\mu_j-\mu'_j|$.
%\siwei{seems no formal definition of this $p_{i}^{D,S}$?} 
\end{condition}

Now we state our main theorem as follows.
\begin{theorem}\label{thm:ccmab_reg_TPVM_lambda}
    For a \ccmab-T instance, when its reward function satisfies monotonicity (Condition~\ref{cond:mono}) and TPVM smoothness (Condition~\ref{cond:TPVMm}) with coefficient $(B_v,B_1, \lambda)$, and its triggering probability $p_i^{\bmu,S}$ satisfies 1-norm TPM smoothness with coefficient $B_p$ (Condition~\ref{cond:TPM_P}),
    if $\lambda \ge 2$, then VAC$^2$-UCB (\Cref{alg:va_cucb}) with an $(\alpha,\beta)$-approximation oracle achieves an $(\alpha,\beta)$-approximate regret bounded by 
    \begin{align}
        O\left(B_v d\sqrt{T}\log T + {B_vB_pd\sqrt{K}\log T}/{\sqrt{p_{\min}}}\right),
    \end{align}
    and if $\lambda \ge 1$, then VAC$^2$-UCB (\Cref{alg:va_cucb}) achieves an $(\alpha,\beta)$-approximate regret bounded by
    \begin{align}
    O\left(B_v d\sqrt{T}\log T + {B_v\sqrt{B_p}(KT)^{1/4}(d\log T)^{3/4}}/{\sqrt{p_{\min}}}\right).
    \end{align}    
\end{theorem}

\textbf{Discussion.}
The leading term of \Cref{thm:ccmab_reg_TPVM_lambda} is $O(B_vd\sqrt{T}\log T)$ when $d\ll K\le m\ll T$, which removes the $1/\sqrt{p_{\min}}$ factor compared with \Cref{thm:ccmab_reg_VM}. Also, notice that \Cref{thm:ccmab_reg_TPVM_lambda} relies on an additional $B_p$-smoothness condition over the triggering probability. However, we claim that this condition is mild and almost always satisfies with $B_p=B_1$ for applications considered in this paper (see \Cref{apdx_sec:apps}). %The purpose of this condition is to handle the mismatch of the triggering probability when using the TPE, which will be introduced shortly after.
% Finally, when there exists some prior knowledge about the variance bound $\bar{V}_i$, s.t. $\Var[X_{t,i}]\le \bar{V}_i\le C_1\Var[X_{t,i}]$, we can achieve $O(B_vd\sqrt{T}\log T)$ bound for general $\lambda \ge 1$, without assuming the $B_p$ smoothness condition. We refer interested readers to the Appendix for its details.
% \end{remark}

\textbf{Analysis.} We use the regret decomposition of \Cref{eq:regret_decompose} to the same term (\rom{1}) and (\rom{2}), and leverage on TPVM condition (Condition~\ref{cond:TPVMm}) to obtain:
\begin{equation}
 \resizebox{.91\linewidth}{!}{$
            \displaystyle
\E\left[\sum_{t\in[T]}\text{(\rom{1})}\right] \overset{(a)}{\le} B_v\E\left[\sum_{t=1}^T\sqrt{\sum_{i \in \tilde{S}_t}(p_i^{\tilde{\bmu}_t, S_t})^{\lambda}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}}\right]$}.\label{eq:TPVM_mismatch_1}
\end{equation}

However, we cannot use TPE as \Cref{eq:regret_derive_VM} because $p_i^{\tilde{\bmu}_t,S_t}\neq p_i^{\bmu_t,S_t}$ in general. To handle this mismatch, we use the fact that triggering probability usually satisfies a smoothness condition in Condition~\ref{cond:TPM_P}, and prove that the mismatch only affect the lower-order term as follows: 

By Condition~\ref{cond:TPM_P}, $(p_i^{\tilde{\bmu}_t,S_t})^\lambda$ is upper bounded by $(p_i^{\bmu_t,S_t}+\min\{1,\sum_{j \in \tilde{S}_t}B_p p_j^{\bmu, S_t}\abs{{\mu}_{t,j}-\tilde{\mu}_{t,j}}\})^2$ when $\lambda \ge 2$, and the regret is bounded by the terms as shown below:
\noindent
\resizebox{.97\columnwidth}{!}{
\begin{minipage}{\columnwidth}
\begin{talign*}
&\text{Eq. }(\ref{eq:TPVM_mismatch_1}) \le \underbrace{\E\left[\sum_{t=1}^T B_v \sqrt{\sum_{i \in \tilde{S}_t}3p_i^{\bmu_t,S_t}{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}/{\bar{V}_{t,i}}} \right]}_{\text{leading term}}\notag\\
&+\underbrace{\frac{B_vB_p\sqrt{K}}{\sqrt{p_{\min}}}\E\left[ \sum_{t=1}^T \sum_{i \in \tilde{S}_t}{p_i^{\bmu_t,S_t}(\bar{\mu}_{t,i}-\ubar{\mu}_{t,i})^2}/{\bar{V}_{t,i}}\right]}_{\text{lower-order term}},
\end{talign*}
\end{minipage}}
where the leading term is of order $O(B_v \sqrt{T}\log T)$ by using the same derivation of step (c)-(e) in \Cref{eq:regret_derive_VM}, and the lower order term is bounded by $O(B_vB_p\sqrt{K/p_{\min}}\log T)$ by TPE and the weighted ellipsoidal potential lemma (\Cref{apdx_lem:ccmab_potential_new}). For $\lambda \ge 1$, the lower-order term becomes $\frac{B_v\sqrt{B_p}K^{1/4}}{\sqrt{p_{\min}}}\E\left[ \sum_{t=1}^T \left(\sum_{i \in \tilde{S}_t}\frac{p_i^{\bmu_t,S_t}(\bar{\mu}_{t,i}-\ubar{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right)^{3/4}\right]$, which results in a larger lower-order regret term. See \Cref{apdx_sec:proof_TPVM_lambda} for details.
% UNKNOWN VARIANCE
% Let $\tilde{\bmu}_{t}$ be the vector whose $i$-th entry is the maximizer that achieves $\bar{V}_{t,i}$, i.e., $\tilde{\mu}_{t,i}=\argmax_{\mu\in [\ubar{\mu}_{t,i}, \bar{\mu}_{t,i}]}\mu(1-\mu)$. We first decompose the regret as follows
% \begin{align}
% &\text{Reg}(T)\le \E\left[\sum_{t=1}^T  \alpha r(S_t^*; \bmu_t)- r(S_t; \bmu_t)\right]\\
% &\le \E\left[\sum_{t=1}^T r(S_t; \bar{\bmu}_t)- r(S_t; \bmu)\right]\\
% &\le \E\left[\sum_{t=1}^T \underbrace{\abs{r(S_t; \bar{\bmu}_t)- r(S_t; \tilde{\bmu}_t)}}_{\text{(\rom{1})}}+\underbrace{\abs{r(S_t; \bmu_t- r(S_t; \tilde{\bmu}_t)}}_{\text{(\rom{2})}}\right]
% % &\le B_v\E\left[\sum_{t=1}^T\left(\sqrt{\sum_{i \in [m]}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}+\sqrt{\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right)\right]\\
% % &\le  B_v\E\left[\sqrt{T\sum_{t=1}^T\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}+\sqrt{T\sum_{t=1}^T\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right]\\
% % &\le B_v\sqrt{T}\sqrt{\E\left[\sum_{t=1}^T\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}+\sqrt{\E\left[\sum_{t=1}^T\frac{(\mu_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}\\
% \end{align}
% where the newly added $r(S_t; \tilde{\bmu}_t)$ is the key term that helps us to use the variance information.
% Now we show a sketched proof to bound the term  (\rom{1}) and one can bound the term \textbf{(\rom{2})} similarly.
% \begin{align}
% &\E\left[\sum_{t\in[T]}\text{(\rom{1})}\right] \le B_v\E\left[\sum_{t=1}^T\sqrt{\sum_{i \in \tilde{S}_t}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right]\notag\\
% & \le  \frac{B_v}{\sqrt{p_{\min}}}\cdot \E\left[\sum_{t=1}^T\sqrt{\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right]\notag\\
% % & \le  \frac{B_v}{\sqrt{p_{\min}}}\cdot \E\left[\sqrt{T\sum_{t=1}^T\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}}\right]\notag\\
% & \le  \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tilde{S}_t}p_{i}^{\bmu_t,S_t}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}\notag\\
% & =  \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tau_t}\frac{(\bar{\mu}_{t,i}-\tilde{\mu}_{t,i})^2}{\bar{V}_{t,i}}\right]}\notag\\
% &\le \frac{B_v}{\sqrt{p_{\min}}}\cdot \sqrt{T\E\left[\sum_{t=1}^T\sum_{i \in \tau_t}\frac{(4\beta\norm{\bphi_t(i)}_{\bG_{t}})^2}{\bar{V}_{t,i}}\right]}\notag\\
% &\le \tilde{O}(B_vd\sqrt{T\log T}/\sqrt{p_{\min}}),
% \end{align}
% where (a) follows from Condition~\ref{cond:TPVMm}, (b) is by applying Condition~\ref{cond:TPM_P} for triggering probability $p_i^{\bar{\bmu}_{t}\tilde{S}_t}\in \le 1$, (c) follows from $\sqrt{a+b}\le \sqrt{a} + \sqrt{b}$, (d) follows from same derivation from \Cref{apdx_eq:va_ccmab_term_1}, (e) follows from $p_i^{\tilde{\bmu}_t,S_t}\ge p^i_{\min}$, (f) follows from Cauchy-Schwarz, (g) follows from $\bar{V}_{t,i}\le 1/4$, (e) follows from the similar analysis of $(b)$ in \Cref{apdx_eq:va_ccmab_term_1} but without the square-root and $B_v/\sqrt{p_{\min}}$. 



==> content/5_new_analysis.tex <==
% \section{Improving CMAB-T Using TPE Trick}\label{sec:nc_c2mab}
% In this section, we present the TPE technique can be used to reproduce the context-free CAMB-T results~\cite{wang2017improving} under TPM condition (in a simpler and more intuitive manner), and to improve the results~\cite{liu2022batch} under the TPVM condition.

% Recall that the context-free CMAB-T is to set $\btheta^*=\bmu\triangleq(\mu_1,...,\mu_m)\in (0,1)^m$, $\bphi_t(i)$ is fixed to the one hot vector $\be_i\in \R^{m}$, and the mean vector is fixed to $\bmu_t=\bmu$.
% To state the main result and the analysis, we denote 
% \subsection{Reproducing CMAB-T under TPM Condition}
% \begin{theorem}
% THEOREM HERE.
% \end{theorem}

% ANALYSIS. The main idea is to use TPTE trick to replace $\tilde{S}_t$ with $\tau_t$ (whose counter is $T_{t,i}$) regarding conditional expectation $\E_t$. Such replacement bypasses the triggering group analysis that assigns a counter $N_{t,i,j}$ (which adds one only if action $S_t$ could trigger $i$ and $p_i^{\bmu,S}\in [2^{-j}, 2^{-j+1})$ action $S_t$), and uses this counter to associate $T_{t,i}$ for the analysis. Using this trick, we can use a simpler proof (similar to Appendix B.2. of \cite{wang2017improving}) to replace the more involved Appendix B.3 of \cite{wang2017improving}. Specifically, similar to XXX, we bound $\Delta_{S_t}$
% \begin{align}
%     \Delta_{S_t}&\le B_1 \sum_{i \in [m]}p_i^{D, S_t}(\bar{\mu}_{t,i}-\mu_i)\\
%     &\le -\Delta_{S_t} + 2B_1 \sum_{i \in [m]}p_i^{D, S_t}(\bar{\mu}_{t,i}-\mu_i)\\
%     &=-\frac{\sum_{i \in [m]}p_i^{D, S_t}\Delta_{S_t}}{\sum_{i \in [m]}p_i^{D, S_t}}+2B_1 \sum_{i \in [m]}p_i^{D, S_t}(\bar{\mu}_{t,i}-\mu_i)\\
%     &\le 2B_1 \sum_{i \in [m]}p_i^{D,S_t}\left(-\frac{M_i}{2B_1K}+ (\bar{\mu}_{t,i}-\mu_i)\right)\\
%     &\le  2B_1 \sum_{i \in [m]}p_i^{D,S_t}\left(-\frac{M_i}{2B_1K}+ \sqrt{\frac{\log T}{T_{t-1,i}}}\right)\\
%     % &\le \sum_{i \in [m]}p_i^{D,S_t}\kappa_T(M_i, T_{t-1,i}).
% \end{align}

% It follows that 
% \begin{align}
%     \Delta_{S_t}&=\E_t[\Delta_{S_t}]\le \E_t\left[2B_1 \sum_{i \in [m]}p_i^{D,S_t}\left(-\frac{M_i}{2B_1K}+ \sqrt{\frac{\log T}{T_{t-1,i}}}\right)\right]\\
%     &= \E_t\left[2B_1\sum_{i \in [m]}\I\{i \in \tilde{A}_t\}\left(-\frac{M_i}{2B_1K}+ \sqrt{\frac{\log T}{T_{t-1,i}}}\right)\right]\\
%     &= \E_t\left[2B_1\sum_{i \in \tilde{A}_t}\left(-\frac{M_i}{2B_1K}+ \sqrt{\frac{\log T}{T_{t-1,i}}}\right)\right]\\
%     &\le \E_t \left[\sum_{i \in \tilde{A}_t}\kappa_T(M_i,T_{t-1,i})\right].
% \end{align}

% \subsection{Improving CMAB-T under TPVM condition}
% \textbf{(a) When $\lambda \in [1,2)$,} 

% Given filtration $\cF_t$, 

% \begin{align}
%      \Delta_{S_t} &\le \sum_{i \in [m]} \frac{ 4c_1^2 B_v^2 (p_{i}^{D,S_t})^{\lambda}\frac{\log t}{T_{i,t-1}}}{\Delta_{S_t}} \label{eq:ra_def_e1}\\
%     &=-\Delta_{S_t} + 2\sum_{i \in [m]} \frac{ 4c_1^2 B_v^2 (p_{i}^{D,S_t})^{\lambda}\frac{\log t}{T_{i,t-1}}}{\Delta_{S_t}}\\
%     &=-\frac{\sum_{i\in \tilde{S}_t}p_i^{D,S_t}\Delta_{S_t}/(p_i^{D,S_t})^{\lambda-1}}{\sum_{i \in[m]}(p_i^{D,S})^{2-\lambda}} + 2\sum_{i \in [m]} \frac{ 4c_1^2 B_v^2 (p_{i}^{D,S_t})^{\lambda}\frac{\log t}{T_{i,t-1}}}{\Delta_{S_t}}\\
%     &\le \sum_{i \in [m]}p_i^{D,S_t} \left(\frac{ 8c_1^2 B_v^2 \frac{\log t}{T_{i,t-1}}}{\Delta_{S_t}/(p_i^{D,S_t})^{\lambda-1}}-\frac{\Delta_{S_t}/(p_i^{D,S_t})^{\lambda-1}}{K}\right)\\
%     &= \sum_{i \in [m]}p_i^{D,S_t} \left(\frac{ 8c_1^2 B_v^2 \frac{\log t}{T_{i,t-1}}}{{\tDelta}_{S_t,\lambda}}-\frac{\tilde{\Delta}_{S_t}}{K}\right),
% \end{align}
% where $K=\sum_{i\in [m]}(p_i^{D,S})^{2-\lambda}$, $\tDelta_{S_t}=\Delta_{S_t}/(p_i^{D,S})^{\lambda-1}$. The rest follows exactly the same as $\lambda=2$ case in previous section.
% \begin{align}
%     \Delta_{S_t} =\E_t[\Delta_{S_t}]  &\le  \E_t\left[\sum_{i \in [m]}p_i^{D,S_t}\left(\frac{ 8c_1^2 B_v^2 \frac{\log t}{T_{i,t-1}}}{\tilde{\Delta}_{S_t,\lambda}}-\frac{\tilde{\Delta}_{S_t}}{K}\right)\right]\\
%     &= \E_t\left[ \sum_{i \in \tilde{A}_t}\left(\frac{ 8c_1^2 B_v^2 \frac{\log t}{T_{i,t-1}}}{\tDelta_{S_t,\lambda}}-\frac{\tDelta_{S_t}}{K}\right)\right]\\
%     &\le \E_t\left[\sum_{i \in \tilde{A}_t}{ \kappa_{i,T}(T_{t-1,i})}\right]\label{eq:kappa_tpvm_general}
% \end{align}
% where we define a regret allocation function 
% \begin{equation}
% \kappa_{i,T}(\ell) = \begin{cases}
% \frac{c_1^2 B_v^2} {\tilde{\Delta}_{i,\lambda}^{\min}}, &\text{if $\ell=0$,}\\
% 2\sqrt{\frac{4c_1^2 B_v^2 \log T}{\ell }}, &\text{if $1\le\ell\le L_{i,T,1}$,}\\
% \frac{8c_1^2 B_v^2 \log T}{\tilde{\Delta}_{i,\lambda}^{\min} }\frac{1}{\ell}, &\text{if $L_{i,T,1} < \ell \le L_{i,T,2}$,}\\
% 0, &\text{if $\ell > L_{i,j,T,2}$,}
% \end{cases}
% \end{equation}
% where $L_{i,T,1}=\frac{4c_1^2 B_v^2\log T}{\tilde{\Delta}_{i}^{\min}\cdot \tilde{\Delta}_{i,\lambda}^{\min}}$, $L_{i,T,2}=\frac{8c_1^2 B_v^2K\log T}{\tilde{\Delta}_{i}^{\min}\cdot \tilde{\Delta}_{i,\lambda}^{\min}}$, $\tilde{\Delta}_{i}^{\min}=\min_{S: p_i^{D,S}>0, \Delta_S>0}\Delta_{S_t}/p_i^{D,S_t}$, $ \tilde{\Delta}_{i,\lambda}^{\min}=\min_{S: p_i^{D,S}>0, \Delta_S>0}\Delta_{S_t}/(p_i^{D,S_t})^{\lambda-1}$.

% \begin{align}
% \text{Reg}(T) &\le\sum_{i\in [m]}\frac{c_1^2 B_v^2 }{\tDelta_{i,\lambda}^{\min}}+  \sum_{i \in [m]} \frac{8c_1^2 B_v^2 \log T}{\tDelta_{i,\lambda}^{\min} } (1+\log K) \\
% &+ \sum_{i \in [m]} \frac{16c_1^2 B_v^2 \log T}{\sqrt{\tDelta_{i,\lambda}^{\min}\cdot\tDelta_{i}^{\min}} }.    
% \end{align}

==> content/6_applications.tex <==

\section{Applications and Experiments}\label{sec:app}
% \jinhang{Comments for this section: 1) be careful about the parameters for different applications; 2) there's no application for Alg 2, maybe put PMC and add some examples there}
% \siwei{Maybe we can move this part to just below Theorem 1. In this section we mainly focus on how the applications follow our condition 3.} \carlee{I agree with this suggestion.} 
We now move to applications and experimental results.  We first show how our theoretical results improve various \ccmab~and \ccmab-T applications under 1-norm TPM, TPVM and VM smoothness conditions with their corresponding $B_1, B_v, \lambda$ coefficients. Then, we provide an empirical comparison in the context of the contextual cascading bandit application.

The instantiation of our theoretical results in the context of a variety of specific \ccmab~ and \ccmab-T applications is shown in \Cref{tab:app}.  The final column of the table details the improvement in regret that our results yield in each case. For detailed settings, proofs, and the discussion of the application results, see \Cref{apdx_sec:apps}.

Our experimental results are summarized in \Cref{fig:reg}, which details experiments on the MovieLens-1M dataset\footnote{ \href{https://grouplens.org/datasets/movielens/1m/}{grouplens.org/datasets/movielens/1m/}}.  Experiments on other data are included in the Appendix. \Cref{fig:reg} illustrates that our VAC$^2$-UCB algorithm outperforms C$^3$-UCB~\cite{li2016contextual}, the variance-agnostic cascading bandit algorithm, and CascadeWOFUL~\cite{vial2022minimax}, the state-of-the-art variance-aware cascading bandit algorithm, eventually incurring $45\%$ and $25\%$ less regret.
For detailed settings, comparisons, and discussions, see \Cref{sec:apps-exp}.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.43\linewidth]{figures/ICML/real_all.png}
%     \caption{Results for MovieLens data}
%     \label{fig:syn_lin}
% \end{figure}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.43\linewidth]{figures/ICML/real_genre.png}
%     \caption{Results for MovieLens data}
%     \label{fig:syn_lin}
% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{real_all.png}
    \caption{All genres}
    \label{fig:real_all}
    \end{subfigure}
    \begin{subfigure}[t]{0.48\linewidth}
    \includegraphics[width=\linewidth]{real_genre.png}
    \caption{Particular genre}
    \label{fig:real_genre}
    \end{subfigure}
    \caption{Regret results for MovieLens data.}
    \label{fig:reg}
\end{figure}

==> content/7_conclusion.tex <==
% \vspace{-7pt}
\section{Conclusion}\label{sec:conclusion}
% \vspace{-7pt}
This paper studies contextual combinatorial bandits with probabilistically triggered arms (\ccmab-T) under a variety of smoothness conditions. 
Under the triggering probability modulated (TPM) condition, we design the C$^2$-UCB-T algorithm 
and propose a novel analysis to achieve an $\tilde{O}(d\sqrt{KT})$ regret bound, removing a potentially exponentially large factor $O(1/p_{\min})$.
Under the variance modulated conditions (VM or TPVM), we propose a new variance-adaptive algorithm  VAC$^2$-UCB and derive a regret bound $\tilde{O}(d\sqrt{T})$, which removes the batch-size $K$ dependence. As valuable by-product, we find our TPE analysis technique and variance-adaptive algorithm can be applied to the CMAB-T and \ccmab~setting, improving existing results as well. Experiments show that our algorithm can achieve at least 13\% and 25\% improvement compared with benchmark algorithms on synthetic and real-world datasets, respectively.
For the future study, it would be interesting to extend our application scenarios. One could also relax the perfectly linear assumption by introducing model mis-specifications or corruptions.

\section*{Acknowledgement}
The work of John C.S. Lui was supported in part by RGC’s GRF 14215722. The work of Mohammad Hajiesmaili is supported by NSF CAREER-2045641, CPS-2136199, CNS-2106299, and CNS-2102963. Wierman is supported by NSF grants CNS-2146814, CPS-2136197, CNS-2106403, and NGSDI-2105648.

% This paper formulates the multi-layered network exploration via random walks (\mulane) as a budget allocation problem, requiring that the total weights of distinct nodes visited on the multi-layered network is maximized.
% % We systematically study the \mulane{} problem from offline optimization to online learning for both overlapping and non-overlapping networks.
% % For the offline setting, we propose offline algorithms which achieve a constant ratio approximation for the overlapping case and the optimal solution for the non-overlapping case.
% For the offline setting, we propose four algorithms for \mulane{} according to the specification of multi-layered network (overlapping or non-overlapping) and starting distributions (arbitrary or stationary), each of which has a provable guarantee on approximation factors and running time.
% We further study the online setting where network structure and the node weights are not known a priori.
% We propose the CUCB-MAX algorithm for overlapping \mulane{} and the CUCB-MG algorithm for the non-overlapping case, both of which are bounded by a $O(\log T)$ (approximate) regret.
% Finally, we conduct experiments on a social network dataset to show the empirical performance of our algorithms.

% There are many compelling directions for the future study.
% For example, it would be interesting to extend our problem where the decision maker can jointly optimize the starting distribution and the budget allocation.
% One could also study the adaptive \mulane{} by using the feedback from
% the exploration results of the previous steps to determine the exploration strategy for future steps.



==> content/9_linear_extension.tex <==
\clearpage
\section{Variance-Adaptive Algorithms for Linear Contextual Combinatorial Multi-Armed Bandits}
Our goal is to apply our TPVM or VM condition to the contextual combinatorial bandits, with the hope of removing $\sqrt{K}$ factor of previous results $\tilde{O}(\frac{d}{p^*}\sqrt{KT})$ \cite{li2016contextual}. For simplicity, we consider the non-triggering CMAB for now.

\subsection{Setting}
Our setting is similar to that of \cref{sec: problem setting}, the difference is that we now have a feature map $\phi:[m]\rightarrow \R^d$, an unknown parameter vector $\btheta^*\in \R^d$, and the mean reward $\mu_i = \inner{\boldsymbol{\phi(i)},\btheta^*}$ for $i \in [m]$. At each time $t$ and given history $\cH_t$, the outcome $X_{t,i}=\mu_i + \eta_{t,i}$ of arm $i$ is bounded within $[0,1]$. We assume $X_{t,i}$ is a random variable with $\E[\eta_{t,i}|\cH_t]=0$, $\E[\eta_{t,i}^2|\cH_t]\le \sigma_i^2 $, are \textbf{independent} across arm set.
To this end, we can rewrite $r(S;\bmu)=r(S;\btheta^*,\phi)$ and $S^*=\arg\max_{S \in \cS}r(S;\btheta^*,\phi)$.

Note that we can extend to time-variant contexts, i.e., $\phi_t$ and define $S_t^*=\arg\max_{S \in \cS} r(S;\btheta^*, \phi_t)$. 
The $(\alpha, \beta)$-approximate regret is defined as
\begin{align}
     Reg(T;\alpha, \beta)= \sum_{t=1}^T \alpha\beta \cdot r(S_t^*;\btheta^*, \phi_t)-\E\left[\sum_{t=1}^Tr(S_t;\btheta^*,\phi_t)\right].
\end{align}

Let $\Phi_t=[\phi_{t,1}, ..., \phi_{t,m}]\in \R^{d \times m}$, the reward is $\inner{\Phi^{\top}\theta, S_t}=\inner{\theta, \Phi S_t}=\theta^{\top} \Phi S_t$. $\tilde{\btheta}_{t}(i)=\arg\max_{i \in [m]}{\hat{\btheta}_t+\frac{(G_{t})^{-1}\phi_{t,i}}{\norm{(G_{t})^{-1/2}\phi_{t,i}}_2}}$.

\subsection{Algorithm}
\begin{algorithm}[h]
	\caption{BC$^2$UCB-T: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Known Variance Upper Bound $\bar{\sigma}_i^2$}\label{alg:BC^2UCB-T_known}
			\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, known variance upper bound $\bar{\sigma}_i$, computation oracle ORACLE.
	   % \OUTPUT Budget allocation $\bk$.
	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
	   \For{$t=1, ...,T$ }
	   \State $\hat{\btheta}_{t}=\bG_{t-1}^{-1}\bb_{t-1}$. \Comment{Compute the empirical estimator.}
	   %\State Construct the confidence set, one for decision, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$.
	   \For{$i \in [m]$}
	    \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + \sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}$.
	    \Comment{UCB value for base arm $i$.}
	    \State $\bar{\mu}_{t,i} =\min\{\bar{\mu}_{t,i},1\} $
	    \EndFor
	   %\State $G_t=\lambda \boldsymbol{I} + \sum_{\tau < t}\bphi(i)\bphi(i)^{\top}$.
	   %$\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1, i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.
	   %\State Set UCB value $\bar{\mu}_{t,i}=\min \{\hat{\mu}_{t-1, i}+\rho_{t, i},1\}$.
	   %\State $S_t=\text{ORACLE}(C_t^{\theta}, \phi_t)$.  \qquad\qquad\qquad\qquad\qquad//$S_t=\arg\max_{S \in \cS, \bnu \in C_t^{\theta}} r(S;\bnu, \phi_t)$.
	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. \Comment{Computational oracle using UCBs.}
	    \For{$ i \in \tau_t$ } \Comment{Update statistics using the triggered arms' observation.}
	   %\State $v_{t,i}=\max_{\bnu \in C^{v}_{t}}\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})$.
	   \State $\bG_t=\bG_{t-1}+ (\bar{\sigma}_i^2)^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
	   \State $\bb_t=\bb_{t-1}+ (\bar{\sigma}_i^2)^{-1}\bphi_{t}(i) X_{t,i}$.
	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
	   % \label{line:trigger_upd}
	   \EndFor
	    	   \EndFor
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}
Inspired by \cite{lattimore2015linear,zhou2021nearly,vial2022minimax}, we adopt the weighted ridge-regression to learn the unknown parameter $\theta^*$. 
Intuitively, if we know an upper bound of $\sigma_i$,  which we denote as $\bar{\sigma}_i$, and we only select one arm each round (i.e., $K=1$), then $\hat{\btheta}_t$ is the closed form solution of the following \textit{weighted ridge regression} problem:
\begin{align}
    \hat{\btheta}_t = \arg\min_{\btheta \in \R^d} \sum_{\tau=1}^{t}\sum_{i \in S_{\tau}}(\inner{\btheta, \bphi_\tau(i)}-X_{\tau,i})/\bar{\sigma}_i^2 + \lambda \norm{\btheta}_2^2.
\end{align}
The term ``weighted" corresponds the variance upper bound $\bar{\sigma}$. The above estimator is known as the best linear unbiased estimator (BLUE)~\cite{henderson1975best}. Concretely, $\hat{\btheta}_t$ is the lowest variance estimator of $\btheta$ among all unbiased linear estimators.

For our problem, we have three key ingredients: (1) We use $v_{t,i}$ is an estimation of $\bar{\sigma}_i$ at round $t$ instead of assuming a known upper bound $\bar{\sigma}_i$; (2) At each round, we select a combinatorial action which consists of multiple arms, i.e., $K > 1$. (3) We incorporate VM condition (\cref{cond:VM}) to remove the factor of $\sqrt{K}$.

\subsection{Analysis}
\subsubsection{Known Variance Upper Bound}
Suppose we know an upper bound of $\sigma_i$, i.e., $\bar{\sigma}_i^2=C_1^2\sigma_i^2$ for some $C_1^2 \ge 1$.
\begin{align}
    Reg(T) &= \sum_{t=1}^T \alpha r(S_t^*; \btheta^*, \phi_t) - r(S_t; \btheta^*, \phi_t) \\
    &\le \sum_{t=1}^T  r(S_t^*; \tilde{\btheta}_t, \phi_t)- r(S_t; \btheta^*, \phi_t) 	& \mbox{$(\tilde{\btheta}_t, S_t)=\arg\max_{S \in \cS, \btheta \in C_t^{\theta}}r(S;\btheta,\phi_t)$} \label{apdx_eq: linear_mono}\\
    &\le\sum_{t=1}^T B_v\sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}{\sigma_i^2}} 	& \mbox{\cref{cond:VM} with $\zeta_i = \inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}$}\label{apdx_eq: linear_use_cond_VM}\\
    &=\sum_{t=1}^T B_vC_1\sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}{\bar{\sigma}_i^2}} 	& \mbox{$\bar{\sigma}_i^2=C_1^2\sigma_i^2$}\\
   &\le\sum_{t=1}^T B_vC_1\sqrt{\sum_{i \in S_t}\frac{\norm{\tilde{\btheta}_t-\btheta^{*}}_{\bG_t}^2\norm{ \bphi_t(i)}_{\bG_t^{-1}}^2}{\bar{\sigma}_i^2}} 	& \mbox{Cauchy–Schwarz Inequality}\\
   &\le\sum_{t=1}^T B_vC_1\sqrt{\beta\sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}} 	& \mbox{the definition of $C_t^{\theta}$}\\
   & \le B_vC_1\sqrt{\beta}\sqrt{T\sum_{t=1}^T \sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}} 	& \mbox{Cauchy–Schwarz Inequality over $t$}\\
   & \le B_vC_1d\sqrt{T}\log T,
 \end{align}
 where the last inequality uses $\beta \le \tilde{O}(d\log (KT))$ (Theorem 3~\cite{zhou2021nearly}), and the potential lemma $\sum_{t=1}^T \sum_{i \in S_t}{\norm{ \bphi_t(i)/\bar{\sigma}_i}_{\bG_t^{-1}}^2}\le \tilde{O}(d\log (KT))$ (Eq. (44)~\cite{zhou2021nearly}).
 
 Intuitively, the source of improvement comes from the saving of one use of Cauchy-Schwarz from the 1-norm TPM condition from \cref{apdx_eq: linear_use_cond_VM}: 
 \begin{align}
      Reg(T)&\le\sum_{t=1}^T B_1 \sum_{i \in S_t}\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}\\
     &\le \sum_{t=1}^T B_1 \sqrt{ K\sum_{i \in S_t}\inner{\tilde{\btheta}_t-\btheta^{*}, \bphi_t(i)}^2}
 \end{align}

\subsection{Unknown Variance}
% \begin{algorithm}[h]
% 	\caption{BC$^2$UCB: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Unknown Variance but with Monotonicity Assumption}\label{alg:BC^2UCB-T}
% 			\resizebox{.99\columnwidth}{!}{
% \begin{minipage}{\columnwidth}
% 	\begin{algorithmic}[1]
% 	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, computation oracle ORACLE.
% 	   % \OUTPUT Budget allocation $\bk$.
% 	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0},$ optimistic variance $\bv_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
% 	   \For{$t=1, ...,T$ }
% 	   \State Compute empirical estimator $\btheta_{t}=\bG_t^{-1}\bb_t$.
% 	   \State Construct two confidence sets, one for decision and one for the variance, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$, $C^{v}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\}$.
% 	   %\State $G_t=\lambda \boldsymbol{I} + \sum_{\tau < t}\bphi(i)\bphi(i)^{\top}$.
% 	   %$\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1, i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.
% 	   %\State Set UCB value $\bar{\mu}_{t,i}=\min \{\hat{\mu}_{t-1, i}+\rho_{t, i},1\}$.
% 	   \For{$i \in [m]$}
% 	   \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}} + 2\sqrt{\beta}\norm{\phi_{i}}_{\bG_t}$. // optimistic mean, double radius
% 	   \State $\ubar{\mu}_{t,i}=\inner{\bphi_t(i), \hat{\btheta}} - 2\sqrt{\beta}\norm{\phi_{i}}_{\bG_t}.$
% 	   \State Compute the optimistic variance by solving $\max_{\bnu \in C^{v}_t}{\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})}$ \begin{equation}
%     v_{t,i}= \begin{cases}
% (1-\bar{\mu}_{t,i})\bar{\mu}_{t,i}, &\text{if $\bar{\mu}_{t,i} \le \frac{1}{2}$}\\
% (1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}, &\text{if $\ubar{\mu}_{t,i} \ge \frac{1}{2}$}\\
% \frac{1}{4}, &\text{otherwise}.
% \end{cases}
% \end{equation} 
% \State Let $ \tilde{\bnu}_{t}(i), \tilde{\mu}_{t,i}$ are parameters that achieve $v_{t,i}$.
% 	   \EndFor
% 	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. 
% 	    \For{$ i \in S_t$ }
% 	   \State $\bG_t\pluseq v_{t,i}^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
% 	   \State $\bb_t\pluseq v_{t,i}^{-1}\bphi_{t}(i) X_{t,i}$.
% 	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
% 	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
% 	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
% 	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
% 	   % \label{line:trigger_upd}
% 	   \EndFor
% 	    	   \EndFor
% 		\end{algorithmic}
%           		\end{minipage}}
% \end{algorithm}

\begin{algorithm}[h]
	\caption{BC$^2$UCB-T: Bernstein Contextual Combinatorial Upper Confidence Bound Algorithm for Non-triggering CMAB with Unknown Variance but with Monotonicity Assumption}\label{alg:BC^2UCB-T}
			\resizebox{.99\columnwidth}{!}{
\begin{minipage}{\columnwidth}
	\begin{algorithmic}[1]
	    \State {\textbf{Input:}} Base arms $[m]$, dimension $d$, regularizer $\lambda$, exploration parameter $\beta$, computation oracle ORACLE.
	   % \OUTPUT Budget allocation $\bk$.
	   \State \textbf{Initialize:} Empirical mean $\hat{\btheta}_0=\boldsymbol{0},$ optimistic variance $\bv_0=\boldsymbol{0}$, Gram matrix $\bG_{0}=\lambda\boldsymbol{I}$, regressand $\bb_{0}=\boldsymbol{0}$. 
	   \For{$t=1, ...,T$ }
	   \State $\hat{\btheta_{t}}=\bG_{t-1}^{-1}\bb_{t-1}$. \Comment{Compute empirical estimator.}
	   %\State Construct two confidence sets, one for decision and one for the variance, $C^{\theta}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le \beta\}$, $C^{v}_t=\{\bnu: \norm{\bnu-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\}$.
	   \For{$i \in [m]$}
	   \State $\bar{\mu}_{t,i} = \inner{\bphi_t(i), \hat{\btheta}_t} + 2\sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}$.  \Comment{UCB value for arm $i$.}
	   \State $\bar{\mu}_{t,i}=\min \{\bar{\mu}_{t,i},1\}$.
	   \State $\ubar{\mu}_{t,i}=\inner{\bphi_t(i), \hat{\btheta}_t} - 2\sqrt{\beta}\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}}.$ \Comment{LCB value for arm $i$.}
	   \State $\ubar{\mu}_{t,i}=\max\{\ubar{\mu}_{t,i},0\}$.
	   %\State Compute the optimistic variance by solving $\max_{\bnu \in C^{v}_t}{\inner{\bphi_t(i), \bnu}(1-\inner{\bphi_t(i), \bnu})}$     
	   \State\begin{equation}\label{eq:var_upper}
 \bar{V}_{t,i}= \begin{cases}
(1-\bar{\mu}_{t,i})\bar{\mu}_{t,i}, &\text{if $\bar{\mu}_{t,i} \le \frac{1}{2}$}\\
(1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}, &\text{if $\ubar{\mu}_{t,i} \ge \frac{1}{2}$}\\
\frac{1}{4}, &\text{otherwise}.
\end{cases}
\end{equation} \Comment{Upper bound of the variance $V_i=(1-\mu_i)\mu_i$.}
% \State Let $ \tilde{\bnu}_{t}(i), \tilde{\mu}_{t,i}$ are parameters that achieve $v_{t,i}$.
	   \EndFor
	   \State $S_t=\text{ORACLE}(\bar{\mu}_{t,1}, ..., \bar{\mu}_{t,m})$. \Comment{Computational oracle using UCBs.}
	    \For{$ i \in \tau_t$ }\Comment{Update statistics.}\label{line:update_G}
	   \State $\bG_t=\bG_{t-1}+ \bar{V}_{t,i}^{-1}\bphi_{t}(i)\bphi_{t}(i)^{\top}$.
	   \State $\bb_t=\bb_{t-1}+ \bar{V}_{t,i}^{-1}\bphi_{t}(i) X_{t,i}$.\label{line:update_b}
	   %\State Play $S_t$, which triggers arms $\tau_t \subseteq [m]$ with outcome $X_{t,i}$'s, for $i \in \tau_t$.\label{line:trigger_obs}.
	   % \State For every $i \in \tau_t$, update $T_{t,i}= T_{t-1, i}+1$, $\hat{\mu}_{t,i}= \hat{\mu}_{t-1,i}+(X_{t,i}-\hat{\mu}_{t-1,i})/T_{t,i}$,
	   %% $\hat{V}_{t, i}=\frac{T_{t-1, i}(\hat{V}_{t-1,i}+\hat{\mu}_{t-1}^2)+X_{t,i}^2}{T_{t, i}} -\hat{\mu}_{t,i}^2$. 
	   %$\hat{V}_{t, i}= \frac{T_{t-1, i}}{T_{t, i}}\left(\hat{V}_{t-1,i} + \frac{1}{T_{t, i}} \left(\hat{\mu}_{t-1,i} - X_{t,i}\right)^2\right) $.
	   % \label{line:trigger_upd}
	   \EndFor
	    	   \EndFor
		\end{algorithmic}
           		\end{minipage}}
\end{algorithm}

As in \cref{alg:BC^2UCB-T}, for each arm $i$, we use $\bar{V}_{t,i}$ as an optimistic estimation of the variance. Indeed, $\bar{V}_{t,i}$ is the optimal value of the following problem, 
\begin{align}\label{eq:var_upper_explain}
\max_{\btheta \in C_t}{f_{t,i}(\btheta)=\inner{\bphi_t(i), \btheta}(1-\inner{\bphi_t(i), \btheta})}
\end{align}
where $C_t=\left\{\btheta: \norm{\btheta-\hat{\btheta}_t}_{\bG_{t-1}}^2 \le 4\beta\right\}$ is the confidence ellipsoid for $\btheta^{*}$. To see why $\bar{V}_{t,i}$ takes the closed form as in \cref{eq:var_upper}, consider $f_{t,i}(x)=x(1-x)$ as a quadratic function of $x=\inner{\bphi_t(i), \btheta} \in [\ubar{\mu}_{t,i},\bar{\mu}_{t,i}]$. If $0.5 \in  [\ubar{\mu}_{t,i},\bar{\mu}_{t,i}]$, else if $\bar{\mu}_{t,i}\le 0.5$, max value is $\bar{\mu}_{t,i}(1-\bar{\mu}_{t,i})$, else if $\ubar{\mu}_{t,i} \ge 0.5$, max value is $(1-\ubar{\mu}_{t,i})\ubar{\mu}_{t,i}$.

For notational convenience, we use $\tilde{\mu}_{t,i}=\argmax_{x} f_{t,i}(x)$ and $\bar{\bnu}_t(i)=\argmax_{\btheta}f_{t,i}(\theta)$ at round $t$ for arm $i$ as in \cref{eq:var_upper_explain}. Note that $\inner{\bphi_t(i),\bnu_t(i)}=\tilde{\mu}_{t,i}$. We also denote $\bar{\btheta}_{t}(i)$ be the vector that $\inner{\bphi_t(i),\bar{\btheta}_{t}(i)}=\bar{\mu}_{t,i}$.

\begin{align}
    &Reg(T)=\sum_{t=1}^T  r(S_t^*; \bmu)- r(S_t; \bmu)\\
    &\le \sum_{t=1}^T  r(S_t; \bar{\bmu}_{t})- r(S_t; \bmu) \\
    &\le \sum_{t=1}^T \abs{r(S_t; \bar{\bmu}_{t}) - r(S_t;\tilde{\bmu}_{t})} +\abs{ r(S_t; \tilde{\bmu}_t) - r(S_t; \bmu)}\\
    % & \mbox{$\tilde{\mu}_{t,i}, \tilde{\bnu}_{t}(i)$ are para. that achieve $v_{t,i}$}\\
    &\le\sum_{t=1}^T B_v \sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\bnu}_{t}(i)-\bar{\btheta}_{t(i)}, \bphi_t(i)}^2}{\bar{V}_{t,i}}} + B_v \sqrt{\sum_{i \in S_t}\frac{\inner{\tilde{\bnu}_{t}(i)-\btheta^*, \bphi_t(i)}^2}{\bar{V}_{t,i}}}& \mbox{(Apply \Cref{cond:VM} twice)}\\
    &\le\sum_{t=1}^T 2B_v \sqrt{\beta\sum_{i \in S_t}{\norm{ \bphi_t(i)/\sqrt{\bar{V}_{t,i}}}_{\bG_{t-1}^{-1}}^2}}  \\
    &\le  B_vd\sqrt{T}\log T 
\end{align}
\begin{remark}
The intuition of using variance is from the exploitation perspective: the smaller the variance, the more accurate the data point is, and thus more important for the agent to learn unknown $\btheta$. So we use the inverse of $\bar{V}_{t,i}$ in \cref{line:update_G} and \cref{line:update_b} to re-weight the observation.
\end{remark}

\subsection{Lower Bound for Contextual CMAB with Linear Reward}
Consider a $KT$ round linear bandit with $2^d$ feature vectors $\bx_t(i)\in\{-1,1\}^d$ and $\Theta=\{-1/\sqrt{T}, 1/\sqrt{T}\}$, each base arm's reward is $X_{t,i}==\inner{\bx_t(i), \btheta^*} + \eta_{t,i}$, where $\eta_{t,i}$ are independent. Then for any policy there exists a vector $\theta\in \Theta$ such that $R_T(A,\theta)\ge \Omega(d\sqrt{T})$ by Theorem 24.1 \cite{lattimore2020bandit}. For $KT$ rounds, if the algorithm can adaptively update each base arm observation, the regret is $\Omega(d\sqrt{KT})$.

\begin{remark}
Compared with the tabular case with independent base arms, where ESCB work~\cite{combes2015combinatorial} gives $\tilde{\Theta}(\sqrt{dT})$ regret, the lower bound of contextual CMAB has a $\sqrt{dK}$ gap. This gap comes from the fact that in the tabular case, base arms are independent and the feature vectors are orthogonal. In particular, the $\sqrt{d}$ term comes from the confidence coefficient $\beta$, where ESCB has order $\beta={O}(\sqrt{d+\log T})$, while LinUCB gives $\beta=\sqrt{d{\log T}}$ (though for fix-design actions, this can be relaxed in Eq. (20.3) to $\beta={O}(\sqrt{d+\log T})$~\cite{lattimore2020bandit}). The $\sqrt{K}$ term comes from that the arm feature vector in contextual CMAB could lie in the same direction (or exactly the same vector), and prevents the $\sqrt{K}$ improvement from ESCB.
\end{remark}

\subsection{Bandit Feedback is Sufficient to Match the Lower Bound}
Let $\Phi_t(S_t)=\sum_{i \in S_t}\bx_t(i)$, the reward $Y_t(S_t; \btheta)=\inner{\btheta, \Phi_t(S_t)} + \sum_{i \in S_t}\eta_t(i)$, which is a $\sqrt{K}$-subGaussian random variable. Following the linear bandit algorithm, we use pair oracle to select $\Phi_t(S_t)$ based on confidence ball $C_t$, the regret is $O(d\sqrt{KT})$~\cite{abbasi2011improved}.

\subsection{Contextual CMAB with Triggering Arms}
% Suppose we consider a simpler case, where $\bx_t$ is the context at round $t$, and $\E[\mu_a|\bx_t]=\inner{\bx_t, \theta_a}$. The triggered arms are $\tilde{S}_t$.

We start with the 1-norm TPM condition, and we have the following construction of the gram matrix and the $b$-value. For each round,

\begin{align}
    \bG_t&=\bG_{t-1}+\I\{i \in \tilde{A}_t\}\bphi_{t(i)}\bphi_{t(i)}^T.\\
    \bb_t&=\bb_{t-1}+\I\{i \in \tilde{A}_t\}\bphi_{t(i)}X_{t,i}.\\
    \hat{\btheta}_t&=\bG_{t-1}^{-1} \bb_{t-1}.
\end{align}

% \begin{align}
%     \tilde{G}_i(t)&=\tilde{G}_i(t-1)+p_i^{D,S_t}\bx_t^T \bx_t.\\
%     \tilde{b}_i(t)&=\tilde{b}_i(t-1)+p_i^{D,S_t}\bx_t r_t.\\
%     \hat{\btheta}_i(t)&=\tilde{G}_i(t)^{-1} \tilde{b}_i(t).
% \end{align}

Now for the regret, suppose $\alpha=\beta=1$, $\Delta_{S_t}=r(S_t^*;\btheta^*, \phi_t)-r(S_t;\btheta^*,\phi_t)$
\begin{align}
    Reg(T)&=  \E\left[\sum_{t=1}^T\Delta_{S_t}\right]\\
    &\le \E\left[\sum_{t=1}^T\sum_{i \in [m]}B_1p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)\right]\\
    &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1\E_{\tau_t}[\I\{i \in \tilde{A}_t\}](\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in [m]}B_1\I\{i \in \tilde{A}_t\}(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\\
     &=\E\left[\sum_{t=1}^T\E\left[\sum_{i \in \tilde{A}_t}B_1(\bar{\mu}_{t,i}-\mu_i)\mid \cF_{t-1}\right]\right]\label{eq:trigger_prob_ieq}
\end{align}

For \cref{eq:trigger_prob_ieq}, it equals to the following,
\begin{align}
    &\E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}B_1(\bar{\mu}_{t,i}-\mu_i)\right]\\
    &\le \E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}B_1(\norm{\bar{\btheta}_t-\btheta^{*}}_{\bG_{t-1}}\cdot \norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}})\right]\\
    &\le B_1\sqrt{\beta}\E\left[\sum_{t=1}^T\sum_{i \in \tilde{A}_t}(\norm{\bphi_{t}(i)}_{\bG_{t-1}^{-1}})\right]\\
    &\le B_1\sqrt{\beta}\E\left[\sqrt{KT \sum_{t=1}^T\sum_{i \in \tilde{A}_t}(\norm{\bphi_{t}(i)}^2_{\bG_{t-1}^{-1}})}\right]\\
    &\le B_1 \sqrt{d\log T} \sqrt{KT d\log(KT)}=B_1 d \sqrt{KT}\log(KT)
\end{align}
This gives the Contextual CMAB-T version under 1-norm TPM condition, which extends \citet{li2016contextual}.

Now if we use TPVM condition (and ignore $(1-\mu_i)\mu_i$ term for now), similarly, the regret is bounded by,
\begin{align}
     Reg(T)&=  \E\left[\sum_{t=1}^T\Delta_{S_t}\right]\\
    &\le \E\left[\sum_{t=1}^T B_v\sqrt{\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2}\right]\\
    &\le \E\left[ B_v\sqrt{T\sum_{t=1}^T\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2}\right]\\
    &\le B_v\sqrt{T} \sqrt{\E\left[\sum_{i \in [m]}p_i^{D,S_t}(\bar{\mu}_{t,i}-\mu_i)^2\right]}\\
    &\le B_v\sqrt{T} \sqrt{\E\left[\sum_{t \in T}\sum_{i \in \tilde{A}_t}(\bar{\mu}_{t,i}-\mu_i)^2\right]}\\
    &\le B_v\sqrt{\beta}\sqrt{T} \sqrt{\E\left[\sum_{t \in T}\sum_{i \in \tilde{A}_t}(\norm{\bphi_t(i)}_{\bG_{t-1}^{-1}}^2\right]}\\
    &\le d\sqrt{T}\log(KT).
\end{align}

This improves the Contextual CMAB-T with $\sqrt{K}$ factor under TPVM condition.


% For the regret, if we apply 1-norm bounded smoothness, we would have
% \begin{align}
%     Reg(T)&\le B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}( \bar{\mu}_{t,i}-\mu_i)\\
%     &\le  B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\inner{\bx_t,\bar{\theta}_i(t)-\theta_i}\\
%     &\le  B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\norm{\bx_t}_{G_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{G_i(t)}
% \end{align}
% If the last line is $B_1\sum_{t}\sum_{i \in \tilde{S}_t}p_i^{D,S_t}\norm{\bx_t}_{\tilde{G}_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{\tilde{G}_i(t)}$, we can use $\tilde{\bx}_t=\sqrt{p_i^{D,S_t}}$ and prove the result using \begin{align}
%     &B_1\sum_{t}\sum_{i \in \tilde{S}_t}\norm{\tilde{\bx}_t}_{\tilde{G}_i^{-1}(t)}\cdot \norm{\bar{\theta}_i(t)-\theta_i}_{\tilde{G}_i(t)}\\
%     &\le B_1\sqrt{\beta} \sum_{i \in [m]}\sum_{t: i \in \tilde{S}_t} \sqrt{d N_i(T)\log T}\le B_1d\sqrt{\sum_{a}N_i(T)}\sqrt{\sum_{i} 1}\le B_1d\sqrt{mKT}.
% \end{align} However, we can only use $G_i(t)$, where $E[G_i(t)]=\tilde{G}_i(t)$? Or there is no difference?


\subsection{Technical Lemmas}

\begin{lemma}[Ellipsoidal potential lemma, \cite{abbasi2011improved}] Let $\bx_1,...,\bx_n$ be a sequence of vectors with $\norm{\bx_t}_2^2$, and let $G_t=I+\sum_{s=1}^{t-1}\bx_s \bx_s^T$. Then $\sum_{t=1}^n\min\{1,\norm{\bx_t}^2_{G_{t-1}^{-1}}\}\le 2 d \log (1+\frac{cn}{d}).$
\end{lemma}

\begin{lemma}[Theorem 3, \cite{lattimore2015linear}]
Let $\lambda>0, \delta=1/(TK), N=(4T^4d^2)^d, B\ge \max_{k}\norm{\btheta^*}_2^2,$ so that $\beta=(1+\sqrt{\alpha}+2\sqrt{\log\left(\frac{6TN}{\delta}\log\left(\frac{3TN}{\delta}\right)\right)})=O(\sqrt{d\log T})$. We have $\norm{\hat{\btheta}-\btheta_t}_{\bG_{t-1}}^2\le \beta$ for all $t\le T$ with probability at least $1-\delta=1$. 
\end{lemma}


\subsection{Next Steps}
\begin{enumerate}
    \item Plug in the details of the regret analysis (triggering \& variance parts).
    \item Check improved (?) analysis for 1-norm TPM condition without triggering groups.
    \item Check relation between the proof with pair oracles (Shuai's paper) and the proof with standard oracles (ours).
    \item Check upper and lower bound discussion (indicating whether or not our result is tight).
    \item Applications, e.g., cascading bandits, PMC, and rank-1 influence maximization.
\end{enumerate}
% \begin{itemize}
%     \item Confidence set and potential lemma for the unknown variance.
%     \item C$^2$MAB-T and triggering arms, one related RL paper using the peeling technique~\cite{he2021logarithmic}. Another work by \citet{demirel2021combinatorial} also considers TPM condition, where they use pseudo information gain to deal with the triggering arms.
%     \item Empirical Bernstein Inequality for self-normalized process, similar to the tabular case~\cite{audibert2009exploration}.
%     \item \sout{Lower bound for \citet{takemura2021near} is probably incorrect}.
%     \item Lower bound for contextual TPVM.
% \end{itemize}

==> content/acknowledgement.tex <==
\section{Acknowledgement}
The work of John C.S. Lui was supported in part by the GRF 14200420.

==> content/algorithm.tex <==






==> content/analysis.tex <==
%%\OnlyInFull{\vspace{-5pt}}
% \section{Regret Analysis for CMAB-T with Gini-smoothness}\label{sec: online learning}
\ts{Construction principle of the confidence radius}
\begin{lemma}[Empirical Bernstein Inequality]\label{lem:empirical_bern} (\cite{audibert2009exploration}) Let $(X_i)_{i \in [n]}$ be $n$ i.i.d random variables with bounded support $[0,1]$ and mean $\E[X_i]=\mu$. Let $\hat{X}_n$ and $\hat{V}_n$ be the empirical mean and empirical variance of $(X_i)_{i \in [n]}$. Then for any $n \in \mathbb{N}$ and $y > 0$, it holds that
\begin{equation}
    \Pr\left[|\hat{X}_n-\mu| \ge \sqrt{\frac{2\hat{V}_n y}{n}} + \frac{3y}{n}\right] \le 3 e^{-y}
\end{equation}
\end{lemma}

By setting $y=3\log t$ and $n = T_{t-1, i}$, the construction of confidence radius for base arm $i$ is then $\rho_{t,i}=\sqrt{\frac{6\hat{V}_{t-1,i} \log t}{T_{t-1, i}}} + \frac{9\log t}{T_{t-1, i}}$.

To prove the regret bound, we have the following lemma to upper bound the empirical variance with high probability.
\begin{lemma} Let $\hat{V}_n$ be the empirical variance of $n$ i.i.d random variables with support $[0,1]$ and mean $\E[X_i]=\mu$. Then, it holds that
\begin{equation}\label{lem:bounded_var}
    \Pr\left[\hat{V}_n \le 2\mu(1-\mu) +  \frac{7\log (1/\delta)}{6n}\right] \le 1-\delta.
\end{equation}
\end{lemma}

Combining \cref{lem:empirical_bern} and \cref{lem:bounded_var}, it holds that
\begin{equation}
     \mu_{i} \le \bar{\mu}_{t,i} \le\mu_{i} + 2 \rho_{t,i} \le  \mu_{t-1,i} + 4\sqrt{3}\sqrt{\frac{\mu_i(1-\mu_i) \log t}{T_{t-1, i}}} + \frac{34\log t}{T_{t-1, i}}.
\end{equation}

Let $\bar{\bmu}_{t}=(\bar{\mu_{t,i}}_{i \in [m]})$ and $\bar{M}=\sum_{j \in [M]}w_j$, we can derive that
\begin{align*}
    \alpha r(S^*; \bmu) &\le \alpha r(S^*; \bar{\bmu}_t) \le r(S_t; \bar{\bmu}_t)=\sum_{j \in [M]}w_j r_j(S_t;\bar{\bmu}_t)\\
    &\le \sum_{j \in [M]} w_j \left(r_j(S_t;\bmu) + 4\sqrt{3}B_g\sqrt{\sum_{i\in [m]}\frac{ \log t}{T_{t-1, i}}} + 34B_1\sum_{i \in [m]}\frac{\log t}{T_{t-1, i}}\right)\\
    &=r(S_t;\bmu) + \bar{M}\left(4\sqrt{3}B_g\sqrt{\sum_{i\in [m]}\frac{ \log t}{T_{t-1, i}}} + 34B_1\sum_{i \in [m]}\frac{\log t}{T_{t-1, i}}\right)
\end{align*}

% \ts{The motivation and the definition of the event-filtered regret.}

% The regret analysis of CMAB-T with Gini-smooth reward functions relies on a series of high probability events.
% Specifically, at round $t$, we will divide the probability space for this round into (perhaps infinitely many) mutually exclusive and exhaustive events.
% We then separately bound the regret filtered by the above events and sum them together to bound the total regret.
% Formally, we give the following definition for the event-filtered regret.
% \begin{definition}[Event-filtered regret]
% For any series of events $(E_t)_{t \ge 1}$ indexed by round number $t$, the regret filtered by events $(E_t)_{t \ge 1}$ is defined as,
% \begin{equation}
%     Reg(T, (E_t)_{t \ge 1}; \alpha, \bmu)=\E\left[\sum_{t=1}^T \I(E_t) \left(\alpha r(S^*;\bmu)-r(S_t; \bmu)\right)\right].
% \end{equation}
% \end{definition}
% Note that the event filtered regret is only counted when $E_t$ happens at round $t$ and we will simply write $Reg(T, (E_t)_{t \ge 1}; \alpha, \bmu)$ as $Reg(T, E_t)$ when contexts are clear.

\begin{definition}[(Approximation) gap]
Fix a distribution $D$ and its mean vector $\bmu$. For each action $S$, we define the (approximation) gap as $\Delta_S=\max\{0, \alpha r(S^*;\bmu)-r(S;\bmu)\}$. For each arm, we define



\end{definition}
\ts{Event 1: $\Delta_{S_t} \le E_t$.}

We first use $(\lambda, B_1, B_g)$ TPM Gini-smoothness and derive the regret form filtered by the event $E_t = \{\Delta_{S_t} \le e_t(S_t)\}$, where the error term $e_t$ is shown in the following lemma. 
\begin{restatable}{lemma}{error_term}[TPM gini-smooth error term]
Let $r(S;p)$ be Gini-smooth functions with coefficients $(B_1,B_g,\lambda)$, and define the error term
\begin{align}
        e_t(S_t)&=12\sqrt{6}B_g\sqrt{\sum_{i\in \tilde{S}_t}(\frac{\log t}{T_{t-1,i}}\wedge 1)(p_{i}^{D,S_t})^\lambda} + 34B_1\sum_{i \in \tilde{S}_t}(\frac{\log t}{T_{t-1,i}}\wedge 1)(p_{i}^{D,S_t}).
\end{align}
The regret of Algorithm~\ref{alg:BCUCB-T}, when used with $(\alpha, \beta)$ approximation oracle is bounded by 
\begin{equation}\label{eq:e_t}
    Reg(T) \le \E[\sum_{t=L+1}^T\Delta_{S_t}\I\{\Delta_{S_t} \le Me_t(S_t)\}] + L \Delta_{\max}(1+M \frac{2\pi^2}{3}).
\end{equation}  

\end{restatable}
Following this lemma, we give the regret bound in the following main theorem.

% \ts{Event 2: $E_t$ can be further decomposed by infinitely many mutually exclusive and exhaustive events.}

% For $e \in \{e_1, e_2\}$, let $\alpha_{1,e} > \alpha_{2,e} > ... > \alpha_{k,e} > ...$ and $1=\beta_{0,e} > \beta_{1,e} > ... > \beta_{k,e} > ...$ be two infinite number sequences that are positive and decreasing.

% Define $A_{k,e}^{S_t}=\{i \in \tilde{S}_t: N_{i,j_i^{S_t}, t-1} \le \alpha_{k,e} \frac{g_e(m, \Delta_{S_t})f(t)}{\Delta_{S_t}^2}, j_i^{S_t} \le j_{i,e}^{\max}\}=\{i \in \tilde{S}_t \cap O_{S_{t,e}}: N_{i,j_i^{S_t}, t-1} \le \alpha_{k,e} \frac{g_e(m, \Delta_{S_t})f(t)}{\Delta_{S_t}^2}  \}$ the set of base arms whose counter is small and triggering probability is not small.

\ts{Regret bound.}
Let $c_1=12\sqrt{6}, c_2=34$.

\begin{restatable}{theorem}{lambda2}
When the reward function $r(S;p)$ is $(B_1,B_g,\lambda)$ Gini-smooth and $\lambda > 1$, the total regret is bounded by
\begin{equation}
    \left[ \sum_{i=1}^m\frac{2880c_1^2}{1-2^{-(\lambda-1)}}\frac{ \bar{M}^2B_{g}^2}{\Delta_{i}^{\min}} +\sum_{i=1}^m\left(720c_2\log\frac{4c_2B_1 K}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{\Delta_{i}^{\max}}{\Delta_{i}^{\min}}\right)B_1\bar{M}  \right] \left(\log K\right)^2\log T
\end{equation}
Reverse amortization:
\begin{equation}
    \left[ \sum_{i=1}^m\frac{288c_1^2}{1-2^{-(\lambda-1)}}\frac{ \bar{M}^2B_{g}^2}{\Delta_{i}^{\min}} (3+\log K)  +\sum_{i=1}^m\left(144c_2\bar{M}B_1\log\frac{4c_2\bar{M}B_1 K}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{\Delta_i^{\max} K}{\Delta_{i}^{\min}}\right) \right] \log T
\end{equation}
\end{restatable}

\begin{restatable}{theorem}{lambda2}
When the reward function $r(S;p)$ is $(B_1,B_g,\lambda)$ Gini-smooth and $\lambda = 1$, the total regret is bounded by
\begin{equation}
    O\left(\left[ \sum_{i=1}^m \left(\log\frac{8c_1^2\bar{M}^2B_{g}^2 K}{(\Delta_{i}^{\min})^2}\right)\frac{2880c_1^2}{\Delta_{i}^{\min}} \bar{M}^2B_{g}^2 +\sum_{i=1}^m\left(720c_2\log\frac{4c_2B_1\bar{M} K}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{\Delta_{i}^{\max}}{\Delta_{i}^{\min}}\right)B_1  \right] \left(\log K\right)^2\log T\right)
\end{equation}
Reverse amortization:
\begin{equation}
    O\left(\left[ \sum_{i=1}^m \left(\log\frac{8c_1^2\bar{M}^2B_{g}^2 K}{(\Delta_{i}^{\min})^2}\right)\frac{288c_1^2}{\Delta_{i}^{\min}}\bar{M}^2 B_{g}^2 (3+\log K)  +\sum_{i=1}^m\left(144c_2\bar{M}B_1\log\frac{4c_2\bar{M}B_1 K}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{\Delta_i^{\max} K}{\Delta_{i}^{\min}}\right) \right]\log T\right)
\end{equation}
\end{restatable}




==> content/application_proof.tex <==
\section{Proof of TPVM Smoothness Conditions for Various Applications (Related to Theorem \cref{lem:app_tab})}\label{apdx_sec:proof_app}
For convenience, we show our table again in this section.
        \begin{table*}[h]
	\caption{Summary of the coefficients, regret  bounds and improvements for various applications.}	\label{tab:app_restate}	
		\resizebox{1.00\columnwidth}{!}{
	\centering
	\begin{threeparttable}
	\begin{tabular}{|ccccc|}
		\hline
		\textbf{Application}&\textbf{Condition}& \textbf{$(B_v, B_1, \lambda)$} & \textbf{Regret}& \textbf{Improvement}\\
	\hline

		Disjunctive Cascading Bandits~\citep{kveton2015combinatorial} & {\TPVMm} & $(1,1,2)$ & $O(\sum_{i \in [m]}\frac{\log K\log T}{\Delta_i^{\min}})$ & $O(K/\log K)$ \\
			\hline
% 			\rowcolor{LightGray}
		Conjunctive Cascading Bandits~\citep{kveton2015combinatorial} & TPVM & $(1,1,1)$ & $O( \sum_{i \in [m]}\log \frac{K}{\Delta_{\min}}\frac{ \log K\log T}{\Delta_{i,\min}})$ & $O(K/(\log K\log \frac{K}{\Delta_{\min}}))$\\
			\hline
		Multi-layered Network Exploration~\citep{liu2021multi} & TPVM & $(\sqrt{1.25|V|},1,2)$ $^\dagger$ & $O(\sum_{i \in \cA}\frac{|V|\log (n|V|)\log T}{\Delta_i^{\min}})$ & $O(n/\log (n|V|))$\\
			\hline
				% \rowcolor{LightGray}
% 			Influence Maximization on TPG \cite{wang2017improving} & TPVM & $(\sqrt{2}|V|,|V|,1)$ & $O( \sum_{i \in [m]}\log \frac{|E|}{\Delta_{\min}}\frac{|V|^2\log |E| \log T}{\Delta_i^{\min}})$  & $O(|E|/(\log |E|\log \frac{|E|}{\Delta_{\min}}))$\\
				% \hline
	    Influence Maximization on DAG \cite{wang2017improving} & {\TPVMm} &$(\sqrt{L}|V|,|V|,1)$ $^{\dagger}$  & $O( \sum_{i \in [m]}\log \frac{|E|}{\Delta_{\min}}\frac{L|V|^2\log |E| \log T}{\Delta_i^{\min}})$ & $O(|E|/(L\log |E|\log \frac{|E|}{\Delta_{\min}}))$\\
	    \hline
	   % 	\rowcolor{LightGray}
	    Probabilistic Maximum Coverage \cite{merlis2019batch}$^*$ & VM & $(3\sqrt{2|V|},1,-)$ & $O(\sum_{i \in [m]}\frac{|V|\log T}{\Delta_i^{\min}})$ & $O(\log^2 k)$.\\
	    \hline
	\end{tabular}
	  \begin{tablenotes}[para, online,flushleft]
	\footnotesize%\smallskip
	\item[]\hspace*{-\fontdimen2\font}$^*$ This row is for the application in \cref{sec:independent} and the rest of rows are for \cref{sec:TPVM}; 
	\item[]\hspace*{-\fontdimen2\font}$^{\dagger}$ $|V|, |E|, n, k, L$ denotes the number of target nodes, the number of edges that can be triggered by the set of seed nodes, the number of layers, the number of seed nodes and the length of the longest directed path, respectively.
% 	\item[]\hspace*{-\fontdimen2\font}$^\ddagger$ $|V|, |E|, n, |L|$ denotes the number of layers, the number of longest;
% 	\item[]\hspace*{-\fontdimen2\font}$^\ddagger$ $L$ is the number of ;
% 	\item[]\hspace*{-\fontdimen2\font}$^{\S}$ This work gives sufficient smoothness condition with factor $\gamma_g$ and translates to $B_v=3\sqrt{2}\gamma_g$ in our setting.
	\end{tablenotes}
			\end{threeparttable}
	}
\end{table*}


\subsection{Combinatorial cascading bandits}
Combinatorial cascading bandits has two categories: conjunctive cascading bandits and disjunctive cascading bandits~\cite{kveton2015combinatorial}.



\textbf{Disjunctive form}
For the disjunctive form, we want to select an ordered list $S$ of $K$ items from total $L$ items, so as to maximize the probability that at least one of the outcomes of the selected items are $1$.
Each item is associated with a Bernoulli random variable with mean $\mu_i$, indicating whether the user will be satisfied with the item if he scans the item.
This setting models the movie recommendation system where the user sequentially scans a list of recommended items and the system is rewarded when the user is satisfied with any recommended item.
After the user is satisfied with any item or scans all $K$ items but is not satisfied with any of them, the user leaves the system.
Due to this stopping rule, the agent can only observe the outcome of items until (including) the first item whose outcome is $1$. If there are no satisfactory items, the outcomes must be all $0$. In other words, the triggered set is the prefix set of items until the stopping condition holds.
For this application, we have the following lemma. 

\begin{lemma}\label{lem:app_cas_dis}
Disjunctive conjunctive cascading bandit problem satisfies {\TPVMm} bounded smoothness condition with coefficient $(B_v,B_1,\lambda)=(1,1,2)$.
\end{lemma}

\begin{proof}
Without loss of generality, let the action be $\{1,...,K\}$, then the reward function is $r(S;\bmu)=1-\prod_{j=1}^K(1-\mu_j)$ and the triggering probability is $p_{i}^{D,S}=\prod_{j=1}^{i-1}(1-\mu_j)$.
Let $\bar{\bmu}=(\bar{\mu}_1, ..., \bar{\mu}_K)$ and $\bmu=(\mu_1, ..., \mu_K)$, where $\bar{\bmu}=\bmu+\boldzeta + \boldeta$ with $\bar{\bmu}, \bmu \in (0,1)^K, \boldzeta, \boldeta \in [0,1]^K$.
\begin{align}
    &\abs{r(S;\bar{\bmu})-r(S;\bmu)}\notag\\
    &=\prod_{i=1}^K(1-\mu_i)-\prod_{i=1}^K(1-\bar{\mu}_i)\label{apdx_eq:cas_dis_mono}\\
    &=\sum_{i \in [K]} (\bar{\mu}_i-\mu_i)((1-\mu_1)...(1-\mu_{i-1}) (1-\bar{\mu}_{i+1})...(1-\bar{\mu}_{K}))\label{apdx_eq:cas_dis_tlscp}\\
    &=\sum_{i \in [K]} (\zeta_i+\eta_i)((1-\mu_1)...(1-\mu_{i-1}) (1-\bar{\mu}_{i+1})...(1-\bar{\mu}_{K}))\label{apdx_eq:cas_dis_def_zeta}\\
    &\le \sum_{i \in [K]} (\zeta_i)((1-\mu_1)...(1-\mu_{i-1})(1-\mu_{i+1})...(1-\mu_{K})) +  \sum_{i \in [K]} (\eta_i)((1-\mu_1)...(1-\mu_{i-1}))\label{apdx_eq:cas_dis_bigger}\\
    &\le \sum_{i \in [K]} \frac{\zeta_i p_i^{D,S}}{\sqrt{(1-\mu_i)\mu_i}} \sqrt{(1-\mu_{i+1})...(1-\mu_{K}) \mu_i} + \sum_{i \in [K]} \eta_i p_i^{D,S}\label{apdx_eq:cas_dis_two_sides}\\
    &\le\sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}(p_i^{D,S})^2 }\sqrt{ \sum_{i \in [K]} (1-\mu_{i+1})...(1-\mu_{K}) \mu_i } + \sum_{i \in [K]} \eta_i p_i^{D,S}\label{apdx_eq:cas_dis_cauchy}\\
    &\le \sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}(p_i^{D,S})^2 }\sqrt{ 1-(1-\mu_1)...(1-\mu_K) } + \sum_{i \in [K]} \eta_i p_i^{D,S}\label{apdx_eq:cas_dis_ineq}\\
    &\le\sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}(p_i^{D,S})^2 } + \sum_{i \in [K]} \eta_i p_i^{D,S},
\end{align}
where \cref{apdx_eq:cas_dis_mono} uses $\mu_i \le \bar{\mu}_i, i \in [m]$, \cref{apdx_eq:cas_dis_tlscp} is by telescoping the reward difference, \cref{apdx_eq:cas_dis_def_zeta} is by definition of $\boldzeta,\boldeta$, \cref{apdx_eq:cas_dis_bigger} is due to $\bar{\mu}_i \ge {\mu}_i, i \in [m]$ , \cref{apdx_eq:cas_dis_two_sides} is due to the definition of $p_i^{D,S}$ and we multiply the first term by $\sqrt{\mu_i}$ but divide it by $\sqrt{(1-\mu_i)\mu_i}$, \cref{apdx_eq:cas_dis_cauchy} is due to the Cauchy–Schwarz inequality on the first term, \label{apdx_eq:cas_dis_ineq} is by math calculation.
Hence, $(B_g, B_1, \lambda)=(1,1,2)$.

\end{proof}

\textbf{Conjunctive form.}
For the conjunctive form, the learning agent wants to select $K$ paths from total $L$ paths (i.e., base arms) so as to maximize the probability that the outcomes of the selected paths are all $1$.
Each item is associated with a Bernoulli random variable with mean $\mu_i$, indicating whether the path will be live if the package will transmit via this path.
% The outcome of the selected items are observed only before (or at) the first position whose outcome is 0.
Such a setting models the network routing problem~\cite{kveton2015combinatorial}, where the items are routing paths and the package is delivered when all paths are alive. 
The learning agent will observe the outcome of the first few paths till the first one that is down, since the transmission will stop if any of the path is down. In other words, the triggered set is the prefix set of paths until the stopping condition holds.
We have the following lemma.
\begin{lemma}\label{lem:app_cas_con}
Conjunctive cascading bandit problem satisfies TPVM bounded smoothness condition with coefficient $(B_v,B_1,\lambda)=(1,1,1)$.
\end{lemma}

\begin{proof}
Without loss of generality, suppose the selected base arms are $\{1,...,K\}$, then the reward function is $r(S;\bmu)=\prod_{j=1}^K\mu_j$ and the triggering probability is $p_{i}^{\mu,S}=\prod_{j=1}^{i-1}\mu_j$.
Let $\bar{\bmu}=(\bar{\mu}_1, ..., \bar{\mu}_K)$ and $\bmu=(\mu_1, ..., \mu_K)$, where $\bar{\bmu}=\bmu+\boldzeta + \boldeta$ with $\bar{\bmu}, \bmu \in (0,1)^K, \boldzeta, \boldeta \in [-1,1]^K$.

\begin{align}
    &\abs{r(S;\bar{\bmu})-r(S;\bmu)}\notag\\
    &=\abs{\prod_{i=1}^K\bar{\mu}_i-\prod_{i=1}^K\mu_i}\notag\\
    &\le\abs{\sum_{i \in [K]} (\bar{\mu}_i-\mu_i)(\mu_1...\mu_{i-1} \bar{\mu}_{i+1}...\bar{\mu}_{K})}\notag\\
    &=\sum_{i \in [K]} (\abs{\zeta_i}+\abs{\eta_i})(\mu_1...\mu_{i-1} \bar{\mu}_{i+1}...\bar{\mu}_{K})\notag\\
    &\le \sum_{i \in [K]} \abs{\zeta_i}(\mu_1...\mu_{i-1}) +  \sum_{i \in [K]} \abs{\eta_i}(\mu_1...\mu_{i-1})\label{apdx_eq:cas_con_mono}\\
    &\le \sum_{i \in [K]} \frac{\abs{\zeta_i}}{\sqrt{(1-\mu_i)\mu_i}}\sqrt{p_i^{D,S}} \sqrt{(\mu_1...\mu_{i-1}) (1-\mu_i)} + \sum_{i \in [K]} \abs{\eta_i}p_i^{D,S}\label{apdx_eq:cas_con_bigger}\\
    &\le\sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}p_i^{D,S} }\sqrt{ \sum_{i \in [K]} (\mu_1...\mu_{i-1}) (1-\mu_i) } + \sum_{i \in [K]} \abs{\eta_i}p_i^{D,S}\label{apdx_eq:cas_con_cauchy}\\
    &\le \sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}p_i^{D,S} }\sqrt{ 1-\mu_1...\mu_K } + \sum_{i \in [K]}\abs{\eta_i}p_i^{D,S}\label{apdx_eq:cas_con_ieq}\\
    &\le\sqrt{ \sum_{i \in [K]} \frac{\zeta_i^2}{(1-\mu_i)\mu_i}p_i^{D,S} } + \sum_{i \in [K]} \abs{\eta_i} p_i^{D,S}\label{apdx_eq:cas_con_ieq_2}
\end{align}
where \cref{apdx_eq:cas_con_mono} uses $ \bar{\mu}_i \in [0,1], i \in [m]$, \cref{apdx_eq:cas_con_bigger} is due to the definition of $p_i^{D,S}$ and multiply the first term by $\sqrt{1-\mu_i}$ but divided it by $\sqrt{(1-\mu_i)\mu_i}$, \cref{apdx_eq:cas_con_cauchy} is due to the Cauchy–Schwarz inequality on the first term, \cref{apdx_eq:cas_con_ieq} is by math calculation and \cref{apdx_eq:cas_con_ieq_2} is due to $\mu_i \in [0,1], i \in [m]$.
Hence, $(B_g,B_1,\lambda)=(1,1,1)$.
\end{proof}

% For $\gamma_\infty$ and base arm $i$, 
% \begin{align*}
%     &\frac{\partial r(S;\mu)}{\partial \mu_{i}  } \frac{1}{p_{i}^{\mu,S}}\\
%     &=\prod_{j \in [K] \backslash i}{\mu_{l}}/\prod_{j=1}^{i-1}\mu_j \\
%     &=\prod_{j=i+1}^{K}\mu_j\le 1. 
% \end{align*}
% So $\gamma_{\infty}=1$.

% For $\gamma_g$, we have 
% \begin{align*}
%     &\sum_{i \in [K]}\mu_i (1-\mu_i)\left(\prod_{j\in [K] \backslash i}\mu_j/ \prod_{j=1}^{i-1}\mu_j\right)^2\\
%     &=\sum_{i \in [K]}\mu_i(1-\mu_i) \left(\prod_{j=i+1}^K\mu_j\right)\\
%     &=\sum_{i\in [K]}\left((1-\mu_i) \prod_{j=i+1}^K\mu_j\right) \left( \prod_{j=i}^K\mu_j\right)\\
%     &\le \sum_{i \in [K]}\left((1-\mu_i) \prod_{j=i+1}^K\mu_j\right)\\
%     &=(1-\mu_1)\mu_2\mu_3\dots \mu_K + (1-\mu_2)\mu_3\mu_4 \dots\mu_K + \dots + (1-\mu_{K-1}\mu_K) + (1-\mu_K)\\
%     &=1-\mu_1\mu_2\dots\mu_K\le 1.
% \end{align*}
% We have another way to get a tighter bound with $1/2$ instead of $1$. The idea is to use recursion on the $K=1, ..., \infty$. 
% The above is bounded by $f(k)$, with recursion $f(k+1)=\frac{1}{4(1-f(k))}$ and $f(1)=1/4$. 
% Because $f(k)$ is increasing and converges to $1/2$, we have $\gamma_g=1/\sqrt{2}$.

% Therefore, we have the following regret bound,
% \begin{equation}
%     O\left(\left[ \sum_{i=1}^L\frac{1}{\Delta_{i, \min}} +\sum_{i=1}^L\left(\log_2\frac{ K}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{1}{\Delta_{i, \min}}\right)  \right] \left(\log K\right)^2\log T\right),
% \end{equation}
% while CMAB gives

% \begin{equation}
%     O\left(\left[  \sum_{(i,j)\in \cA} \frac{K}{\Delta_{i,j,\min}}  \right] \log T\right).
% \end{equation}

\subsection{Multi-layered Network Exploration Problem (MuLaNE)~\cite{liu2021multi}}
We consider the MuLaNE problem with random node weights.
After we apply the bipartite coverage graph, the corresponding graph is a tri-partite graph $(n,V,R)$ (i.e., a 3-layered graph where the first layer and the second layer forms a bipartite graph, and the second and the third layer forms another bipartite graph), where the left nodes represent $n$ random walkers; Middle nodes are $|V|$ possible targets $V$ to be explored; Right nodes $R$ are $V$ nodes, each of which has only one edge connecting the middle edge. The MuLaNE task is to allocate $B$ budgets into $n$ layers to explore target nodes $V$ and the base arms are $\cA=\{(i,u,b): i \in [n], u \in V, b \in [B]\}$.

With budget allocation $k_1, ..., k_L$, the (effective) base arms consists of two parts: 

(1) $\{(i,j): i\in[n], j \in V\}$, each of which is associated with visiting probability $x_{i,j}\in[0,1]$ indicating whether node $j$ will be visited by explorer $i$ given $k_i$ budgets. All these base arms corresponds to budget $k_i, i\in [n]$ are triggered.

(2) $y_j\in[0,1]$ for $j \in V$ represents the random node weight. The triggering probability $p_{j}^{D, S}=1-\prod_{i \in [n]}{(1-x_{i,j})}$.

We have the following lemma.
\begin{lemma}\label{lem:app_mulane}
MuLaNE problem satisfies TPVM bounded smoothness condition with coefficient $(B_v,B_1,\lambda)=(\sqrt{1.25|V|},1,2)$, where $|V|$ is the total number of vertices to be explored.
\end{lemma}

\begin{proof}
Let effective base arms $\bmu=(\bx,\by) \in (0,1)^{(n|V|+|V|)}, \bar{\bmu}=(\bar{\bx}, \bar{\by})\in (0,1)^{(n|V|+|V|)}$, where $\bar{\bx}=\boldzeta_{x}+\boldeta_{x}+\bx, \bar{\by}=\boldzeta_{y}+\boldeta_{y}+\by$, for $\boldzeta, \boldeta \in [-1,1]^{(n|V|+|V|)}$.
For the target node $j \in V$, the per-target reward function $r_j(S;\bx,\by)=y_j(1-\prod_{i \in [n]}(1-x_{i,j}))$.
Denote $\bar{p}_j^{D,S}=1-\prod_{i \in [n]}{(1-\bar{x}_{i,j})}$.

\begin{align}
    &\abs{r(S;\bar{\bmu})-r(S;\bmu)}\notag\\
    &=\abs{\sum_{j \in V} r_j(S;\bar{\bx},\bar{\by}) - r_j(S;\bx,\by)}\notag\\
    &=\abs{ \sum_{j \in V} \bar{y}_j \bar{p}_j^{D,S} - \bar{y}_j p_{j}^{D, S} + \bar{y}_j p_{j}^{D, S} - y_j p_{j}^{D, S}}\notag\\
    &=\abs{\sum_{j \in V} \bar{y}_j \left(\prod_{i \in [n]}(1-x_{i,j})-\prod_{i \in [n]}(1-\bar{x}_{i,j}))\right) + \sum_{j \in V} (\bar{y}_j-y_j)p_{j}^{D, S}}\label{apdx_eq:mulane_tlscp}\\
    &\le\abs{\sum_{j \in V} \sum_{i \in [n]}(\bar{x}_{i,j}-x_{i,j})\left((1-x_{1,j})...(1-x_{i-1,j})(1-\bar{x}_{i+1,j})...(1-\bar{x}_{L,j})\right)\bar{y}_j}\notag\\
    &+\abs{\sum_{j \in V} (\bar{y}_j-y_j)p_{j}^{D, S}}\notag\\
    &\le\sum_{j \in V}\sum_{i \in [n]}(\abs{\zeta_{x,i,j}}+\abs{\eta_{x,i,j}})\left((1-x_{1,j})...(1-x_{i-1,j})\right)\bar{y}_j+\sum_{j \in V}(\abs{\zeta_{y,j}}+\abs{\eta_{y,j}})p_{j}^{D, S}\label{apdx_eq:mulane_bigger}\\
    &\le\sum_{j \in V}\sum_{i \in [n]}(\frac{\abs{\zeta_{x,i,j}}}{\sqrt{(1-x_{i,j})x_{i,j}}})\sqrt{\left((1-x_{1,j})...(1-x_{i-1,j})\right)x_{i,j}}\bar{y}_j\notag\\
    &+\sum_{j \in V}\left(\frac{\abs{\zeta_{y,j}}p_{j}^{D, S}}{\sqrt{(1-y_j)y_j}}\right)\sqrt{(1-y_j)y_j}+\left(\sum_{j \in V}\sum_{i \in [n]}\abs{\eta_{x,i,j}} + \sum_{j \in V}\abs{\eta_{y,j}}p_{j}^{D, S}\right)\label{apdx_eq:mulane_multiply}\\
    &\le \sqrt{ \sum_{j \in V}\sum_{i \in [n]}(\frac{\zeta_{x,i,j}^2}{(1-x_{i,j})x_{i,j}})+\sum_{j \in V}\frac{\zeta_{y,j}^2(p_{j}^{D, S})^2}{(1-y_j)y_j}}\notag\\
    &\cdot\sqrt{\sum_{j \in V}\sum_{i \in [n]}\left((1-x_{1,j})...(1-x_{i-1,j})\right)x_{i,j}\bar{y}^2_j + \sum_{j \in V}(1-y_j)y_j}\notag\\
    &+ \left(\sum_{j \in V}\sum_{i \in [n]}\abs{\eta_{x,i,j}} +\sum_{j \in V} \abs{\eta_{y,j}}p_{j}^{D, S}\right)\label{apdx_eq:mulane_cauchy}\\
    &= \sqrt{ \sum_{j \in V}\sum_{i \in [n]}(\frac{\zeta_{x,i,j}^2}{(1-x_{i,j})x_{i,j}})+\sum_{j \in V}\frac{\zeta_{y,j}^2(p_{j}^{D, S})^2}{(1-y_j)y_j}} \sqrt{\sum_{j \in V}\left(1-\prod_{i \in [n]}(1-x_{i,j})\right)\bar{y}^2_j + \sum_{j \in V}(1-y_j)y_j}\notag\\
    &+ \left(\sum_{j \in V}\sum_{i \in [n]}\abs{\eta_{x,i,j}} + \sum_{j \in V}\abs{\eta_{y,j}}p_{j}^{D, S}\right)\label{apdx_eq:mulane_fold}\\
    &\le \sqrt{\sum_{j \in V} \sum_{i \in [n]}(\frac{\zeta_{x,i,j}^2}{(1-x_{i,j})x_{i,j}})+\sum_{j \in V}\frac{\zeta_{y,j}^2(p_{j}^{D, S})^2}{(1-y_j)y_j}} \sqrt{\sum_{j \in V}\bar{y}^2_j + (1-y_j)y_j}+  \notag\\
    &\left(\sum_{j \in V}\sum_{i \in [n]}\abs{\eta_{x,i,j}} + \sum_{j \in V}\abs{\eta_{y,j}}p_{j}^{D, S}\right)\label{apdx_eq:mulane_bounded}\\
    &\le \sqrt{ \sum_{j \in V}\sum_{i \in [n]}(\frac{\zeta_{x,i,j}^2}{(1-x_{i,j})x_{i,j}})+\sum_{j \in V}\frac{\zeta_{y,j}^2(p_{j}^{D, S})^2}{(1-y_j)y_j}} \cdot \sqrt{1.25|V|} \notag\\
    &+ \left(\sum_{j \in V}\sum_{i \in [n]}\abs{\eta_{x,i,j}}+\sum_{j \in V}\abs{\eta_{y,j}}p_{j}^{D, S}\right),\label{apdx_eq:mulane_bounded_2}
\end{align}
where \cref{apdx_eq:mulane_tlscp} is by telescoping the difference of $\left(\prod_{i \in [n]}(1-x_{i,j})-\prod_{i \in [n]}(1-\bar{x}_{i,j}))\right)$, \cref{apdx_eq:mulane_bigger} is due to $\bar{x}_{i,j} \in [0,1]$ for any $i,j$, \cref{apdx_eq:mulane_multiply} is because we multiply the first term by $\sqrt{x_{i,j}}$ but divide it by $\sqrt{x_{i,j}(1-x_{i,j})}$  and we multiply the second term by $\sqrt{y_j}$ but divide it by $\sqrt{y_j(1-y_j)}$, \cref{apdx_eq:mulane_cauchy} is by applying the Cauchy-Schwarz inequality to the first term and the second term simultaneously, \cref{apdx_eq:mulane_fold} is due to the math calculation on , \cref{apdx_eq:mulane_bounded} is due to the support of $x_{i,j}$ are bounded with $[0,1]$ for any $i,j$ and \cref{apdx_eq:mulane_bounded_2} is due to the support of $y_{j}, \bar{y}_{j}$ are bounded with $[0,1]$ for any $j$.
Hence $(B_g, B_1, \lambda)=(\sqrt{1.25|V|}, 1, 2)$.
\end{proof}

\subsection{Online Influence Maximization Bandit~\cite{wang2017improving}}
In this section, we first introduce the general problem setting of online influence maximization (OIM). Then we start with a easier problem instance, i.e., OIM on tri-partite graph (TPG) to get some intuition, where reward functions have closed form solutions. Finally, we give the results for OIM on the directed acyclic graph (DAG), which are much more involved since the reward function have no closed form solutions.

\subsubsection{Setting of the Online Influence Maximization}
Following the setting of \citep[Section 2.1]{wang2017improving}, we consider a weighted directed graph $G(V,E,p)$, where $V$ is the set of vertices, $E$ is the set of directed edges, and each edge $(u,v)\in E$ is associated with a probability $p(u,v)\in [0,1]$. When the agent selects a set of seed nodes $S \subseteq V$, the influence propagates as follows: At time $0$, the seed nodes $S$ are activated; At time $t > 1$, a node $u$ activated at time $t-1$ will have one chance to activate its inactive out-neighbor $v$ with independent probability $p(u,v)$. The influence spread of $S$ is denoted as $\sigma(S)$ and is defined as the expected number of activated nodes after the propagation process ends. The problem of Influence Maximization is to find seed nodes $S$ with $|S|\le k$ so that the influence spread $\sigma(S)$ is maximized. 

For the problem of online influence maximization (OIM), we consider $T$ rounds repeated influence maximization tasks and the edge probabilities $p(u,v)$ are assumed to be unknown initially. For each round $t\in [T]$, the agent selects $k$ seed nodes as $S_t$, the influence propagation of $S_t$ is observed and the reward is the number of nodes activated in round $t$. The agent's goal is to accumulate as much reward as possible in $T$ rounds. The OIM fits into CMAB-T framework: the edges $E$ are the set of base arms $[m]$, the (unknown) outcome distribution $D$ is the joint of $m$ independent Bernoulli random variables for the edge set $E$, the action $S$ are any seed node sets with size $k$ at most $k$. For the arm triggering, the triggered set $\tau_t$ is the set of edges $(u,v)$ whose source node $u$ is reachable from $S_t$. Let $X_t$ be the outcomes of the edges $E$ according to probability $p(u,v)$ and the live-edge graph $G_t^{\text{live}}(V,E^{\text{live}})$ be a induced graph with edges that are alive, i.e., $e \in E^{\text{live}}$ iff $X_{t,e}=1$ for $e \in E$. The triggering probability distribution $D_{\text{trig}}(S_t,X_t)$ degenerates to a deterministic triggered set, i.e., $\tau_t$ is deterministically decided given $S_t$ and $X_t$. The reward $R(S_t, X_t, \tau_t)$ equals to the number activated nodes at the end of $t$, i.e., the nodes that are reachable from $S_t$ in the live-edge graph $G_t^{\text{live}}$. The offline oracle is a $(1-1/e-\varepsilon, 1/|V|)$-approximation algorithm given by the greedy algorithm from~\cite{kempe2003maximizing}.


\subsubsection{Online Influence Maximization Bandit on Tri-partite Graph (TPG)}
We consider a OIM scenario where the underlying graph is a graph with three layers: the seed node layer, the intermediate layer and the target node layer.
Specifically, the underlying graph is denoted as $(L,M,R)$, where the first layer consists of $L$ candidates for the seed node selection, the second layer consists of $M$ intermediate nodes and the third layer are $R$ target nodes.
Such a setting is of significant interest since the edges connecting the target nodes can only be triggered and cannot be observed by seed-node selection, which requires the notion of triggering arms.
Another favorable feature is that the reward function of this setting can be explicitly expressed, whereas for general IM, even calculating the explicit form of the reward function is NP-hard~\cite{chen2009efficient}.

In this application, the base arms consists of two parts:

(1) $\{(i,j): i\in[L], j \in [M]\}$, each of which is associated with probability $x_{i,j}\in[0,1]$ indicating the probability whether edge $(i,j)$ is alive when $i$ is selected as seed nodes. Without loss of generality, we assume the seed nodes are $S=\{1,...,K\}$.

(2)$\{(j,k): j\in[M], k \in [R]\}$, each of which is associated with probability $y_{j,k} \in [0,1]$ indicating whether edge $(j,k)$ is live when $j$ is triggered for the first time. The triggering probability $p_{j}^{D, S}=1-\prod_{i \in [K]}{(1-x_{i,j})}$.

Let $\bmu=(\bx,\by)\in (0,1)^{(LM+MR)}, \bar{\bmu}=(\bar{\bx}, \bar{\by})\in  (0,1)^{(LM+MR)}$, where $\bar{\bx}=\boldzeta_{x}+\boldeta_{x}+\bx, \bar{\by}=\boldzeta_{y}+\boldeta_{y}+\by$, for $\boldzeta, \boldeta \in [0,1]^{(LM+MR)}$.
Fix any target node $k$, the reward function $r_k(S;\bx,\by)=1-\prod_{j \in [M]}\left(1-y_{j,k}(1-\prod_{i \in [K]}(1-x_{i,j}))\right)$.


\begin{lemma}\label{lem:app_tbg}
OIM-TPG problem satisfies {\TPVMm} bounded smoothness condition with coefficient $(B_v,B_1,\lambda)=(\sqrt{2}R,R,1)$, where $R$ is the total number of target nodes.
\end{lemma}

\begin{proof}

For notational brevity, we denote $p_j\triangleq p_j^{D,S}=1-\prod_{i \in [L]}{(1-x_{i,j})}$, $\bar{p}_j=1-\prod_{i \in [K]}(1-\bar{x}_{i,j}), g_j=1-\bar{y}_{j,k} p_j, \bar{g}_j=1-\bar{y}_{j,k}\bar{p}_j$.

The difference of $r_k(S; \bar{\bmu}),r_k(S; \bmu)$ can be written as,
\begin{align}
    \abs{r(S; \bar{\bmu})-r(S; \bmu)}&= \sum_{k \in [R]}r_k(S; \bar{\bmu})-r_k(S; \bmu)\label{apdx_eq:tpg_mono}\\
    &= \sum_{k \in [R]}\underbrace{\left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k}\bar{p}_j) \right) - \left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k} p_j) \right)}_{\text{term (a)}} \notag\\
    &+ \sum_{k \in [R]}\underbrace{\left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k} p_j) \right) - \left(1-\prod_{j\in [M]}(1-y_{j,k} p_j) \right)}_{\text{term} (b)}\label{apdx_eq:tpg_add_minus},
\end{align}
where \cref{apdx_eq:tpg_add_minus} is by adding and subtracting the same $\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k} p_j) \right)$.

For term $(a)$, it holds that
\begin{align}
    &\text{term} (a) = \sum_{j \in [M]}(g_j-\bar{g}_j)(g_1...g_{j-1} \bar{g}_{j+1}...\bar{g}_M)\label{apdx_eq:tpg_a_tlscp}\\
    &= \sum_{j \in [M]}\bar{y}_{j,k}(\bar{p}_j-p_j)(g_1...g_{j-1} \bar{g}_{j+1}...\bar{g}_M)\notag\\
    &= \sum_{j \in [M]}\bar{y}_{j,k}(g_1...g_{j-1} \bar{g}_{j+1}...\bar{g}_M)\left(\left(1-\prod_{i \in [K]}(1-\bar{x}_{i,j})\right)- \left( 1-\prod_{i \in [K]}(1-x_{i,j}) \right)\right)\notag\\
    &= \sum_{j \in [M]}\bar{y}_{j,k}(g_1...g_{j-1} \bar{g}_{j+1}...\bar{g}_M)\sum_{i \in [K]}(\bar{x}_{i,j}-x_{i,j})\left((1-x_{1,j})...(1-x_{i-1,j}) (1-x_{i+1,j})...(1-x_{K,j})\right)\label{apdx_eq:tpg_a_tlscp_p}\\
    &=\sum_{i \in [K]}\sum_{j \in [M]}(\zeta_{x,i,j}+\eta_{x,i,j})\bar{y}_{j,k}(g_1...g_{j-1} \bar{g}_{j+1}...\bar{g}_M)\left((1-x_{1,j})...(1-x_{i-1,j}) (1-x_{i+1,j})...(1-x_{K,j})\right)\notag\\
    &\le \underbrace{\sum_{i \in [K]}\sum_{j \in [M]}\left(\frac{\zeta_{x,i,j}}{\sqrt{(1-x_{i,j})x_{i,j}}}\right)\sqrt{x_{i,j}(1-x_{1,j})...(1-x_{i-1,j})\bar{y}_{j,k} (g_1...g_{j-1})}}_{\text{term} (c)} \notag\\
    &+ \underbrace{\sum_{i \in [K]}\sum_{j \in [M]}\eta_{x,i,j}}_{\text{term} (d)}\label{apdx_eq:tpg_a_multi_div},
\end{align}
where \cref{apdx_eq:tpg_a_tlscp} is by telescoping the term (b), \cref{apdx_eq:tpg_a_tlscp_p} is by telescoping $\bar{p}_j-p_j$, \cref{apdx_eq:tpg_a_multi_div} is because $\bar{g}_j\in [0,1]$ for all $j$ and multiplying the first term by $\sqrt{x_{i,j}}$ but dividing it by $\sqrt{(1-x_{i,j})x_{i,j}}$.

For term $(b)$, it holds that 
\begin{align}
    \text{term} (b) &= \left(1-\prod_{j \in [M]}(1-\bar{y}_{j,k} p_j) \right) -\left(1-\prod_{j \in [M]}(1-y_{j,k} p_j) \right)\notag\\
    &=\sum_{j \in [M]}p_j (\bar{y}_{j,k} - y_{j,k}) (1-y_{1,k} p_1)...(1-y_{j,k} p_j) (1-\bar{y}_{j+1,k}p_{j+1})... (1-\bar{y}_{M,k} p_M)\label{apdx_eq:tpg_b_tlscp_p}\\
    &\le \underbrace{\sum_{j \in [M]}\left(\frac{\zeta_{y,j,k}\sqrt{p_j}}{\sqrt{(1-y_{j,k})y_{j,k}}}\right)\sqrt{y_{j,k}p_j(1-y_{1,k} p_1)...(1-y_{j-1,k}p_{j-1})}}_{\text{term} (e)} + \underbrace{\sum_{j\in [M]}p_{j}\eta_{y,j,k}}_{\text{term} (f)}\label{apdx_eq:tpg_b_multi_div},
\end{align}
where \cref{apdx_eq:tpg_b_tlscp_p} is by telescoping on the term (b), \cref{apdx_eq:tpg_b_multi_div} is by multiplying the first term by $\sqrt{y_{i,j}}$ but dividing it by $\sqrt{(1-y_{i,j})y_{i,j}}$.

Next, we apply Cauchy–Schwarz inequality to term (c) and term (e) simultaneously,
\begin{align}
    &\sum_{k \in [R]}(\text{term} (c) + \text{term} (e))\notag\\ 
    &\le \sqrt{\left(\sum_{i \in [K], j \in [M], k \in [R]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\notag\\
    &\cdot \Bigg[\left(\sum_{i \in [K]}\sum_{j\in [M]}\sum_{k \in [R]}x_{i,j}(1-x_{1,j})...(1-x_{i-1,j})\bar{y}_{j,k} (g_1...g_{j-1})\right)\notag\\
    &+\left(\sum_{j \in [M]}\sum_{k \in [R]}y_{j,k}p_j(1-y_{1,k} p_1)...(1-y_{j-1,k}p_{j-1})\right)\Bigg]^{1/2}\notag\\
    &\le \sqrt{\left(\sum_{i \in [K], j \in [M], k \in [R]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\notag\\
    &\cdot \sqrt{\left(\sum_{j\in [M]}\sum_{k \in [R]}(1-\prod_{i \in [K]}(1-x_{i,j}))\bar{y}_{j,k} (g_1...g_{j-1})\right)+\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-y_{j,k}p_{j})\right)}\label{apdx_eq:tpg_ce_math_x}\\
    &= \sqrt{\left(\sum_{i \in [K], j \in [M], k \in [R]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\notag\\
    &\cdot \sqrt{\sum_{k \in [R]}\left(\sum_{j\in [M]}(1-g_j) (g_1...g_{j-1})\right)+\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-y_{j,k}p_{j})\right)}\label{apdx_eq:tpg_ce_def_g}\\
        &= \sqrt{\left(\sum_{i \in [K], j \in [M], k \in [R]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\notag\\
        &\cdot \sqrt{\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k}p_{j})\right)+\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-y_{j,k}p_{j})\right)}\label{apdx_eq:tpg_ce_math_g}\\
             &\le \sqrt{R}\sqrt{\left(\sum_{i \in [K]}\sum_{j \in [M]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\notag\\
             &\cdot \sqrt{\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-\bar{y}_{j,k}p_{j})\right)+\sum_{k \in [R]}\left(1-\prod_{j\in [M]}(1-y_{j,k}p_{j})\right)}\label{apdx_eq:tpg_ce_i_in_K}\\
        &\le \sqrt{\left(\sum_{i \in [K], j \in [M], k \in [R]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\cdot\sqrt{2}R\label{apdx_eq:tpg_ce_bounded},
\end{align}
where \cref{apdx_eq:tpg_ce_math_x} is due to the math calculation on the summation over $i \in [K]$, \cref{apdx_eq:tpg_ce_def_g} is due to the definition of $g_j$, \cref{apdx_eq:tpg_ce_math_g} is due to the math calculation on the summation over $j \in [M]$, \cref{apdx_eq:tpg_ce_i_in_K} is because we take one summation over $k \in [R]$ out for the first square root term and \cref{apdx_eq:tpg_ce_bounded} is because $y_{j,k},\bar{y}_{j,k}, p_j$ are all bounded with support $[0,1]$.

Combined with $\sum_{k \in [R]}(\text{term}(d)+ \text{term}(f))$, we can derive that 
\begin{align}
    \abs{r(S; \bar{\bmu})-r(S; \bmu)} &= \sqrt{\left(\sum_{i \in [K]}\sum_{j \in [M]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\cdot\sqrt{2}R \notag\\
    &+ \sum_{i \in [K]}\sum_{j \in [M]}\sum_{k \in [R]}\eta_{x,i,j} + \sum_{j\in [M]}\sum_{k \in [R]}p_{j}\eta_{y,j,k}\notag\\
    &\le\sqrt{\left(\sum_{i \in [K]}\sum_{j \in [M]}\frac{\zeta^2_{x,i,j}}{(1-x_{i,j})x_{i,j}}\right) + \left(\sum_{j \in [M]}\sum_{k \in [R]}\frac{\zeta^2_{y,j,k}p_j}{(1-y_{j,k})y_{j,k}}\right)}\cdot\sqrt{2}R \notag\\
    &+ R\left( \sum_{i \in [K]}\sum_{j \in [M]}\eta_{x,i,j} + \sum_{j\in [M]}\sum_{k \in [R]}p_{j}\eta_{y,j,k}\right)\label{apdx_eq:tpg_all_i_in_K},
\end{align}
where \cref{apdx_eq:tpg_all_i_in_K} is because the summation over $k \in [R]$ in the second term.

Hence we have $(B_g, B_1, \lambda)=(\sqrt{2}R, R, 1)$.
\end{proof}



% For $\gamma_\infty$ and base arm $p_{i,j}$, 
% \begin{align*}
%     &\frac{\partial r(S;p,y)}{\partial p_{i,j}  } \frac{1}{p_{i}^{D,S}}\\
%     &=y_j \prod_{l \in [L] \backslash i}(1-p_{l,j}) \le 1.
% \end{align*}
% For base arm $y_j$,
% \begin{align*}
%     &\frac{\partial r(S;p,y)}{\partial y_{j}  } \frac{1}{p_{j}^{D,S}}\\
%     &= (1-\prod_{i \in [L]}{(1-p_{i,j})})/(1-\prod_{i \in [L]}{(1-p_{i,j})}) \\
%     &= 1.
% \end{align*}
% So $\gamma_{\infty}=1$.

% For $\gamma_g$,
% \begin{align*}
%     &\sum_{i,j}p_{i,j}(1-p_{i,j})y_j^2 \left(\prod_{l \in [L] \backslash i}(1-p_{l,j})\right)^2 + \sum_{j \in [M]}y_j (1-y_j)(1-\prod_{i \in [L]}{(1-p_{i,j})})^2/(p_{j}^{D,S})^2\\
%     &=\sum_{j \in [M]}\prod_{i \in [L]}(1-p_{i,j})\sum_{i \in [L]} p_{i,j} \prod_{l \in [L] \backslash i}(1-p_{l,j}) + \sum_{j \in [M]}y_j (1-y_j)\\
%     &\le \sum_{j\in[M]} \frac{y_j^2}{4} + y_j(1-y_j)\\
%     &\le M/3
% \end{align*}
% So $\gamma_g\le M/\sqrt{3}$.

% Therefore, we have the following regret bound,
% \begin{equation}
%     O\left(\left[ \sum_{i=1}^m\frac{1}{\Delta_{i, \min}} +\sum_{i=1}^m\left(\log_2\frac{ M(L+1)}{\Delta_{i}^{\min}}\right) \left(1+\log \frac{M}{\Delta_{i, \min}}\right)  \right] \left(\log M(L+1)\right)^2\log T\right),
% \end{equation}
% while CMAB gives

% \begin{equation}
%     O\left(\left[  \sum_{(i,j)\in \cA} \frac{M(L+1)}{\Delta_{i,j,\min}}  \right] \log T\right).
% \end{equation}

\subsubsection{Influence Maximization on Directed Acyclic Graphs (DAG)}
In this section, we introduce how to derive $(B_g, B_1, \lambda)$ for DAGs. Note that TBG (or even multi-layered bipartite graphs) are special cases of DAG. However, the main challenge is that for general DAGs, there are no closed-form solutions for the reward function since it is NP-Hard to compute their influence spread \cite{chen2009efficient}. To deal with this challenge, we will use the live-edge graph and edge coupling technique as \cite{li2020online} and prove the following lemma.

\begin{lemma}\label{lem:app_dag}
OIM-DAG problem satisfies {\TPVMm} bounded smoothness condition with coefficient $(B_v,B_1,\lambda)=(\sqrt{L}|V|,|V|,1)$, where $L$ is the length of the longest directed path.
\end{lemma}
\begin{proof}
Denote the DAG graph as $G(V,E)$ where $V$ are nodes and $E$ are the edges. With a little abuse of the notation, we will denote $u(e), v(e)$ as the starting node and ending node of the edge $e$.
Inspired by previous applications with closed-form solutions, we will partition edges $E$ (i.e., base arms) into $L$ groups, where $L$ is the length of the longest directed path of $G$. More specifically, we apply the topological sort on $G$ and label each node with $l(v)\in \{0,1,...,L\}$, where $l(v)$ is the length of the longest path that starts from node $v$. For simplicity, we say node $v$ in layer $l(v)$. This sorting and labelling procedure can be done in $O(V+E)$ time complexity. Given this labelling $l(v)$ for $v\in V$, we partition edges $E$ into $L$ disjoint edge sets so that $E = \bigcup_{s \in [L]}E_s$, where $E_s$ contains edges that point from node in layer $s$ to node in lower layers, i.e., $E_s=\{(u,v): l(u)=s, l(v)< s\}$. One critical property we will use later is that for any two edges $e, e' \in E_s$ in the same layer $s$, there are no directed path $p$ from any node $v \in V$ so that both $e, e'$ are in the path $p$, or otherwise $l(u(e))\neq l(u(e'))$ which contradicts the assumption that starting nodes $u(e)$ and $u(e')$ belong to the same layer $s$.

Let $\bmu= (\bmu_1, ..., \bmu_L)$ be the true mean vector for the partitions $(E_1, ..., E_L)$ mentioned above, where each partition contains $n_{s}=|E_{s}|$ base arms (with $\bmu_{s} \in (0,1)^{n_{s}}$), for $s \in [L]$. Similarly, we denote $\bar{\bmu}=(\bar{\bmu}_1, ..., \bar{\bmu}_L), \boldzeta= (\boldzeta_1, ..., \boldzeta_L), \boldeta= (\boldeta_1, ..., \boldeta_L)$ such that $\bar{\bmu}=\bmu + \boldzeta + \boldeta$ and $\bar{\bmu}_s \in (0,1)^{n_s}, \boldzeta, \boldeta \in [0,1]^{n_s}$.
Now for the reward, we focus on each node $t$ as target, so that $r(S;\bmu)\triangleq \sum_{t \in V} r_t(S;\bmu)$ and $r(S;\bar{\bmu})\triangleq \sum_{t \in V} r_t(S;\bar{\bmu})$. Now fix any target node $t \in V$, we can telescope the reward by gradually changing one partition from $\bar{\bmu}_s$ to $\bmu_s$ as follows:
\begin{align}
    &\abs{r_t(S;\bar{\bmu})-r_t(S;\bmu)}\notag\\
    &=r_t(S;\bar{\bmu}_1, ..., \bar{\bmu}_L)-r_t(S;\bmu_1, \bar{\bmu}_2, ..., \bar{\bmu}_L)\notag\\
        &=r_t(S;\bmu_1, \bar{\bmu}_2, ..., \bar{\bmu}_L)-r_t(S;\bmu_1, \bmu_2, \bar{\bmu}_3, ..., \bar{\bmu}_L)\notag\\
    &+ ... \notag\\
    &+\underbrace{r_t(S;\bmu_1,... \bmu_{s-1}, \bar{\bmu}_{s}, ..., \bar{\bmu}_{L})-r_t(S;\bmu_1,..., \bmu_{s}, \bar{\bmu}_{s+1}, ..., \bar{\bmu}_{L})}_{\text{s-th partition}}\notag\\
    &+ ... \notag\\
    &+r_t(S;\bmu_1, ..., \bmu_{L-1}, \bar{\bmu}_L)-r_t(S;\bmu_1, ..., \bmu_L)
\end{align}

For the s-th partition, since the first term and the second term differs only in $\bmu_s$ and $\bar{\bmu}_s$, we denote the first $s-1$ partitions as $\cup_{\ell=1}^{s-1}\bmu_{\ell}$ and the last $L-s$ partitions as $\cup_{\ell=s+1}^L \bar{\bmu}_{\ell}$. We can further telescope the reward difference by gradually changing one parameter from $\bar{\mu}_{s,i}$ to $\mu_{s,i}$ as follows:

\begin{align}
    &\text{s-th partition}\notag\\     
    &=r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \bar{\mu}_{s,1}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})-r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1}, \bar{\mu}_{s,2}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})\notag\\
        &=r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1}, \bar{\mu}_{s,2}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})-r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1}, \mu_{s,2}, \bar{\mu}_{s,3}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})\notag\\
    &+ ... \notag\\
    % &+\underbrace{r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1},... \mu_{s,i-1}, \bar{\mu}_{s,i}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})-r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1},..., \mu_{s,i}, \bar{\mu}_{s,i+1}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}))}_{\text{i-th change in s-th partition}}\notag\\
    &+\underbrace{r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \cup_{\ell=1}^{i-1}\mu_{s,\ell}, \cup_{\ell=i}^{n_s}\bar{\mu}_{s,\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})-r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \cup_{\ell=1}^{i}\mu_{s,\ell}, \cup_{\ell=i+1}^{n_s}\bar{\mu}_{s,\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}))}_{\text{i-th change in s-th partition}}\notag\\
    &+ ... \notag\\
    &+r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1}, ..., \mu_{s,n_s-1}, \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})-r_t(S;\cup_{\ell=1}^{s-1}\bmu_{\ell}, \mu_{s,1}, ..., \mu_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})
\end{align}

For the i-th change in s-th partition, we use the live edge graph~\cite{chen2013information} technique (which links the probability of a node is activated to the probability this node is reachable in the random live-edge graph where each edge $i$ is independently selected as live-edge with probability $\mu_i$), in order to transform the reward difference into the probability of some events happens. Note that by using ``bypass of edge $e$", we mean the path that connects seed nodes $S$ and target node $t$ but does not contains edge $e$ in this path.
Let $e_{s,i}=(u(e_{s,i}), v(e_{s,i}))$ denote the $i$-th edge with staring node $u(e_{s,i})$ and ending node $v(e_{s,i})$ in partition $E_s$, for $i\in [n_s]$. We use $\Pr[A| \bmu]$ to denote the probability of all live-edge graphs under parameter $\bmu$ so that event $A$ happens. Consider the live-edge graphs without $e_{s,i}$,

\begin{align}
    &\text{i-th change in s-th partition}\notag\\
    &=(\bar{\mu}_{s,i}-\mu_{s,i}) \Pr[S\rightarrow u(e_{s,i}), v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s-1}\bmu_{\ell},\notag\\
    &\mu_{s,1},... \mu_{s,i-1}, \bar{\mu}_{s,i+1}, ..., \bar{\mu}_{s,n_s}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]\label{apdx_eq:oim_dag_live_edge}\\
    &\le (\bar{\mu}_{s,i}-\mu_{s,i}) \Pr[S\rightarrow u(e_{s,i}), v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}, \bmu_{s} \backslash \mu_{s,i}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]\label{apdx_eq:oim_dag_live_edge_change}\\
    &\le \zeta_{s,i} \Pr[S\rightarrow u(e_{s,i}), v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}, \bmu_{s} \backslash \mu_{s,i}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}] \notag\\
    &+\eta_{s,i}\Pr[S\rightarrow u(e_{s,i}) \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]\label{apdx_eq:oim_dag_second_obs}\\
    &=\sqrt{\frac{\zeta^2_{s,i}}{\mu_{s,i}}} \sqrt{\mu_{s,i}(\Pr[S\rightarrow u(e_{s,i}), v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}, \bmu_{s}\backslash \mu_{s,i}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}])^2}\notag\\
    &+ \eta_{s,i}\Pr[S\rightarrow u(e_{s,i}) \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]\label{apdx_eq:oim_dag_multiply_divide}\\
    &\le\sqrt{ \frac{\zeta^2_{s,i}\Pr[S\rightarrow u(e_{s,i})\mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]}{(1-\mu_{s,i})\mu_{s,i}}} \notag\\
    &\cdot\sqrt{\Pr[S\rightarrow u(e_{s,i}), e_{s,i} \text{ is live},  v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s}\bmu_{\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]}\notag\\
    &+ \eta_{s,i}\Pr[S\rightarrow u(e_{s,i}) \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]\label{apdx_eq:oim_dag_divide},
\end{align}
where \cref{apdx_eq:oim_dag_live_edge} is due to the coupling technique~\cite{li2020online} and the contribution of live-edge graph $G'$ to the reward difference is $\bar{\mu}_{s,i} - \mu_{s,i}$ if $u(e_{s,i})$ is reachable from $S$, the target node $t$ is reachable from $v(e_{s,i})$ but $t$ is not reachable from any other paths in $G'$ that bypasses edge $e_{s,i}$ or otherwise the contribution of $G'$ is $0$; \cref{apdx_eq:oim_dag_live_edge_change} is due to $e_{s,i}$ and $e_{s,j}$ for $j \in [n_s]\backslash\{i\}$ are in the same s-th partition, so that the parameter change from $\bar{\mu}_{s,j}$ to $\mu_{s,j}$ for $j \in [n_s]\backslash\{i\}$ neither affects the probability of $u(e_{s,i})$ is reachable from $S$ nor affects the probability of the target node $t$ is reachable from $v(e_{s,i})$, but only increases the probability of there is no bypass of $e_{s,i}$ (since there is less possibility of a path connects $S$ and $t$ by reducing $\bar{\mu}_{s,j}$ to $\mu_{s,j}$); \cref{apdx_eq:oim_dag_second_obs} is because for the second term, we only require $u(e_{s,i})$ is reachable from $S$; \cref{apdx_eq:oim_dag_multiply_divide} is because we multiply and divide the first term by $\sqrt{\mu_{s,i}}$ at the same time; \cref{apdx_eq:oim_dag_divide} is because we divide the first term by $\sqrt{1-\mu_{s,i}}$ which is within $(0,1)$.


Now we can summation over all $(s,i)_{s \in [L], i \in [n_s]}$, we have
\begin{align}
    &\abs{r_t(S;\bar{\bmu})-r_t(S;\bmu)}\notag\\
    &\le\sum_{s,i}\sqrt{ \frac{\zeta^2_{s,i}\Pr[S\rightarrow u(e_{s,i})\mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]}{(1-\mu_{s,i})\mu_{s,i}}} \notag\\
    &\cdot\sqrt{\Pr[S\rightarrow u(e_{s,i}),e_{s,i} \text{ is live},  v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s}\bmu_{\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]}\notag\\
    &+ \sum_{s \in [L]}\sum_{i \in [n_s]}\eta_{s,i}\Pr[S\rightarrow u(e_{s,i}) \mid \cup_{\ell=1}^{s-1}\bmu_{\ell}]\notag\\
    &\le \sqrt{\sum_{i \in [m]}\frac{\zeta_{i}^2 p_i^{D,S}}{\mu_i(1-\mu_i)}\left(\sum_{s \in [L]}\sum_{i \in [n_s]}\Pr[S\rightarrow u(e_{s,i}),e_{s,i} \text{ is live},  v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s}\bmu_{\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]\right)}\notag\\
    &+ \sum_{i \in [m]}\eta_{i}p_{i}^{D,S}\label{apdx_eq:oim_dag_cauchy}\\
    &\le \sqrt{\sum_{i \in [m]}\frac{\zeta_{i}^2 p_i^{D,S}}{\mu_i(1-\mu_i)}}\sqrt{L}+ \sum_{i \in [m]}\eta_{i}p_{i}^{D,S},\label{apdx_eq:oim_dag_no_overlap}
\end{align}
where \cref{apdx_eq:oim_dag_cauchy} uses the Cauchy-Schwatz Inequality; \cref{apdx_eq:oim_dag_no_overlap} uses the critical property that for $e_{s,i}$ and $e_{s,j}$ with $i\neq j$, there does not exist any path that can contain both $e_{s,i}$ and $e_{s,j}$ as mentioned earlier, which means under the same parameter $(\cup_{\ell=1}^{s}\bmu_{\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell})$, the live edge graphs that satisfies $\{S\rightarrow u(e_{s,i}),e_{s,i} \text{ is live},  v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i}\}$ and the live edge graphs that satisfies $\{S\rightarrow u(e_{s,j}),e_{s,j} \text{ is live},  v(e_{s,j})\rightarrow t, \text{ no bypass of } e_{s,j}\}$ are disjoint (or otherwise contradicts the fact that there is no bypass of $e_{s,i}$ or $e_{s,j}$), so it holds that $\sum_{i \in [n_s]}\Pr[S\rightarrow u(e_{s,i}),e_{s,i} \text{ is live},  v(e_{s,i})\rightarrow t, \text{ no bypass of } e_{s,i} \mid \cup_{\ell=1}^{s}\bmu_{\ell}, \cup_{\ell=s+1}^L\bar{\bmu}_{\ell}]\le 1$.

Considering all the target nodes $t \in [V]$, we have $(B_v, B_1, \lambda)=(|V|\sqrt{L}, |V|, 1)$.
\end{proof}

\subsection{Probabilistic Maximum Coverage Bandit~\cite{chen2016combinatorial,merlis2019batch}}
In this section, we consider the probabilistic maximum coverage (PMC) problem. PMC is modeled by a weighted bipartite graph $G=(L,V,E)$, where $L$ are the source nodes, $V$ is the target nodes and each edge $(u,v) \in E$ is associated with a probability $p(u,v)$. The task of PMC is to select a set $S \subseteq L$ of size $k$ so as to maximize the expected number of nodes activated in $V$, where a node $v \in V$ can be activated by a node $u \in S$ with an independent probability $p(u,v)$. PMC can naturally models the advertisement placement application, where $L$ are candidate web-pages, $V$ are the set of users, and $p(u,v)$ is the probability that a user $v$ will click on web-page $u$. 

PMC fits into the non-triggering CMAB framework: each edge $(u,v) \in E$ corresponds to a base arm, the action is the set of edges that are incident to the set $S \subseteq L$, the unknown mean vectors $\bmu \in (0,1)^E$ with $\mu_{u,v}=p(u,v)$ and we assume they are independent across all base arms. In this context, the reward function $r(S;\bmu)=\sum_{v\in V}(1-\prod_{u \in S}(1-\mu_{u,v}))$.

\begin{lemma}\label{lem:app_pmc}
PMC problem satisfies VM bounded smoothness condition (Condition~\ref{cond:VM}) with coefficient $(B_v,B_1)=(3\sqrt{2|V|},1)$.
\end{lemma}

\begin{proof}
We prove PMC satisfies VM condition by the definition of Gini-smoothness condition (Condition~\ref{cond:gini-smooth}) and \cref{lem:lemma6_no_trigger}.
First, we know $\frac{\partial r(S;\bmu)}{\partial \mu_{u,v}}=\prod_{i \in S, i \neq u} (1-\mu_{i,j}) \le 1$, thus $\gamma_{\infty}=1$. Also $\sqrt{\sum_{u \in S, v \in V}\mu_{u,v}(1-\mu_{u,v} \frac{\partial (r(S;\bmu)}{\partial \mu_{u,v}})^2}=\sqrt{\sum_{u \in S, v \in V} \mu_{u,v}(1-\mu_{u,v}) \prod_{i \in S, i \neq u} (1-\mu_{i,v})^2}= \sqrt{\sum_{v \in V} \sum_{u \in S}\left( \mu_{u,v} \prod_{i \in S,  i \neq u}(1-\mu_{i,v})\right)\left(\prod_{i \in S}(1-\mu_{i,v})\right)}\le \sqrt{\sum_{v\in V} 1/4}=\sqrt{|V|/4}$, where the second last inequality uses the fact consider $S$ coins and the $i$-th coin is up with prob. $\mu_{i,v}$, the first term $\left( \mu_{u,v} \prod_{i \in S,  i \neq u}(1-\mu_{i,v})\right)$ corresponds to probability $P_1$ that only one coin is up and the second term $\left(\prod_{i \in S}(1-\mu_{i,v})\right)$ corresponds to the probability $P_2$ that all coins are down, thus $P_1*P_2 \le P_1 (1-P_1)\le 1/4$. Hence $\gamma_g=\sqrt{V/4}$. By \cref{lem:lemma6_no_trigger}, we have $(B_v,B_1)=(3\sqrt{2}\gamma_g, \gamma_{\infty})=(3\sqrt{|V|/2},1)$. 
\end{proof}

==> content/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:TPVM} and \cref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Since this work is mainly about online learning models, algorithms and analytical techniques, there is no foreseeable societal impact.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \cref{sec:TPVM} and \cref{sec:independent}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See the Appendix.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{We only use open-sourced datasets and codes.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We only use open-sourced datasets and codes.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> content/experiments.tex <==
%%\vspace{-6pt}
\section{Experiments}\label{sec: experiments}
%%\vspace{-3pt}
\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/offline/fftwyt_uniform_overlapping_smaller_2500_3000_05.pdf}
		\caption{Offline, overlapping.}
		\label{fig: offline over fix}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/offline/fftwyt_uniform_non-overlapping_smaller_2500_3000_05.pdf}
		\caption{Offline, non-overlapping.}
		\label{fig: offline non over fix}
	\end{subfigure}
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/overlapping/new2_fftwyt_ci_overlapping_uniform_3000.pdf}
		\caption{Online, overlapping.}
		\label{fig: online over fix 3000}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.235\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/non-overlapping/icml_fftwyt_ci_non_overlapping_uniform_3000.pdf}
		\caption{Online, non-overlapping.}
		\label{fig: online non over fix 3000}
	\end{subfigure}
	%%\vspace{-10pt}
	\caption{Above: total weights of unique nodes visited for offline algorithms. Below: regret for online algorithms when $B=3000$.
	}\label{fig: offline algorithms}
\end{figure}

\begin{table}
\centering
%%\vspace{-5pt}
\caption{Statistics for FF-TW-YT network}
\label{tab: FF-TW-YT}
\begin{minipage}{0.90\columnwidth}
\begin{tabular}{cccc}
    \toprule
        Layer&FriendFeed & Twitter & YouTube  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     \# of vertices & 5,540 & 5,702 & 663 \\
     \# of edges & 31,921 & 42,327 & 614\\
     %FriendFeed (FF) & 5,540 & 31,921 \\
     %Twitter (TW) & 5,702 & 42,327 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
\end{minipage}
\end{table}

\begin{table*}[h]
\caption{Running time (seconds) for offline and online algorithms.}
% \vspace{-6pt}
    \begin{subtable}[h]{0.3\textwidth}
        \begin{minipage}{0.70\columnwidth}
        \begin{tabular}{cccccc}
    \toprule
     & B=2.6k & B=2.8k & B=3.0k  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     BEG & 0.274 & 0.316 & 0.363 \\
    %  MG & 0.028  & 0.031 &  0.033\\
     BEGE & 34.37  & 45.51 &  59.20 \\
     OPT & 91.16 & 98.42 &  105.63 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
\end{minipage}
       \caption{Running time of offline algorithms for the overlapping case with different budgets B.}
       \label{tab:offline, over}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.3\textwidth}
        \centering
        \begin{tabular}{cccc}
    \toprule
      & B=2.6k & B=2.8k & B=3.0k  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     DP & 0.038  & 0.044 &  0.050 \\
     MG & 0.008  & 0.009 &0.010\\
     OPT & 70.10  & 75.78 & 81.11 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
        \caption{Running time of offline algorithms for the non-overlapping case with different budgets B.}
        \label{tab:offline, non-over}
     \end{subtable}
     \hfill
         \begin{subtable}[h]{0.3\textwidth}
        \centering
        \begin{tabular}{ccc}
    \toprule
     Overlapping? & \checkmark  & $\times$  \\
     %Layer& \# of vertices & \# of edges  \\
     \midrule
     BEG & 1.22  & NA \\
     BEGE & 60.03  & NA\\
     DP  & NA  & 0.86  \\
     OPT & 107.33 & 82.01 \\
     %YouTube (YT) & 663 & 614 \\
     \bottomrule
\end{tabular}
        \caption{Per-round running time for CUCB-MAX (or CUCB-MG) with different oracles when B=3.0k.
%        	, NA means not applicable.
        }
        \label{tab:online}
     \end{subtable}
     \vspace{-10pt}
     \label{tab:runing time}
\end{table*}

\textbf{Dataset and settings.} We conduct experiments on a real-world multi-layered network FF-TW-YT, which contains $m=3$ layers representing users' social connections in FriendFeed (FF), Twitter (TW) and YouTube (YT)~\cite{dickison2016multilayer}.
% This multi-layered network is built upon the FF network, and the TW and YT layers are generated by exploiting the feature of FriendFeed as a social media aggregator.
In total, FF-TW-YT has $6,407$ distinct vertices representing users and $74,836$ directed edges representing connections (``who follows whom") among users.
The statistics for each layer is summarized in Table~\ref{tab: FF-TW-YT}.
% \textbf{Experimental settings.}
We transform the FF-TW-YT network $\cG(\cV,\cE)$ into a symmetric directed
network (by adding a new edge $(v,u)$ if $(u,v)\in \cE$ but $(v,u) \notin \cE$) because a user can be visited via her followers or followees.
Each edge weight is set to be $1$ and the node weights are set to be $\sigma_u\in\{0,0.5,1\}$ uniformly at random. 
Each random walker always starts from the smallest node-id in each layer and we set constraints $c_i$ equal to the total budget $B$. 
Note that in order to test the non-overlapping case, we use the same network but relabel node-ids so that they do not overlap between different layers.
To handle the randomness, we repeat $10,000$ times and present the averaged total weights of unique nodes visited for offline optimization.
We calculate the regret by comparing with the \textit{optimal} solution, which is stronger than comparing with $(1-e^{-\eta},1)$-approximate solution as defined in Eq.~(\ref{eq: alpha beta regret}).
We average over 200 independent experiments to provide the mean regret with 95\% confidence interval.
To evaluate the computational efficiency, we also present the running time for both offline and online algorithms in Table~\ref{tab:runing time}.

% \vspace{-2pt}
\noindent\textbf{Algorithms in comparison.}
For the offline setting, we present the results for Alg.~\ref{alg: layer traversal greedy} (denoted as BEG), Alg.~\ref{alg: pure greedy} (denoted as MG), BEG with partial enumeration (denoted as BEGE) and \OnlyInFull{Alg.~\ref{alg: dynamic programming}}\OnlyInShort{the dynamic programming algorithm in the supplementary material} (denoted as DP).
We provide two baselines PROP-S and PROP-W, which allocates the budget proportional to the layer size and proportional to the total weights if we allocate $B/3$ budgets to that layer, respectively.
The optimal solution (denoted as OPT) is also provided by enumerating all possible budget allocations. 
For online settings, we consider CUCB-MAX (Alg.~\ref{alg: over online}) and CUCB-MG \OnlyInFull{(Alg.~\ref{alg: non-over online})}\OnlyInShort{(Sec.~\ref{sec:cucbmg})} algorithms.
We shrink the confidence interval by $\gamma$, i.e., $\rho_{i,u,b} \leftarrow \gamma\rho_{i,u,b}$, to speed up the learning, though our theoretical regret bound requires $\gamma = 1$.
%Note that we no longer have theoretical guarantee when $\gamma < 1$, so the rest can be thought of heuristic algorithms.
For baselines, we consider the EMP algorithm which always allocates according to the empirical mean, and the $\epsilon$-Greedy algorithm which allocates budgets according to empirical mean with probability $1-\epsilon$ and allocates all $B$ budgets to the $i$-th layer with probability $\epsilon/m$.
We also compare with the Thompson sampling (TS) method~\cite{wang2018thompson}, which uses Beta distribution $\text{Beta}(\alpha,\beta)$ (where $\alpha=\beta=1$ initially) as prior distribution for each base arm.

% \vspace{-2pt}
\noindent\textbf{Experimental results.}
We show the results for \mulane{} problems in Figure~\ref{fig: offline algorithms}.
For the offline overlapping case, both BEG and MG outperform
two baselines PROP-W and PROP-S in receiving total weights.
Although not guaranteed by the theory, BEG are empirically close to BEGE and the optimal solution (OPT).
As for the computational efficiency, in Table~\ref{tab:offline, over}, the BEG is at least two orders of magnitude (e.g.,163 times when B=3.0k) faster than BEGE and OPT. 
Combining that the reward of BEG is empirically close to BEGE and the optimal solution, this shows that BEG is empirically better than BEGE and OPT.
For the offline non-overlapping case, the results are similar, but the difference is that we have the theoretical guarantee for the optimality of DP.
% For the online overlapping case, all CUCB-MAX curves grow sub-linearly w.r.t round $T$, due to the fact that our offline oracle achieves near optimal solutions.
% Comparing to two baselines, the CUCB-MAX ($\gamma=1.0$) curve has larger regret because it is relative conservative to theoretically guarantee the regret bound.
% As we decrease $\gamma$, the regret decreases and consistently outperforms baseline algorithms when $\gamma=0.1, 0.05$.
%Although the theoretical guarantee no longer holds when $\gamma < 1$, we have superior empirical performance, which 
For the online setting, all CUCB-MAX/CUCB-MG curves outperform the baselines.
This demonstrates empirically that CUCB-MAX algorithm can effectively learn the unknown parameters while optimizing the objective.
For the computational efficiency of online learning algorithms, since the running time for algorithms with the same oracle is similar, we present the running time for CUCB-MAX with different oracles in Table~\ref{tab:online}.
CUCB-MAX with BEG is 50 times faster than BEGE, which is consistent with our theoretical analysis.
% % For the non-overlapping case, we can observe that the CUCB-MG ($\gamma=1.0$) curve mostly lies between the baseline algorithms.
% % The CUCB-MG algorithm outperforms two baselines when $\gamma$ decreases to $0.5$.
% Interestingly, the regret of CUCB-MG ($\gamma=0.05$) is larger than CUCB-MG ($\gamma=0.01$), which is the opposite for overlapping cases.
% This is because the number of base arms is only $1/|\cV|$ of that for the overlapping case, which makes $\gamma=0.05$ too aggressive for the online learning process.
The results for different budgets $B$ are consistent with $B=3000$, which are included in the \OnlyInFull{Appendix~\ref{appendix: expriment for diff budgets}}\OnlyInShort{supplementary material}.
Results and analysis for stationary starting distributions are also in the\OnlyInFull{ Appendix~\ref{appendix: expriment for stationary distributions}}\OnlyInShort{supplementary material}.



























==> content/nips_rebuttal.tex <==
\clearpage
\section{Rebuttal}

\subsection{Reviewer HNeW: score 6 (weak accept), confidence 3}
\textbf{Is the notion of regret still $(\alpha, \beta)$-approximate regret in Section 4?}

We thank the reviewer for raising this good question. The regret in Section 4 is the exact regret, i.e., $\alpha=\beta=1$, since our SESCB algorithm (Algorithm 2) enumerates all possible solutions and selects the optimal one. 

Inspired by the reviewer's question, we can actually generalize our SESCB algorithm by allowing an $(\alpha, \beta)$-approximation oracle, similar to line 5 of our BCUCB-T algorithm. In particular, we can change lines 4-7 by defining $\bar{r}_t(S)$ for all $S \in \mathcal{S}$ instead of explicitly computing them. We then treat $\bar{r}_t(S)$ as a general set function, described by $2m$ parameters consisting of $m$ empirical means $\hat{\mu}_{t-1,i}$ and $m$ counters $T_{t,i}$, for $i \in [m]$. Now we assume an $(\alpha, \beta)$-approximation oracle $\bar{O}:[0,1]^m \times \mathbb{Z}^{m}\rightarrow \mathcal{S}$ which can produce
\begin{align}\label{apdx_eq:oracle_new}
   S=\bar{O}(\hat{\boldsymbol{\mu}}_{t-1}, \boldsymbol{T}_{t}) \text{ s.t. }  \Pr\left[\bar{r}_t(S)\ge \alpha \cdot \bar{r}_t(\bar{S}^*_t)\right] \ge \beta,
\end{align}
where $\bar{S}^*_t=\arg\max_{S\in \mathcal{S}} \bar{r}_t(S)$.
In this case, we can improve the computational efficiency of SESCB when there exists an efficient oracle that can 
	(approximately) optimize the set function $\bar{r}_t(S)$ over $S \in \mathcal{S}$. For the analysis, it is straightforward to change Eq. (136)-(139) as follows. 
\begin{align}
\Delta_S &= \alpha r(S^*; \boldsymbol{\mu}) - r(S;\boldsymbol{\mu})\\
&\le \alpha ( r(S^*;\hat{\boldsymbol{\mu}}_{t-1}) + \rho_t(S^*)) - r(S; \boldsymbol{\mu}) \\
&\le \bar{r}_t(S) - r(S; \boldsymbol{\mu})\\
&= r(S;\hat{\boldsymbol{\mu}}_{t-1}) + \rho_t(S) - r(S; \boldsymbol{\mu})  \\
&\le 2\rho_t(S),
\end{align}
where the first inequality is because of Eq. (135) over $S^*$, the second inequality is due to the $(\alpha, \beta)$-approximation oracle $\bar{O}$ mentioned above, and the last inequality is due to Eq. (135) over $S$.
Since the last inequality remains exactly the same as Eq. (139) in the previous version, this change does not affect later analysis. As for the $\beta$ part, we can apply the similar proof as in Eq. (54) to bound the regret when the oracle fails by $(1-\beta)T\Delta_{\max}$, which is absorbed by our $(\alpha, \beta)$-approximate regret definition, and the final regret bound remains unchanged. The only difference is that we have an $(\alpha, \beta)$-approximate regret, instead of the exact regret given by the enumeration. For the existence of such efficient oracles, see our PMC example in the response to Reviewer uueH. 

% \begin{align}
% \Delta_S &= \alpha r(S^*; \boldsymbol{\mu}) - r(S;\boldsymbol{\mu})\\
% &\le \alpha ( r(S^*;\hat{\boldsymbol{\mu}}_{t-1}) + \rho_t(S^*)) - r(S; \boldsymbol{\mu}) & \mbox{by \cref{apdx_eq:se_conf_interv} over $S^*$} \\
% &\le \bar{r}_t(S) - r(S; \boldsymbol{\mu}) & \mbox{$S$ is produced by $\bar{O}$ in \cref{apdx_eq:oracle_new}}\\
% &= r(S;\hat{\boldsymbol{\mu}}_{t-1}) + \rho_t(S) - r(S; \boldsymbol{\mu})  \\
% &\le 2\rho_t(S) & \mbox{by \cref{apdx_eq:se_conf_interv} over $S$},
% \end{align}
% \carlee{maybe mention the PMC example that you give in the response to Reviewer uueH here}
% \wei{This part does not account for the $\beta$ part in the $(\alpha,\beta)$-approximation oracle. We may need to say something about how we
% 	handle $\beta$ in our analysis.
% }
	
% To clarify the regret definition of both Theorem 1 and Theorem 2, we submit a revision where the green colored texts are revised contents. We also generalize Algorithm 2 by revising lines 4-9 and the analysis mentioned above as in Appendix D.2.

\textbf{About the experimental results.}

We thank the reviewer for this question. We have provided experiments to support the theoretical improvements of our work in the Appendix F. Specifically, we consider two representative applications, the combinatorial cascading bandits (Appendix F.1) and the PMC bandit (Appendix F.2), for the CMAB-T and the CMAB with independent arms, respectively. Compared with benchmark algorithms, our BCUCB-T algorithm achieves about 20\% less regrets for the combinatorial cascading bandits, and our SESCB achieves about 15\% less regrets for the PMC bandits. We will move these experimental results into our main paper in a future version.



\subsection{Reviewer uueH: score 7 (Accept), confidence 4}

\textbf{About the computationally efficient algorithm for SESCB (Algorithm 2).}

We thank the reviewer for the positive comments. The reviewer raises a concern about the computational efficiency of our SESCB algorithm, which can completely remove the $O(\log K)$ dependence. As we mentioned in line 318, the computation efficiency issue comes from the fact that the SESCB enumerates all possible actions, which is the same issue experienced by other ESCB-type algorithms that also use the brute force method, e.g., [8], [24].

One way to avoid the brute-force search is to introduce an $(\alpha,\beta)$-approximation oracle that could be efficient, as mentioned in our reply to the first question of reviewer HNeW. 
Generally speaking, we can define $\bar{r}_t(S)$ for all $S \in \mathcal{S}$ instead of explicitly computing them. We then treat $\bar{r}_t(S)$ as a general set function. Now can we assume an $(\alpha, \beta)$-approximation oracle $\bar{O}$ which can efficiently produce $S \in \mathcal{S}$ such that $\Pr\left[\bar{r}_t(S)\ge \alpha \cdot \bar{r}_t(\bar{S}^*_t)\right] \ge \beta$, where $\bar{S}^*_t=\arg\max_{S\in \mathcal{S}} \bar{r}_t(S)$. In this way, we can easily change the regret to $(\alpha,\beta)$-approximate regret to trade-off the efficiency. 

For the existence of such an oracle, the main difficulty lies in whether one can efficiently solve the optimization problem over a non-linear set function $r(S;\hat{\boldsymbol{\mu}}_{t-1})$ plus another non-linear set function $\rho_t(S)$.
In fact, we can find an efficient $(1-1/e, 1)$ greedy oracle when the reward function $r(S;\hat{\boldsymbol{\mu}}_{t-1})$ and $\rho_t(S)$ are both monotone submodular functions.

Take the PMC problem for example, for which $r(S;\bmu)$ is monotone submodular. To make the interval $\rho_t(S)=B_v\sqrt{\sum_{i \in S} \frac{C_1}{T_{t-1,i}}+ \max\left\{8C_1\sqrt{\sum_{i \in S}\frac{\log(2|\mathcal{S}|T)}{T_{t-1,i}^2}}, \frac{8C_1\log(2|\mathcal{S}|T)}{T^{\min}_{t-1, S}}\right\}}$ submodular, we can change it to $\rho'_t(S)=B_v\sqrt{\sum_{i \in S} \frac{C_1}{T_{t-1,i}}+ 8C_1\sqrt{\sum_{i \in S}\frac{\log(2|\mathcal{S}|T)}{T_{t-1,i}^2}}+ \frac{8C_1\log(2|\mathcal{S}|T)}{T^{\min}_{t-1, S}} }$, where the $\max$ is replaced with a sum ($+$). We know that $g(f(S))$ is submodular if $f(S)$ is submodular and $g$ is a non-decreasing concave function, so it suffices to show three terms within the (non-decreasing concave) square root  in $\rho'_t(S)$ are submodular. The first term is a modular function, the second term is the square root of a modular function, and the third term can be rewritten as $\max_{i \in S}\frac{8C_1\log(2|\mathcal{S}|T)}{T_{t-1, i}}$, which is also submodular. Now we can use the greedy oracle to maximize a new optimistic reward $\bar{r}_t(S)=r(S;\hat{\boldsymbol{\mu}}_{t-1})+\rho'_t(S)$ in our SESCB algorithm. As for the final regret, using $\rho'_t(S)$ instead of $\rho_t(S)$ only worsens the final regret by a constant factor, since it only affects the analysis of case 1 of Appendix D.2 by multiplying a factor of two in line 1006 to deal with the larger $\rho'_t$. Now compared with Merlis and Mannor [22] that achieves $(1-1/e, 1)$-approximate regret bound, our SESCB achieves the same $(1-1/e, 1)$-approximate regret bound but completely removes the $O(\log K)$ dependency. Moreover, our greedy oracle is efficient with computational complexity $O(TKL)$, where $T$ is the total number of rounds, $K$ is the number of source nodes to be selected in each round and $L$ is the total number of source nodes, which is much faster than our previous enumeration method. We will add the above discussion to improve the computational efficiency of SESCB.
% \wei{Why calling it a joint optimization? It makes me thinking about the pair oracle that jointly optimize for the action and the parameters, but this is not
% 	that case. I think it is just an optimization with a complicated non-linear reward function.
% 	Speaking of a non-linear set function, is it possible to show that $\bar{r}_t(S)$ is actually monotone submodular in some setting, such as PMC?
% 	Its first part $r(S)$ is monotone submodular, right? For the second part, it is a linear function under square root, so perhaps also monotone submodular?
% 	If so, we can at least get a constant approximation algorithm for this oracle, is that right? Then we can have a much better result for SESCB, with an
% 	efficient solution?
% }
% To the best of our knowledge, the only work that can solve this ESCB-type of oracle in polynomial time is [1] (i.e., [9] in our paper), which involves rounding/scaling, solving several budgeted linear optimization problems, and maximizing over the budget to get the final results. However, their paper is designed for the linear reward, i.e., $r(S;\boldsymbol{\mu})=\sum_{i \in S} \mu_i$, and their confidence interval does not contain the min-arm's counter $T^{\min}_{t-1,S}$ as ours, which prohibits the use of linear programming methods. Therefore, we cannot directly use their results to handle the SESCB algorithm, and it remains a challenging open problem on how to improve the efficiency of SESCB or ESCB with general reward functions.

% One way to avoid the brute-force search is to introduce an $(\alpha,\beta)$-approximation oracle that could be efficient, as mentioned in our reply to
% 	the first question of reviewer HNeW. 
% Roughly speaking, we can define $\bar{r}_t(S)$ for all $S \in \mathcal{S}$ instead of explicitly computing them. We then treat $\bar{r}_t(S)$ as a general set function. Now can we assume an $(\alpha, \beta)$-approximation oracle $\bar{O}$ which can efficiently produce $S \in \mathcal{S}$ such that $\Pr\left[\bar{r}_t(S)\ge \alpha \cdot \bar{r}_t(\bar{S}^*_t)\right] \ge \beta$, where $\bar{S}^*_t=\arg\max_{S\in \mathcal{S}} \bar{r}_t(S)$. In this way, we can easily change the regret to $(\alpha,\beta)$-approximate regret to trade-off the efficiency. For the existence of such an oracle, the main difficulty lies in whether one can efficiently solve the joint optimization problem over a non-linear set function $r(S;\hat{\mu}_{t-1})$ plus another set function $\rho_t(S)$ that is in the square-root form. 
% \wei{Why calling it a joint optimization? It makes me thinking about the pair oracle that jointly optimize for the action and the parameters, but this is not
% 	that case. I think it is just an optimization with a complicated non-linear reward function.
% 	Speaking of a non-linear set function, is it possible to show that $\bar{r}_t(S)$ is actually monotone submodular in some setting, such as PMC?
% 	Its first part $r(S)$ is monotone submodular, right? For the second part, it is a linear function under square root, so perhaps also monotone submodular?
% 	If so, we can at least get a constant approximation algorithm for this oracle, is that right? Then we can have a much better result for SESCB, with an
% 	efficient solution?
% }
% To the best of our knowledge, the only work that can solve this ESCB-type of oracle in polynomial time is [1] (i.e., [9] in our paper), which involves rounding/scaling, solving several budgeted linear optimization problems, and maximizing over the budget to get the final results. However, their paper is designed for the linear reward, i.e., $r(S;\boldsymbol{\mu})=\sum_{i \in S} \mu_i$, and their confidence interval does not contain the min-arm's counter $T^{\min}_{t-1,S}$ as ours, which prohibits the use of linear programming methods. Therefore, we cannot directly use their results to handle the SESCB algorithm, and it remains a challenging open problem on how to improve the efficiency of SESCB or ESCB with general reward functions.

% As a final remark, we also propose a computational-efficient algorithm, BCUCB-T, and reduces the batch-size dependency from $O(K)$ to $O(\log K)$, which can be used as an alternative when the efficiency is the first priority.

% [1] Cuvelier, T., Combes, R., \& Gourdin, E. (2021). Statistically efficient, polynomial-time algorithms for combinatorial semi-bandits. Proceedings of the ACM on Measurement and Analysis of Computing Systems, 5(1), 1-31.


\subsection{Reviewer kHgZ: score 7 (Accept), confidence 4}
\textbf{About the improvement over prior work in the disjunctive cascading bandit setting.}

We thank the reviewer for the positive comments. We agree with the reviewer that our regret does in fact have an extra $\log K$ term compared with [15], and we apologize for the confusion on this point. However, we believe it is reasonable to compare with [16] whose regret bound is $O(K\sum_{i}\frac{\log T}{\Delta_{i}})$, rather than with [15] whose regret bound is $O(\sum_{i}\frac{\log T}{\Delta_{i}})$. The reason is as follows.

The main difference between these two works lies in the set of feasible actions  $\mathcal{S}$.
For [15], $\mathcal{S}$ is the collection of all permutations whose size equals to $K$ (i.e., a uniform matroid). In this case, the items in the feasible solutions are \textbf{exchangeable} (a critical property for matroids), i.e., $S - \{e_1\} + \{e_2\} \in \mathcal{S}$, for any $S \in \mathcal{S}, e_1, e_2 \in [m]$. Based on the exchangeability property, [15] is able to define the item-wise sub-optimal gap $\Delta_{e,e^*}$ in Eq. (3) of [15] and the critical event $G_{e,e^*,t}$ in Theorem 1 of [15]. With these definitions, their proof is basically bounding the number of times that each suboptimal item $e$ is chosen instead of any optimal item $e^*$, which yields a batch-size independent regret bound $O(\sum_{i}\frac{\log T}{\Delta_{i}})$.

For [16], however, $\mathcal{S}$ (i.e., $\Theta$ in [16]) consists of arbitrary feasible actions (perhaps with different sizes), e.g., $S \in \mathcal{S}$ could refer to any path that connects the source and the destination in network routing applications.
[16] refers to cascading bandits with this kind of $\mathcal{S}$  as ``combinatorial cascading bandits", where items in the feasible actions may not be exchangeable (e.g., deleting an edge from a path and adding another edge may not be a valid path anymore). This means the item-wise definition of $\Delta_{e,e^*}$ and $G_{e,e^*, t}$ no longer works. Instead of using the $\Delta_{e,e^*}$, [16] uses another definition for the sub-optimal gap $\Delta_{e,\min}$ that is similar to our Definition 1, and applies a more general proof based on [17] that yields an extra $K$ factor. 

Similar to [7], [16], and [17], our CMAB-T formulation focuses on the arbitrary $\mathcal{S}$. In other words, our BCUCB-T algorithm and its analysis can deal with this general $\mathcal{S}$ whose feasible actions are not exchangeable. So we believe that we should compare [16] with our result, and it is unfair to compare ours with [15] that explicitly assumes $\mathcal{S}$ to be the uniform matroid, which enjoys the additional ``exchangeable property".
We will add this discussion in our final version to make it clear.
% \wei{I recovered this sentence. I think it is good to add this discussion in our final version, since readers may not be clear about the difference between [15] and [16]
% 	and they will only see that [15] is already $K$-free.
% }

\textbf{About the related works and the presentation.}

We thank the reviewer for mentioning three related works about variance-aware algorithms as well as the kind suggestion on our writing. For the related works, (A) is an interesting concurrent work that studies cascading bandits, which shares a similar variance-aware principle as ours. (A) studies two settings: the tabular case which is overlapped with us (though our work focuses on a slightly more general combinatorial cascading bandits [16], see the discussion above this reply) and the linear contextual cascading bandit case. Compared with the overlapped tabular case, our BCUCB-T achieves the matching regret bound when translating to gap-independent regret bound as in Appendix C.5.3. Interestingly, (A) also discusses the regret lower bound, which can show the tightness of our results as well. Moreover, our work is on a more general framework for CMAB-T, summarized by the TPVM condition, while (A) only focuses on cascading bandits.
For the linear contextual case studied by (A), we do not consider this setting in our work and it will be an interesting future direction to see whether the TPVM condition can also be applied to handle the linear contextual CMAB. For related works (B) and (C), we will add them to emphasize the timeliness of the current work as suggested. For the writing, we will add more examples (e.g., combinatorial cascading bandits) in the proofs and discussions to illustrate the intuitions of our definitions, assumptions, and proof techniques, which would be helpful for possible follow-up works.

% We thank the reviewer for mentioning three related works about variance-aware algorithms as well as the kind suggestion on our writing. For the related works, paper (A) is an insteresting concurrent work that studies cascading bandits, which shares a similar variance-aware principle as ours. Compared with paper (A), our BCUCB-T achieves the matching regret bound when translating to gap-independent regret bound as in Appendix C.5.3. Interestingly, Paper (A) also discusses the lower bound, which can show the tightness of our results as well. For the linear contextual case studied by Paper (A), we do not consider this setting in our work but it will be an interesting future direction to see whether the TPVM condition can also be applied to handle the linear contextual CMAB. For related works Paper (B) and Paper (C), we will consider adding them to emphasize the timeliness of the current work as suggested. For the writing, we will add more examples (e.g., combinatorial cascading bandits) to illustrate the intuitions of our definitions, assumptions, and proof techniques, which would be helpful for possible follow-up works.



% Is the notion of regret still $(\alpha, \beta)$-approximate regret in Section 4?

% We thank the reviewer for raising this good question. The regret in Section 4 is the exact regret, i.e., $\alpha=\beta=1$, since our SESCB algorithm (Algorithm 2) enumerates all possible solutions and selects the optimal one. 

% Inspired by the reviewer's question, we can actually generalize our SESCB algorithm by allowing an $(\alpha, \beta)$-approximation oracle, similar to line 5 of our BCUCB-T algorithm. In particular, we can change lines 4-7 by defining $\bar{r}\_t(S)$ for all $S \in \mathcal{S}$ instead of explicitly computing them. We then treat $\bar{r}\_t(S)$ as a general set function, described by $2m$ parameters consisting of $m$ empirical means $\hat{\mu}\_{t-1,i}$ and $m$ counters $T\_{t,i}$, for $i \in [m]$. Now we assume an $(\alpha, \beta)$-approximation oracle $\bar{O}:[0,1]^m \times \mathbb{Z}^{m}\rightarrow \mathcal{S}$ which can produce
% \begin{align}
%   S=\bar{O}(\hat{\boldsymbol{\mu}}\_{t-1}, \boldsymbol{T}\_{t}) \text{ s.t. }  \text{Pr}\left[\bar{r}\_t(S)\ge \alpha \cdot \bar{r}\_t(\bar{S}^\*\_t)\right] \ge \beta,
% \end{align}
% where $\bar{S}^\*\_t=\arg\max\_{S\in \mathcal{S}} \bar{r}\_t(S)$.
% In this case, we can improve the computational efficiency of SESCB when there exists an efficient oracle that can 
% 	(approximately) optimize the set function $\bar{r}\_t(S)$ over $S \in \mathcal{S}$. For the analysis, it is straightforward to change Eq. (136)-(139) as follows,
% \begin{align}
% \Delta\_S &= \alpha r(S^*; \boldsymbol{\mu}) - r(S;\boldsymbol{\mu})\\\\
% &\le \alpha ( r(S^*;\hat{\boldsymbol{\mu}}\_{t-1}) + \rho\_t(S^*)) - r(S; \boldsymbol{\mu}) \\\\
% &\le \bar{r}\_t(S) - r(S; \boldsymbol{\mu})\\\\
% &= r(S;\hat{\boldsymbol{\mu}}\_{t-1}) + \rho_t(S) - r(S; \boldsymbol{\mu})  \\\\
% &\le 2\rho\_t(S),
% \end{align}
% where the first inequality is because of Eq. (135) over $S^*$, the second inequality is due to the $(\alpha, \beta)$-approximation oracle $\bar{O}$ mentioned above, and the last inequality is due to Eq. (135) over $S$.
% Since the last inequality remains exactly the same as Eq. (139) in the previous version, this change does not affect later analysis. As for the $\beta$ part, we can apply the similar proof as in Eq. (54) to bound the regret when the oracle fails by $(1-\beta)T\Delta_{\max}$, which is absorbed by our $(\alpha, \beta)$-approximate regret definition, and the final regret bound remains unchanged. The only difference is that we have an $(\alpha, \beta)$-approximate regret, instead of the exact regret given by the enumeration. For the existence of such efficient oracles, see our PMC example in the response to Reviewer uueH. 

% About the improvement over prior work in the disjunctive cascading bandit setting.

% We thank the reviewer for the positive comments. We agree with the reviewer that our regret does in fact have an extra $\log K$ term compared with [15], and we apologize for the confusion on this point. However, we believe it is reasonable to compare with [16] whose regret bound is $O(K\sum_{i}\frac{\log T}{\Delta_{i}})$, rather than with [15] whose regret bound is $O(\sum_{i}\frac{\log T}{\Delta_{i}})$. The reason is as follows.

% The main difference between these two works lies in the set of feasible actions  $\mathcal{S}$.
% For [15], $\mathcal{S}$ is the collection of all permutations whose size equals to $K$ (i.e., a uniform matroid). In this case, the items in the feasible solutions are **exchangeable** (a critical property for matroids), i.e., $S - \{e_1\} + \{e_2\} \in \mathcal{S}$, for any $S \in \mathcal{S}, e_1, e_2 \in [m]$. Based on the exchangeability property, [15] is able to define the item-wise sub-optimal gap $\Delta_{e,e^*}$ in Eq. (3) of [15] and the critical event $G_{e,e^*,t}$ in Theorem 1 of [15]. With these definitions, their proof is basically bounding the number of times that each suboptimal item $e$ is chosen instead of any optimal item $e^*$, which yields a batch-size independent regret bound $O(\sum_{i}\frac{\log T}{\Delta_{i}})$.

% For [16], however, $\mathcal{S}$ (i.e., $\Theta$ in [16]) consists of arbitrary feasible actions (perhaps with different sizes), e.g., $S \in \mathcal{S}$ could refer to any path that connects the source and the destination in network routing applications.
% [16] refers to cascading bandits with this kind of $\mathcal{S}$  as "combinatorial cascading bandits", where items in the feasible actions may not be exchangeable (e.g., deleting an edge from a path and adding another edge may not be a valid path anymore). This means the item-wise definition of $\Delta_{e,e^*}$ and $G_{e,e^*, t}$ no longer works. Instead of using the $\Delta_{e,e^*}$, [16] uses another definition for the sub-optimal gap $\Delta_{e,\min}$ that is similar to our Definition 1, and applies a more general proof based on [17] that yields an extra $K$ factor. 

% Similar to [7], [16], and [17], our CMAB-T formulation focuses on the arbitrary $\mathcal{S}$. In other words, our BCUCB-T algorithm and its analysis can deal with this general $\mathcal{S}$ whose feasible actions are not exchangeable. So we believe that we should compare [16] with our result, and it is unfair to compare ours with [15] that explicitly assumes $\mathcal{S}$ to be the uniform matroid, which enjoys the additional "exchangeable property".
% We will add this discussion in our final version to make it clear.

==> content/related.tex <==
\vspace{-9pt}
\subsection{Related Work}\label{sec: related work}
\vspace{-5pt}

The multi-armed bandit (MAB) problem is first studied by \citet{robbins1952some} and then extended by many studies (cf. \cite{bubeck2012regret, slivkins2019introduction, lattimore2020bandit}). As mentioned earlier, the stochastic CMAB has received much attention recently. From the model view, these CMAB works can be divided into two categories: CMAB with (i.e. CMAB-T setting) or without probabilistically triggered arms (i.e. non-triggering CMAB). For the former category , our work improves (a) the general framework by \cite{chen2016combinatorial, wang2017improving} (b) the combinatorial cascading bandit \cite{kveton2015combinatorial} (c) the online influence maximization bandits \cite{wang2017improving, perrault2020budgeted}, reducing or removing the batch-size dependent factor $K$ in the regret bounds based on our newly proposed TPVM condition and/or our refined analysis. We defer the detailed technical comparison to \cref{sec:TPVM} and \cref{sec:app}. For the latter category, \cite{gai2012combinatorial} is the first study on stochastic CMAB, and its regret has been improved by \citet{kveton2015tight}, \citet{combes2015combinatorial}, \citet{chen2016combinatorial}, but they still have $O(K)$ factor in their regret. When arms are mutually independent, \citet{combes2015combinatorial} propose the Efficient Sampling for Combinatorial Bandit policy (ESCB), which reduces the dependence on $O(K)$ to $O(\log^2 K)$ at the cost of high computational complexity. Later on, the computational complexity is improved by AESCB~\cite{cuvelier2021statistically} in linear CMAB problem. Recently, \citet{merlis2019batch} focus on the PMC bandit problem and propose the BC-UCB algorithm with the Gini-smoothness condition to achieve the similar improvement as ESCB/AESCB, even without the independent arm assumption. Our work is largely inspired by their work but we propose a new TPVM condition to handle the CMAB-T setting for much broader application scenarios. In addition, we provide refined analysis with an additional $O(\log K)$ factor improvement (which is also appliable for the analysis of BC-UCB and ESCB) and totally remove the dependence on $K$ under the setting of independent arms by our new SESCB algorithm. The detailed comparisons are summarized in \cref{tab:triggering} and \cref{tab:non-triggering}.

From the algorithm view, there are three major approaches for CMAB: Combinatorial Upper Confidence Bound (CUCB) \cite{auer2002finite, gai2012combinatorial, kveton2015tight,wang2017improving,merlis2019batch}, ESCB \cite{combes2015combinatorial,cuvelier2021statistically} and Combinatorial Thompson Sampling (CTS) \cite{thompson1933likelihood,wang2018thompson}. For CMAB-T, most CUCB-type algorithms use Chernoff concentration bounds \cite{wang2017improving}, our BCUCB-T algorithm is different and leverages on the Bernstein concentration bound \cite{audibert2009exploration,merlis2019batch} that considers variance of the arms. For the non-triggering CMAB with independent arms, we are the first to utilize the concentration of Sub-Exponential random variables, compared with other ESCB-type algorithms. \citet{wang2018thompson} study CTS algorithms with comparable regrets to CUCB and AESCB, but they require an exact offline oracle instead of a general $(\alpha,\beta)$-approaximate oracle.
%optimism in the face of uncertainty
%a tighter ellipsoidal confidence region around the empirical mean, which helps to better restrict the exploration

From the application view, this paper mainly studies the applications of PMC bandit~\cite{merlis2019batch}, cascading bandits~\cite{kveton2015combinatorial,li2016contextual}, network exploration~\cite{liu2021multi}, and online influence maximization~\cite{wen2017online,wang2017improving, li2020online}. There are other potential CMAB applications that could be included in our framework, such as matching bandits~\cite{liu2021bandit}, online crowdsourcing bandits\cite{gao2020combinatorial}.

% %\textbf{Related Work}
% Network exploration via random walks has been studied in various application contexts such as community detection~\cite{pons2005computing}, centrality measuring~\cite{gleich2015pagerank},
% 	large-scale network sampling~\cite{li2019walking}, and influence maximization~\cite{wilder2018maximizing}.
% Multiple random walks has also been used, e.g. in~\cite{lv2002search} for query resolution in peer-to-peer networks.
% However, none of these studies address the budgeted MuLaNE problem.
% % (I think this part can be removed if we have no space.)
% \mulane{} is also related to the influence maximization (IM) problem~\cite{kempe2003maximizing, chen2009efficient} and can be viewed as a special variant of IM. 
% Different from the standard Independent Cascade (IC) model~\cite{wang2012scalable} in IM, which randomly broadcasts to all its neighbors, the propagation process of \mulane{} is a random walk that selects one neighbor. Moreover, each unit of budget in \mulane{} is used to propagate one random-walk step, not to select one seed node as in IC. 

% The offline budget allocation problem has been studied by \citet{alon2012optimizing,soma2014optimal}, the latter of which
% propose the lattice submodularity and a constant approximation algorithm based on this property.
% Our offline overlapping MuLaNE setting is based on a similar approach, but we provide a better approximation ratio compared to the original analysis in~\cite{alon2012optimizing}.
% Moreover, we further show that the stationary setting enjoys DR-submodularity, leading to an efficient algorithm with a better approximation ratio.


% The multi-armed bandit (MAB) problem is first studied by \citet{robbins1952some} and then extended by many studies
% (cf. \cite{BCB12}).
% Our online MuLaNE setting fits into the general Combinatorial MAB (CMAB) framework of~\cite{gai2012combinatorial,chen2016combinatorial}.
% CUCB is proposed as a general algorithm for CMAB~\cite{chen2016combinatorial}.
% Our study includes several adaptations, such as handling unknown node weights, defining intermediate random variables as base arms and so on.


% \citet{chen2018community} study the community exploration problem, which is essentially a special case of MuLaNE with
% 	non-overlapping complete graphs.
% As a result, their technique is different and much simpler than ours. 

% The rest of the paper is organized as follows. 
% Section \ref{sec: problem setting} states the settings of \mulane;
% Section \ref{sec: equivalent model} states the equivalent bipartite coverage model to derive the explicit form for our reward function;
% Section \ref{sec: offline opt} states offline algorithms for four offline settings with provable approximation guarantee and running time analysis;
% Section \ref{sec: online learning} states two online learning algorithms with regret analysis;
% Empirical results are shown in Section \ref{sec: experiments};
% and Section \ref{sec: conclusion} concludes the paper.


